Cooperative Infrastructure Perception

Recent works have considered two qualitatively different approaches to overcome line-of-sight limitations of 3D sensors used for perception: cooperative perception and infrastructure-augmented perception. In this paper, motivated by increasing deployments of infrastructure LiDARs, we explore a third approach, cooperative infrastructure perception. This approach generates perception outputs by fusing outputs of multiple infrastructure sensors, but, to be useful, must do so quickly and accurately. We describe the design, implementation and evaluation of Cooperative Infrastructure Perception (CIP), which uses a combination of novel algorithms and systems optimizations. It produces perception outputs within 100 ms using modest computing resources and with accuracy comparable to the state-of-the-art. CIP, when used to augment vehicle perception, can improve safety. When used in conjunction with offloaded planning, CIP can increase traffic throughput at intersections.

==> 0_metadata.tex <==
\ifcameraready
\ifacmartsty
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10003033.10003106.10003112</concept_id>
<concept_desc>Networks~Cyber-physical networks</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10010520.10010521.10010542.10011714</concept_id>
<concept_desc>Computer systems organization~Special purpose systems</concept_desc>
<concept_significance>300</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Networks~Cyber-physical networks}
\ccsdesc[300]{Computer systems organization~Special purpose systems}
\fi

\keywords{Autonomous Cars, ADAS, Collaborative Sensing, Extended Vision}

\newcommand{\grantack}[1]{
  \ifthenelse{\equal{#1}{CTA}}{\thanks{Research was sponsored by the Army Research Laboratory and was accomplished under Cooperative Agreement Number W911NF-09-2-0053 (the ARL Network Science CTA). The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied, of the Army Research Laboratory or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for Government purposes notwithstanding any copyright notation here on.}
    }{}
  \ifthenelse{\equal{#1}{CRA}}{\thanks{Research reported in this paper was sponsored in part by the Army Research Laboratory under Cooperative Agreement W911NF-17-2-0196. The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied, of the Army Research Laboratory or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for Government purposes notwithstanding any copyright notation here on.}}{}
  \ifthenelse{\equal{#1}{Conix}}{\thanks{This work was supported in part by the CONIX Research Center, one of six centers in JUMP, a Semiconductor Research Corporation (SRC) program sponsored by DARPA.}}{}
  \ifthenelse{\equal{#1}{NSFAvail}}{\thanks{This material is based upon work supported by the National Science Foundation under Grant No. 1705086}}{}
  \ifthenelse{\equal{#1}{Conix}}{\thanks{This work was supported in part by the CONIX Research Center, one of six centers in JUMP, a Semiconductor Research Corporation (SRC) program sponsored by DARPA.}}{}
  \ifthenelse{\equal{#1}{CPSSyn}}{\thanks{This material is based upon work supported by the National Science Foundation under Grant No. 1330118 and from a grant from General Motors.}}{}        
  \ifthenelse{\equal{#1}{NeTSLarge}}{\thanks{This material is based upon work supported by the National Science Foundation under Grant No. 1413978}}{}         \ifthenelse{\equal{#1}{NeTSSmall}}{\thanks{This material is based upon work supported by the National Science Foundation under Grant No. 1423505}}{}
}

%%% Uncomment one or more of the following
%\grantack{CTA}
%\grantack{CRA}
%\grantack{NSFAvail}
%\grantack{CPSSyn}
%\grantack{NeTSLarge}
%\grantack{NeTSSmall}

\fi

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> application.tex <==
\section{Applications}
\label{sec:applications}

% Application
% - Intersections
% - ....



==> background.tex <==
\section{Background}
\label{sec:background}

Self-driving vehicles consist of three logical components~\cite{paden2016survey,pendleton2017perception}: perception, planning, and control (\figref{fig:av_stack}). 

\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\columnwidth]{figs/fig_autonomous_driving_stack.pdf}
  \caption{Self-driving stack}
  \label{fig:av_stack}
\end{figure}

\parab{Perception.} To perceive and extract knowledge about the world, a self-driving vehicle uses one or more \textit{3D sensors} capable of depth perception (\eg radars, stereo cameras, and LiDARs). A LiDAR, for example, sends millions of light pulses per second in all directions, whose reflections enable the LiDAR to estimate the depth of different parts of the environment. The output of a LiDAR is a 3D \textit{point cloud} that contains \textit{points} associated with 3D positions. Stereo cameras also output point clouds, but estimate depth using the positions of pixels in the left and right images of their two cameras.

A self-driving vehicle's \textit{perception module} extracts static and dynamic objects from these point clouds. Static objects include road surfaces, lane markers~\cite{lanedetection}, and safe drivable space~\cite{drivablespace}. The module also identifies dynamic objects (other vehicles, pedestrians, bicyclists) and tracks them. Finally, it estimates the vehicle's own position, using SLAM (Simultaneous Localization and Mapping)~\cite{slam_part1,slam_part2} algorithms. 

% understand the scene around it, detect drivable space, and localize itself (\figref{fig:av_stack}). First, the module segments the scene it sees through its sensors into static and dynamic objects. For this, it can use semantic segmentation tools~\cite{DeepLab}, background subtraction~\cite{Octree}, and ground-plane extraction~\cite{groundplane} \etc. Then, it extracts the road surface, detects lane markers~\cite{lanedetection} and safe drivable space~\cite{drivablespace}. To localize the vehicle, the perception module matches \textit{features} in its point cloud with those in SLAM (Simultaneous Localization and Mapping)~\cite{slam_part1,slam_part2} generated \textit{3D maps}~\cite{CarMap}. The map contains the positions of the matched features, using which the vehicle can triangulate its own position.

% and are constructed from LiDARs or 
% cameras (multi-view stereo~\cite{colmap}).

% These maps are dense reconstructions of the physical world 
% around the vehicle and enable it to see beyond it's sensors' range.
% SLAM uses cameras~\cite{ORB-SLAM2} or LiDARs~\cite{LOAM} along 
% with other sensors (GPS) to precisely localize a vehicle by 
% tracking static features in its surroundings.   
%% \ramesh{Do they use SLAM, or SLAM-generated maps? Also, consider whether this detail is important from the perspective of the story. Do we use SLAM anywhere else? If we only plan to make a passing reference, may introduce it there.}
%% \fawad{I think it might be important because we will have a localization experiment later on and then we need to compare our approach with what autonomous vehicles have now.}

%% 2.2 Control
\parab{Planning.} The planning module uses the outputs of the perception module to plan and execute a safe path for the vehicle, while satisfying performance and comfort objectives~\cite{paden2016survey} (\eg smooth driving, minimal travel time \etc). Planning consists of three sub-tasks, distinguished by the time-scales at which they operate.

% Route planning module
\textit{Route planning}, usually executed once per trip, determines a safe \textit{path} (represented as a sequence of way-points through the road network) for the vehicle from the origin to the destination. \textit{Behavior planning}, which operates at time-scales of a few seconds, uses the path way-points and information about other objects and traffic participants (pedestrians, vehicles) to determine a set of driving maneuvers (\eg intersection navigation, lane-following, right turn at stop sign, parking \etc) for the vehicle to use at each part of the planned path. \textit{Motion planning} converts behaviors into short-term \textit{trajectories} (at the timescale of 100s of milliseconds) that the vehicle must follow. A trajectory is a sequence of way-points, together with the precise times at which the vehicle must arrive at those way-points.

\parab{Control.} This component takes a trajectory and converts it, at millisecond timescales, to low-level actuator (\eg throttle, steering, brake) signals. 

%% that uses actuator signals to ensure the vehicle follows the planned 
%% trajectory and minimizes errors in doing so. The vehicle runs the 
%% control module as fast as possible (every millisecond).

%%  \ramesh{In the previous para, do we want to mention the timescales at which these decisions happen? This will be crucial in deciding what we can offload, and what we cannot. Also, in the writing above, you can make it clear what are the inputs/outputs of each stage.}
%%  \fawad{Addressed.}
%%  \ramesh{Your writing has fewer passive voice sentences than it used to, which is good. There are a couple in the para above: behaviors are represented, are caused etc.}
%% \fawad{Addressed.}

%  \ramesh{Do we need the rest of this text? Doesn't seem relevant for our paper. Might be important to discuss briefly in related work, though.}
 

% Move to related work section
% \parab{Connected \& Automated Vehicles.}
% Introducing connectivity and coordination between autonomous vehicles 
% and the infrastructure can reduce sources of uncertainty, enabling 
% safer, and energy-efficient driving. An example of a proposed 
% control and planning architecture for such a 
% system~\cite{guanetti2018control} decouples real-time safety-critical 
% control tasks at the vehicle from 
% remote routing and planning at the cloud. The real-time control 
% module consists of powertrain control, motion control, and 
% motion planning. The remote planning mostly provides routing 
% information but also dynamic road maps, historical traffic 
% data and external compute for non-safety critical tasks. 
% We describe various components of the architecture briefly 
% below because it is similar, in some ways, to our proposed system.

% In such this architecture, remote planning and routing modules 
% perform longer timescale planning using historical data and maps 
% for efficient trip planning. It consists of eco-routing, 
% eco-driving and battery charge planning sub-modules. The 
% eco-driving and routing modules orchestrate vehicles into 
% fleets of vehicle that travel together called platoons. As platoons, 
% coordinated driving reduces frequent speed changes to increase 
% fuel efficiency. Moreover, the battery charge planning 
% module benefit from more extensive and accurate forecasts available 
% to intelligently plan recharge cycles. 

% The real-time motion planning module coordinates with the 
% remote modules to plan a paths for vehicles within the platoons 
% using cooperative adaptive cruise control. It performs  
% functions like collision avoidance and lane-changing but enhances them 
% cooperative perception and control. 
% Motion control governs the longitudinal (acceleration) and 
% lateral (steering) motion of the car along the planned path. 
% This module uses cooperative adaptive cruise control with enabled 
% by cooperative perception for closed-loop in-vehicle robustness. 
% Lastly, powertrain controls supply energy required to move the car 
% (\eg engine on/off, gear control). In a connected architecture, 
% powertrain control is more efficient because traffic forecasts 
% are made available by cooperative perception and maps and 
% this allows more-informed energy-planning.





%% End Ramesh's outline

% Background:
% - LiDAR/depth-perception: these are becoming cheap

% - Background on vehicular control (reading)
% \subsection{Vehicle Control}
% \label{sec:bg_vehicle_control}
% Based on the degree of autonomy, the Levels of Autonomous Driving:
% Level 0: human-driven
% Level 1: driver-assists like adaptive cruise control, anti-lock braking systems and electronic stability control.
% Level 2: advanced assistance such as hazard-minimizing longitudinal/lateral control [19] or emergency braking [20], [21], based upon set-based formal control theoretic methods to compute ‘worst-case’ sets of provably collision free (safe) states [22]–[24].
% Level 3: the system monitors the environment and can drive with full autonomy under certain conditions, but the human operator is still required to take control if the driving task leaves the autonomous system’s operational envelope. 
% Level 4: vehicle is capable of fully autonomous driving in certain conditions and will safely control the vehicle if the operator fails to take control upon request to intervene.
% Level 5: systems are fully autonomous in all driving modes.

% Connected vehicles:
% Improve throughput at intersections and reduce shockwaves


==> background_sensys.tex <==
\section{Background}
\label{sec:background}
In this section, we provide background which is necessary to understand our contributions, and \sysname's application to two use cases (\secref{s:use_cases}) in autonomous driving \ie extending a vehicle's perception, and improving throughput with a centralized planner.

\parab{LiDAR.} A LiDAR sends millions of light pulses per second in all directions.
The reflections of these pulses enable the LiDAR to estimate the depth of different parts of the environment. 
The output of a LiDAR is a \textit{point cloud} that contains \textit{points} associated with 3D positions. 
Similar to human vision, LiDARs also have line-of-sight limitations and hence are prone to occlusions. 
This has serious safety implications for human-driven and autonomous vehicles.
The NHTSA~\cite{NHTSA-precrash} has identified several scenarios (as demonstrated in \figref{fig:red_light_violation} and \figref{fig:unprotected_left_turn}) where occlusions can result in traffic accidents for both human-driven and autonomous vehicles.

\parab{Perception.}
Self-driving vehicles consist of three logical components~\cite{paden2016survey,pendleton2017perception}: perception, planning, and control. 
A self-driving vehicle's \textit{perception module} extracts static and dynamic objects from LiDAR point clouds. Static objects include road surfaces, lane markers~\cite{lanedetection}, and safe drivable space~\cite{drivablespace}. The module also identifies dynamic objects (\eg other vehicles, pedestrians, bicyclists) and tracks them. Finally, it estimates the vehicle's own position using SLAM (Simultaneous Localization and Mapping)~\cite{slam_part1,slam_part2} algorithms. 

\parab{Planning.} The planning module uses the outputs of the perception module to plan and execute a safe path for the vehicle, while satisfying performance and comfort objectives~\cite{paden2016survey} (\eg smooth driving, minimal travel time \etc). Planning consists of three sub-tasks, distinguished by the time-scales at which they operate.
% Route planning module
\textit{Route planning}, usually executed once per trip, determines a safe \textit{path} (represented as a sequence of way-points through the road network) for the vehicle from the origin to the destination. \textit{Behavior planning}, which operates at time-scales of a few seconds, uses the path way-points and information about other objects and traffic participants (pedestrians, vehicles) to determine a set of driving maneuvers (\eg intersection navigation, lane-following, right turn at stop sign, parking \etc) for the vehicle to use at each part of the planned path. \textit{Motion planning} converts behaviors into short-term \textit{trajectories} (at the timescale of 100s of milliseconds) that the vehicle must follow. A trajectory is a sequence of way-points, together with the precise times at which the vehicle must arrive at those way-points.

\parab{Control.} This component takes a trajectory and converts it, at millisecond timescales, to low-level actuator (\eg throttle, steering, brake) signals. 


==> controller.tex <==
% \add{
\section{\sysname Local Controller}
\label{sec:controller}

Every \sysname-compatible vehicle has an on-board local low-level controller and PID controller that receives the set of planned way-points from the centralized planner over the network. The local controller translates these to low-level control signals (throttle, steer, and brake) that can be directly applied to each vehicle. The local controller runs every 2-3~ms in the vehicle. 

The local controller, on-board every vehicles, receives the planned trajectory (for that vehicle) from the centralized planner every 100~ms.
If the local controller does not receive a trajectory from the centralized planner within a latency budget (\eg due to network failure), it initiates a recovery mode.
In the recovery mode, it uses the last valid trajectory received by the vehicle in a previous cycle. The local controller can afford to do this because the planner plans, and sends a trajectory for a longer time horizon (\secref{s:planner}). It would have sufficed to send the vehicle its trajecotry for just the next 100~ms but instead, \sysname sends a trajectory for the next $x$ seconds. This redundancy in the design not only addresses network failures but also helps relax SIPP's instant start/stop assumption and introduces robustness.

% \ramesh{The previous paragraph is important from a networking perspective. This idea is similar to soft state that permits robustness; see the Clark paper in the 551 readings.}

Given the planned trajectory for the next $x$ seconds, the controller determines whether the vehicle has to wait at any point along its planned trajectory. We call this a wait cycle. If there is a wait cycle, it finds the position associated with the wait cycle and the distance of the vehicle from it. The controller then calculates the braking distance (distance to bring the vehicle to a complete stop) of the vehicle using its motion vector. If the braking distance is less than or equal to the distance from the stopping point, the controller generates a signal to apply brake. Without this, vehicles would apply brakes at the spatial position of the wait cycle and hence overshoot it. With this maneuver, \sysname ensures that vehicles can adhere to SIPP's collision-free planned paths. On the other hand, if the vehicle is far away from the stopping point, then the controller generates a signal to continue moving the vehicle towards the stopping point. We calculate braking distance using a standard equation~\cite{brakingdistance}.% and multiply it with a safety factor for robustness.

% \ramesh{I couldn't find where wait cycle was previously defined.}
% \fawad{Addressed.}

If there is no wait cycle in the entire trajectory, the controller selects the next suitable way-point and generates a signal to move the vehicle towards that way-point. Finally, the local controller applies the control signal to the vehicle.


==> deployment.tex <==
\section{Deployment Scenarios}
\label{sec:deployment}
% Deployment scenarios
We envision three deployment scenarios for \sysname as follows. For 
each scenario, we also discuss reliability and benefit costs.
% - Full

\parab{Full deployment.}
% Full deployment means all vehicles will use \sysname
% Vehicles can afford to have fewer sensors and less compute
% For instance, cruise control will be implemented at the edge
In a full deployment, all roads will have infrastructure sensors and edge compute. As such, all self-driving vehicles will rely on them for perception and planning. Today, self-driving cars have a plethora of on-board sensors and powerful compute platforms. This increases the price of a self-driving car by an order of magnitude relative to a human-driven vehicle~\cite{qzvehiclecost,reutersvehiclecost}. By sharing infrastructural resources amongst vehicles, \sysname can significantly lower the cost of self-driving cars. Moreover, with ubiquitous infrastructural LiDARs generating a real-time view of the road, self-driving vehicles will not need pre-built 3D maps. Collecting and building these maps would otherwise cost a few thousand dollars per kilometer~\cite{3dmapcost}.

\ramesh{What about map collection? Point out that we may not need this as well? Reference papers about its cost.}
\fawad{Could not find a paper but found an article instead.}

Moreover, \sysname's centralized approach promises more reliable autonomous driving. For instance, in a full deployment, applications like adaptive cruise control (ACC) will run at the edge. With better perception and coordinated control, ACC can plan more efficient, and safer trajectories for vehicles. Similarly, \sysname can also coordinate vehicles into platoons to for safer driving and increase road throughput by 2x~\cite{varaiyaplatoons}. A platoon is set of tightly coordinated vehicles that move together through traffic~\cite{varaiyaplatoons,platooning2011}. Platooning enables efficient driving because it reduces air resistance, and frequent stops. On the other hand, it also makes driving safer because all vehicles move at the same speed with fixed headway distances.

\ramesh{Why ACC in particular? Also point to platooning? Add references to platooning?}
\fawad{Addressed, would ACC and platooning be enough? Or should we add more applications}

\parab{Augmentation.}
In this deployment, self-driving vehicles will have their on-board sensors and compute but \sysname will augment them. Augmentation deployments can help in in high-risk and high-traffic regions like accident-prone areas, traffic intersections, and highways \etc. 

% Improving reliability through better perception
Occlusions and line-of-sight limits a self-driving vehicle's perception~\cite{AVR}. \sysname can extend a vehicle's vision beyond its sensor range. For instance, in \figref{fig:sys_overtaking}, \sysname can send 3D sensor data (raw point clouds, bounding boxes, or occupancy grids \etc) to the blue vehicle to enable it to see more. This way, the blue vehicle can not only avoid a unsafe maneuver and also save fuel. Similarly, in traffic intersections, \sysname can inform left-turning vehicles of oncoming traffic in the opposite lanes.
% Improving reliability through edge compute
Similarly, \sysname can provision edge compute to self-driving vehicles for heavy, relatively less latency-sensitive computations. This way, vehicles can use on-board compute for safety-critical and latency-sensitive tasks instead.

When \sysname is augmented in high-risk areas, self-driving vehicles can afford to have fewer on-board sensors and less powerful compute. This reduces the per unit cost of self-driving vehicles.

\ramesh{Also point out cost implications: may need fewer sensors on cars, if, for the difficult cases, infrastructure can augment perception and planning. Discuss where the augmentation will be deployed: high-traffic areas, intersections, places with accidents. Also, augmentation doesn't have to mean point cloud transmissions, can transmit other representations such as bounding boxes etc.}
\fawad{Addressed.}

\parab{Backwards compatible.}
% Backwards compatible facilitates legacy vehicles
Human-driven vehicles can also draw benefits from \sysname through vision extension, accident warnings or emergency controls. To extend vision, \sysname can share infrastructure 3D sensor data in the driver's blind spots with the vehicle. The vehicle can then display this on a heads-up display for better perception. This can help in lane changing, overtaking, and pulling out of parking spots \etc. For accident warning, since \sysname tracks every vehicle's motion, it can warn it of potential accidents. In vehicles with on-board diagnostics ports (OBD) and the CAN bus~\cite{savage}, \sysname can also use emergency controls. To do this, after market devices that plug into the OBD can act as a relay between the edge and the vehicle's CAN bus. To avoid accidents, \sysname can send control signals for emergency braking or steering maneuvers to the vehicle's OBD  port.


==> design.tex <==
\section{\sysname Perception}
\label{sec:perception}

\ramesh{Let's have two separate sections, one for perception and one for planning. The architecture section will discuss these at a high-level, so it is probably OK to do that.}

\ramesh{In this section, we should have an overview subsection, followed by three subsections one each for the three main components that we discussed.}
\ramesh{Here is the grouping we discussed today for the three main components, together with suggested new terminology. Please leave comments if you think there is better terminology that we should adopt. (a) \textit{\textbf{View fusion}}, which consists of \textit{alignment} and \textit{stitching}, (b) \textit{\textbf{Participant extraction}}, which consists of \textit{background subtraction}, \textit{point clustering} and \textit{participant association} and (c) \textit{\textbf{Tracking}}, which consists of \textit{track association}, \textit{motion estimation}, \textit{heading estimation}. }

\subsection{Infrastructure-based Perception}

In this section, we detail one of the main contributions of \sysname: Infrastructure LiDAR-based \emph{real time} perception; this component is key to our proposed decoupling (\secref{sec:architecture}) of the state-of-the-art autonomous driving stack. We propose a novel perception algorithm that combines 3D point clouds from multiple geographically-distributed static LiDARs and processes a unified point cloud in real-time to enable fine-grain localization and tracking for autonomous driving. Note that \sysname does not plan the LiDAR placement; \sysname assumes that a deploying authority will use an intelligent topology planner to deploy a sufficient (say, $N$) number of LiDARs in a road intersection.

\ramesh{make sure to update \figref{fig:av_stack} with the components of the perception pipeline, or create a new figure.}

% \sysname relies on 3D sensors deployed on road-side infrastructure for perception. Each 3D sensor generates 3D frames at different frame rates per second. \sysname continuously merges point clouds from all these sensors into a single, stitched, real-time 3D point cloud. We call this component \textit{point-cloud stitching}. It is a part of the perception module, and it runs at the edge. The current autonomous driving pipeline does not contain such capabilities.
% Commented out by Christina

\ramesh{Create a new sub section. Call it design overview or \sysname overview. We have already talked about the architecture in the previous section.}
\parab{Overall Architecture.} 
Let us assume that a set of $N$ LiDARs are deployed in a designated intersection; each LiDAR generates a 3D point-cloud frame at a constant rate of $f$ frames per seconds (\ie 1 frame in every $T = 1/f$ seconds) and transfers it to the perception module of \sysname. In every $T$ seconds, \sysname's perception module processes the most recent set of $N$ frames (1 from each LiDAR) to detect any moving objects (\eg a car or a pedestrian) and to output the motion information of the detected objects; this is further fed to \sysname's planner module (\figref{fig:sys_overtaking}) to generate desired path trajectories for autonomous vehicles. To estimate accurate motion information in real-time, \sysname executes a one-time initialization step\footnote{We may need to re-invoke the initialization step if there is a dramatic change in the surroundings such as the spawning of a new building.} followed by a set of five sequential steps in every sensing period ($T$) as follows.
% \pradipta{The Initialization is run once at the beginning right? Or Do you run it again after some time?}
% \christina{We can run it again to detect some dynamics in roads, if necessary. However, for now, we just can say it runs once at the beginning.}

\ramesh{What do you have below is a great start! However, the overview section needs to be short and crisp. First, instead of having six different components, which is hard for a reader to keep in mind, can we describe the system as having three top level components, each of which we have two or more sub components? What would those be?}
\ramesh{Second, for each sub component start with the "what" (see detailed comments below), and have a brief sentence that describes the "how" and how the "how" is a novel contribution.}
\ramesh{For example, this is how I would describe the initialization component in an overview section. I would pick a better name, such as \textit{calibration} or even \textit{alignment}. (It is not clear that the step needs to be done only once. It may need to be done for example if the Lidar has moved for any reason). Then, the text would be something like: The position of a point in a LiDAR's point cloud is described in that LiDAR's frame of reference. In order to detect objects from multiple LiDARs, \sysname needs to ensure that all LiDAR point clouds are positioned within a common coordinate frame of reference. The alignment step, performed once initially and again whenever a LiDAR is reconfigured, adapts prior work on point cloud registration to be robust to settings, such as ours, when the point clouds are captured from vastly different perspectives.}
\ramesh{Also, if we are claiming alignment to be a contribution, let's find a name to describe it.}

\parag{Initialization.} To efficiently detect the dynamic objects and extract the respective motion information, \sysname needs two basic information: (1) Pair-wise transformation matrices between LiDARs and (2) a background point cloud. In addition, \sysname needs to detect drivable Space to plan the autonomous vehicle trajectories. 

We need the pair-wise transformation matrix to fuse the 3D sensory data from multiple LiDARs into a unified point cloud. Each LiDAR point cloud is represented by its own (and independent) frame of reference (or coordinate system). To combine two LiDAR point clouds, we apply coordinate transformation from one's point cloud to the other; a pairwise transformation matrix is a key to this. Estimation of the transformation matrices takes several minutes and can be done offline as the LiDARs are static. To this, \sysname completes a \emph{Point Cloud Alignment} process as a part of the initialization (detailed below).

A \textit{background point cloud} is a point cloud frame that represents the static background of a sensed region (such as roads, buildings, and traffic signs). \sysname compares a point cloud frame with a background point cloud to identify dynamics objects (such as cars and humans). In a real-world setting, it is challenging to find an empty scene without any dynamic objects to generate a background point cloud. A trivial approach can take an intersection of multiple consecutive frames; however, this may include temporary static objects such as a parked vehicle. 
To this, we take an intersection of $P$ temporally isolated frames to completely filter out dynamic points and form a \emph{common frame}.  A single common frame is, yet, not a robust representation of the background point cloud; it might be missing a significant subset of background static points~\cite{kashani2015review} due to either temporary obstructions or LiDAR hardware issues. To solve this practical problem, we generate $Q$ temporally distributed common frames and aggregate them to form the final background point cloud. 
The background point cloud construction takes a significant amount of time and only needs to be updated after a dramatic change in the surroundings such as the spawning of a new building. Therefore, \sysname performs the \textit{Background Point Cloud Construction} as a part of the initialization.
% \pradipta{I am actually more confused now. You say that P frames should not be consecutive. But then what the reason behind first combing P
\pradipta{What are the typical values of P and Q?}
\pradipta{minor comment: can we come up with a meaningful name instead of "common frame"?}
% \pradipta{Please check. Also, Can you write 1-2 sentences on how does the aggregation helps?}
% \christina{Actually, I was wrong for describing how we get the background construction, so revised the writing. Please check and let me know when it confuses you.}
\ramesh{I noticed that we discuss point cloud alignment in more detail in a later section. Let's move the above paragraph to that section. The principle is that in this overview section, we should be discussing \textit{what} we do, not \textit{how} we do it}

Lastly, for the planner module to design trajectories, we need to inform the planner where vehicles can drive safely and legally.
\pradipta{Please write the drivable space extraction part here.}
\pradipta{Also, can we add an illustrative image for each of the steps?}
\christina{Yes, I think that is a good idea! I will make corresponding images and update the paper.}

% To extract the necessary motion information in real-time, \sysname performs an initialization (or pre-processing) step to perform three time-consuming (takes several minutes) and resource-heavy operations: (1) \textit{Point Cloud Alignment}, (2) \textit{Background Point Cloud Construction} and (3) \textit{Drivable Space Extraction}. The \emph{Point Cloud Alignment} process extracts pair-wise transformation matrix between the LiDARs; this is a key information required to fuse the 3D sensory data from multiple LiDAR into an unified point cloud. We propose a novel algorithm to extract the pairwise transformation matrices (detailed below). \sysname also needs to construct one frame of point cloud that only contains background points from Background Point Cloud Construction. The background point cloud will be used to filter out the background from each collected data. In real-world, however, it is not always easy to collect a point cloud from an empty scene without any vehicle. Thus, we spend some time constructing a robust background point cloud. Given an integer $i$ and $j$, we pick $i \times $j number of random frames such that there are $i$ number of sets of point clouds and each set has $j$ number of consecutive point clouds. Then, we extract common points in each set and merged these $i$ number of intersectioned point clouds into one frame of background point cloud. In this way, we can construct a robust background even under a dynamic situation. For the planner module to design trajectories, we need to let the planner know where vehicles can drive safely and legally.

\parag{Stitching.} After proper initialization, the first step of \sysname's perception module is to stitch the most-recent $N$
\ramesh{Shouldn't this be: the most recent frame from each of the $N$ different LiDARs?} frames from different LiDARs into one unified frame; we call this a \textit{stitched point cloud frame}. Each LiDAR's 3D frame is presented in its coordinate systems. \sysname applies a linear coordinate transformation to each frame with the respective transformation matrix (obtained from \textit{Point Cloud Alignment}) to aggregate them into the stitched point cloud frame. The stitched point cloud presents a full view of the scene; it aggregates information about everything detected by the LiDARs such as ground planes, buildings, and vehicles. We further detail the stitching process below.

\ramesh{Rewrite the previous paragraph to describe the what before the how. The last sentence gets close to the how.} 
\ramesh{Also, as you write, keep in mind that the why is also an important consideration. We should discuss why we do stitching, and what other options are possible. The Overview may not be the best place to do this, it might be better to describe the why closer to the how.}



\parag{Background filtering.} In the second step, \sysname's perception module filters out all points residing in the background and extracts only dynamics object (in our case mainly vehicles) by simply removing the overlapping points between the stitched point cloud and the background point cloud (obtained from the \textit{Background Cloud Construction}). This is sufficient in our setting as the LiDARs are fixed and the background points are mostly static; this is quite different from traditional autonomous vehicle systems with moving LiDARs.
% \pradipta{Do we assume that there is no other dynamic object other than vehicles?}
% \christina{There can be other objects. However, we haven't designed yet how to cope with them.}

\parag{Clustering.} After background filtering, the stitched point cloud only contains dynamic objects. Assuming there exists no dynamic object other than vehicles, \sysname's perception module performs a \textit{Density-based Spatial Clustering with Noise} (DBSCAN)~\cite{ester1996density} to extract multiple clusters where each cluster corresponds to a vehicle.
% \christina{Added a citation.}

\parag{Tracking/Association.} Following the clustering step, \sysname examines the clusters to associate vehicle identities; this is required to persistently track the same vehicles in-between frames. We propose a Kalman filtering~\cite{kalman1960new} based method to find the correct correspondences between the current set of detected vehicles and the vehicles detected in earlier frames and to perform a consistent tracking of individual vehicles. The tracking algorithm also outputs the location of a consistent reference point for each vehicle. This is further detailed later on.
% \christina{Added a citation.}

% \parag{Motion estimation.} In the last step, \sysname's perception module estimates the location and movement state of each vehicle. To this, \sysname estimates four different parameters to completely represent a vehicle's motion: (1) the location of a reference point of the vehicle, (2) the oriented bounding box of the vehicle, (3) the instant heading direction, and (4) the motion vector over a time window. The location of a reference point and the bounding box summarize the dimensions of a vehicle and the location (position and orientation) in the stitched 3D frame. In addition to the localization information, we need the heading direction and the motion vector to characterize the motion of each vehicle in the current stitched 3D frame. We use the term, \textit{heading direction}, to infer an instantaneous heading direction at the time. On the other hand, a \textit{motion vector} embodies the velocity and the heading direction of a vehicle averaged over a short period of time. How \sysname estimates these parameters is further explained in details below.

\parag{Motion estimation.} In the last step, \sysname's perception module estimates the movement state of each vehicle. With the estimated location of a reference point of the vehicle (obtained from \textit{Tracking/Association}), \sysname estimates three different parameters to completely represent a vehicle's motion: (1) the oriented bounding box of the vehicle, (2) the instant heading direction, and (3) the motion vector over a time window. The location of a reference point and the bounding box summarize the dimensions of a vehicle and the location (position and orientation) in the stitched 3D frame. In addition to the localization information, we need the heading direction and the motion vector to characterize the motion of each vehicle in the current stitched 3D frame. We use the term, \textit{heading direction}, to infer an instantaneous heading direction at the time. On the other hand, a \textit{motion vector} embodies the velocity and the heading direction of a vehicle averaged over a short period of time. How \sysname estimates these parameters is further explained in details below.
% \christina{Revised it to remove location estimation in this phase.}

\parab{Point Cloud Alignment.}
As briefly described earlier, \sysname's perception module performs a \textit{point cloud alignment} (also referred to as \textit{point cloud registration}) in the initialization step to estimate the pairwise transformation matrices between the LiDARs; this is further used to combine the 3D point clouds from multiple LiDARs to generate a real-time stitched 3D view. 

The most popular method for point cloud registration is an iterative algorithm called the Iterative Closest Point(ICP)~\cite{bellekens2015benchmark}. In each iteration, ICP minimizes a cost function that represents an estimate of point correspondences between the point clouds. The input to the ICP is an initial guess of the positions and the orientations (roll, pitch, and yaw) of the LiDARs; the output is a set of transformation matrices to register two point clouds. 

To apply ICP in \sysname, we need reasonable estimations of each LiDAR's orientation and position. If a deploying authority can provide \sysname with good estimates for both orientation and position, \sysname directly feeds it to ICP to get the desired transformation matrices. If no such information is available, one can easily obtain a rough location estimate by physical examination; it is, however, challenging to do the same for the orientation information. 


\weiwu{Prior: point clouds are closed to each other}
One of the challenges in getting the correct orientation information is the lack of mapping information between a LiDAR's local coordinate system and the geoidal coordinate system; \eg one LiDAR's yaw of 0 degrees might point to the geoidal North direction while another's yaw of 0 degrees might point to the East. Taking such corner cases into account, we propose a modified point cloud alignment algorithm (\algoref{algo:icp}) that robustly estimates each point cloud's transformation matrix (orientation and position) under the following set of realistic assumptions. 
\begin{itemize}
  \item Rough estimates of the LiDARs' deployed positions or the distance between LiDARs are available
  \item No information about the LiDARs' orientations is available. 
  \item There exists some overlapping sensing region among any two LiDAR sensors.
  \item The ground plane is visible in the LiDAR point clouds and is the largest plane in the scene.
\end{itemize}

\ramesh{the previous paragraph is good but super long. It contains three different ideas: what the problem is, how prior work has approached that problem, and what the downsides of the prior work are. This is a good template to use for all subsequent sections, but please break each of these into separate paragraphs. In general, if the paragraph is more than one fifth of a column, impatient readers may skip over the paragraph.}
\weiwu{addressed}

% As briefly described earlier, \sysname combines the 3D point clouds from different LiDARs and generates a real-time stitched 3D view; this process is also referred to as \textit{point cloud registration/stitching.} To do this, we need an accurate estimation of each LiDAR's orientation and position. However, LiDARs' exact positions and orientations might be unknown to \sysname, we design an point cloud alignment algorithm that robustly estimate each point cloud's transformation matrix(orientation and position). 
% \weiwu{I think we need to emphasize that knowing orientation or not is a big deal. Getting the orientation information will introduce lots of cost in installation. But without knowing that, the alignment problem is hard, and we figure out a way to deal with it. }

% Traditionally, Iterative Closest Point(ICP)\pradiptas{cite} is used to estimate the transformation matrices to register two point clouds. However, ICP requires an initial guess of both position and orientation. While we requires a rough estimate of the position as an input, the orientation is assumed to be unknown. If we have good estimates for both orientation and position, the problem will be solvable by applying ICP.

% \weiwu{I try to explain why the orientation information is important. It's hard to explain about the Yaw angle...}
% However, we cannot make much assumption of a LiDAR's orientation. Most importantly, we cannot assume a LiDAR is deployed horizontally to the ground plane, because a better coverage can require the LiDAR to be tilted in any angles(angle in pitch and roll). A less obvious but equally important orientation information is the angle in yaw. If one LiDAR's yaw's 0 degree points to North direction and another LiDAR's yaw's 0 degree points to East, given that we have good initial guess about position and rotation angle except the yaws, ICP will be hard to find a good alignment.

\noindent
The key idea of our approach is that we can estimate the LiDAR's orientation angles from each LiDAR's known position estimation. The insight is that we don't need a very accurate estimation as the initial guess that ICP can still find the correct alignment. The proposed point cloud alignment method(Algorithm \ref{algo:icp}), first, performs a ground plane segmentation in each point cloud frame(line 3) and aligns them to estimate each LiDAR's roll and pitch angles(line 4). This is followed by another alignment step based on the known position estimates(line 5). To estimate the yaw angle, \sysname performs a grid search over our defined error function(line 6).  Lastly, all estimates are fed to a standard point-to-plane ICP~\cite{bellekens2015benchmark} to output the transformation matrices(line 7).  

\ramesh{In this paragraph, start by describing the key idea behind our approach on a single sentence if possible. I presume it is that, because we may not have accurate estimate of the orientation, the Chi insight is that we can do a group search over different yaw angle. Also, as I recall, ICP is relatively insensitive to yaw angles, so you don't need to search across a large range?}
\ramesh{when you describe an algorithm, please make it a point to (a) reference the algorithm, and (b) reference each line of the algorithm In the sentences that describe that part.}
\weiwu{addressed, but not sure if I convey the insight accurately}

% \pradipta{I think we should add a short description of the steps here.}

\begin{algorithm}
\SetAlgoLined
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\SetKw{KwBy}{by}

\Input{A set of Point Clouds $C = \{c_1, c_2 ... c_n\}$ such that $c_i$ is from LiDAR $i$. \newline
A set of relative distance $D = \{d_2, ... d_n\}$ that $d_i$ is the estimated distance from LiDAR $i$ to LiDAR 1.
}
\Output{A set of transformations $T = \{T_2, T_3 ... T_n\}$ such that point cloud $C_i$ can use $T_i$ to register to $C_1$'s frame.}

Ground Plane Segmentation of $c_1$

\For{$i\gets1$ \KwTo $|T|$ \KwBy $1$}{
Ground Plane Segmentation of $c_i$

Ground Plane Alignment of $c_i$ and $c_1$

Position Alignment of $c_i$ and $c_1$ with the estimated distance $d_i$

Yaw Estimation of $c_i$.

Iterative Closest Point with the previous alignment as the initial guess
}
\caption{Robust Point Clouds Alignment}
\label{algo:icp}
\end{algorithm}

\parag{Ground Plane segmentation and Ground Plane Alignment}. \sysname uses the RANSAC algorithm~\cite{derpanis2010overview} to find all the planes in the point clouds and selects largest plane as the ground plane (based on our assumptions stated above); this process also outputs the equations of the ground plane in each LiDAR's coordinate system. \sysname utilizes these equations to calculate the distance between the respective LiDAR and the ground plane. Since we assume that ground planes are visible in all LiDAR point clouds, we can partly align the point clouds by aligning their respective ground planes. After this step, point clouds from all LiDARs will have their ground plane aligned, and the Z-axis of each point cloud's coordinate system will be perpendicular to their ground plane. With the distance between each LiDAR to its ground plane, we can learn the value of the $z_i$ coordinate of each LiDAR in this partially aligned coordinate system.
% \sysname performs a ground plane alignment to exploit the information from the ground plane segmentation to transform the point cloud such that the Z-axis of the point cloud is perpendicular to the ground plane.
% \pradipta{what is "untilt"? is it a known term?}

\parag{Position Alignment}. $d_i$ is the estimated distance between LiDAR $i$ and LiDAR $1$. This value can be obtained by measuring distance using GPS, or Laser Rangefinder. Even though we are yet to find the correct alignment between the LiDAR's local coordinate system and the geoidal coordinate system, the relative distance between the LiDARs will be constant in either system. In this step, we put the point cloud from LiDAR $1$ at the $(0, 0, z_1)$ and the one from LiDAR $i$ at a position that is $d_i$ away from the origin. To ensure consistency, we pick $(d_i, 0, z_i)$.
% After ground plane segmentation and alignment, \sysname uses the information about the LiDAR positions to align point clouds such that the relative distance between two point cloud's coordinate system would be more or less accurate.
% \pradipta{I do not get this part.}

\parag{Yaw Estimation.} To estimate yaw, we leverage the following empirical observation: if the estimation of yaw angle is correct, the closest/corresponding points between two point clouds will be coplanar \ie they should have the same normal. To this, we define the following error function:  
\[
    Error(\omega, \omega') = \Sigma_{i=1}^{n} Normal(\mathbf{R}_{\omega} p_i) \cdot Normal(\mathbf{R}_{\omega'}  q_i)
    % \label{eqn:errorfn}
\]
% \pradipta{what is n here?}
where $p_i$ is a point in the source cloud, $q_i$ is $p_i$'s nearest neighbor in the target cloud and $n$ is the number of points in the source cloud. $\omega$ and $\omega'$ are the respective yaw angles for stitching and $\mathbf{R}_\omega$ is the rotational matrix for an yaw angle of $\omega$. The function $Normal$ will return the normal vector estimated at the given point.
With this error function, the estimation of the yaw angles can be formulation as the following optimization problem:
\begin{equation}
    Yaw_1, Yaw_2 = \argmin_{\omega,\omega'} Error(\omega, \omega')
\end{equation}
\sysname uses a grid search algorithm with a resolution of 18 degrees (\ie 20 grid points for each LiDAR)  to find the solution to this optimization problem. 
% \pradipta{Do you perform pari
% With a search space of 360 degrees for each LiDAR, the entire space of pairwise yaw estimation h has a searching space of 360 degree.

% The intuition behind the error function is that the closest/corresponding points between two clouds should have the same normal, or in another word, co-planar. The grid search has a resolution of 18 degree and each LiDAR has a searching space of 360 degree. This will make a 20x20 searching grid.

\parag{Final Estimations by ICP.} The estimated orientation information is fed to ICP along with the position information. With these as starting point, ICP performs more finer alignment to improve the quality of the stitched cloud.

% %% - Point-cloud stitching
% \fawad{Weiwu: please write down the details of the point cloud stitching algorithm here.}
% \sysname relies on 3D sensors deployed on road-side infrastructure for perception. Each 3D sensor generates 3D frames at different frame rates per second. \sysname continuously merges point clouds from all these sensors into a single, stitched, real-time 3D point cloud. We call this component \textit{point-cloud stitching}. It is a part of the perception module, and it runs at the edge. Current autonomous driving pipeline do not contain such capabilities.
% Commented out by Weiwu

% %% - Object detection and tracking
% \fawad{Christina: please write down all perception components here. Once you are done, please let me know}
% After generating the real-time stitched 3D map, the perception module uses it to understand condition of the road. In doing so, it segments the scene into static, and dynamic objects and then tracks the motion of the dynamic objects. One way of doing this is to segment the stitched point cloud. This component is also a part of the perception module. It runs at the edge, and we call it \textit{object detection and tracking}. Current autonomous driving pipelines contain similar components for tracking objects. However, they use monolithic (unstitched) point clouds from a single 3D sensor atop a vehicle rather than stitched point clouds.
% Commented out by Christina

\parab{Tracking.}
In this section, we detail our proposed vehicle tracking method based on infrastructure based LiDARs. After the object clustering step (see above), \sysname's perception module assigns an unique ID to each detected object in the scene. The main goal of this step is to identify inter-frame associations and detect same objects over the consecutive frames. Lack of semantic information poses an intrinsic challenge to multi-objects tracking in 3D point cloud as compared to 2D image data~\cite{vaquero2017deconvolutional}. Nonetheless, 3D data is often enriched with geometry information. Researchers often apply \textit{Kalman filtering}~\cite{kalman1960new} or \textit{Hungarian algorithm}~\cite{kuhn1955hungarian} on such geometric data for accurate and fast tracking~\cite{}; the performance of such methods are vulnerable to occluded objects or incomplete point clouds. Interestingly, \sysname do not suffer from such incomplete point cloud problem since we leverage stitched point clouds from multi-LiDARs that capture a more complete picture of the scene.
\christina{Note-to-myself: Need to add kf tracking citations}

\ramesh{please consider re-organizing the above paragraph according to the template discussed for alignment: A few sentences on the problem, A few on prior work, A few sentences describing why is the prior work falls short, and a few sentences that describe the key idea behind our approach.}
\ramesh{the last sentence is good, but we need to discuss how stitched point clouds help. Do they let us design a cheaper algorithm? Or do they give higher accuracy when we use an existing algorithm?}
\ramesh{To the algorithm description below, let's try to answer them contextual information: how similar or different is it from standard ways of doing tracking?}
\ramesh{Also, in the rewrite, we should explicitly mention clustering in this section, otherwise readers will not be able to match the description in the overview to the tracking section.}

% https://www.mathworks.com/help/fusion/ug/introduction-to-assignment-methods-in-tracking-systems.html
\sysname adopts Kalman filtering to track objects and assign corresponding IDs with a simple distance-based scheme. Based on previous history of identified objects, our algorithm applies Kalman filtering to first calculate the expected/estimated positions of the tracked vehicles (\ie vehicles identified in earlier frames). On the other end, \sysname observes a set of vehicles in the current point cloud frame and outputs their clusters. For the purpose of ID assignment, we represent each vehicle by the centroid of the object's cluster in the point cloud; we use these also as the \textit{reference points} for each tracked vehicles. Now, let us denote the estimated positions of $u$ tracked objects as $e_1, e_2, ..., e_u$ and the observed positions of $v$ objects as $o_1, o_2, ..., o_v$, respectively. Lastly, we introduce a distance matrix $D$ where $D_{ij}$ is the Euclidean distance between $e_i$ and $o_j$. With this, the tracking problem is converted into a matching like problem; we use distance metrics to match the estimated locations with the observed locations. Our algorithm finds an assignments $A = \{a_{ij}\}$ that minimizes the summation of distance of assignments as follows:

% \begin{flalign*}
% &\textrm{Minimize}  \hspace{10mm} \sum_{i=0}^{n}\sum_{j=1}^{m}D_{ij}a_{ij} && \\
% &\textrm{Subject to} \hspace{10mm} \sum_{i=0}^{m}a_{ij} = 0, \forall j &&\\
% & \hspace{23mm} \sum_{j=0}^{n}a_{ij} = 0, \forall i &&
% \end{flalign*}

\begin{flalign*}
&\textrm{Minimize}  \hspace{10mm} \sum_{i=1}^{u}\sum_{j=1}^{v}D_{ij}a_{ij} && \\
&\textrm{Subject to} \hspace{10mm} \sum_{i=0}^{u}a_{ij} = 1, \forall j \in \{1, \cdots, v\} &&\\
& \hspace{23mm} \sum_{j=0}^{v}a_{ij} = 1, \forall i \in \{1, \cdots, u\}  &&
\end{flalign*}
\pradipta{The equations did not seem right. I modified it based on my understanding. Please check.}
\pradipta{The cost function seems bit weird to me. This will force to minimize the sum of distance. Then the solution will be all $a_{i0} = 1$ and $a_{0j} = 1$. To circumvent this, typically a large cost is added for the 0 assignment case. But even then the problem will be it will always try to assign a matching even though there is no correlation. I guess the best cost function would be to use $D_{i0}$ and $D_{0,1}$ to be a threshold distance for matching. Maybe you are already doing that. But please check.}
\christina{Yes, I get your point. Our current implementation is using the distance threshold (5m) for the matching so maybe we need to add what you suggested? Also, other than that, I was wrong on the equation and the changed one makes sense!}
\pradipta{I see. In that case, please update the equation and the description.}
Here, $a_{ij} = 1$ implies estimated object $e_i$ is matched to observed object $o_j$. If an estimated object $e_i$ is not matched with any observed object, $a_{i0} = 1$. Similarly, if $o_j$ is not matched with any estimations, then $a_{0j} = 1$. The optimization function makes sure that the closest pair is matched together while the constraints ensures each estimation is associated with no more than one observation, vice versa.

After solving this optimization, we should have correct ID assignment to each vehicles. We feed the output \ie a list of tracked object ID with their respective reference points ($o_j$) to the motion estimation and planning module.

% Our algorithm set a position of objects to a centroid of the object's point cloud. The main idea to do association between these estimations and observations is to assign a nearest observation to an identified estimation. We introduce estimation positions as $e_1, e_2, ..., e_n$ , observed positions as $o_1, o_2, ..., o_m$, and a distance matrix $D_{ij}$ where $D_{ij}$ is an euclidean distance between $e_i$ and $o_j$.

% As mentioned above, detected objects are almost free from the occlusion problem because \sysname utilizes stitched point clouds from multi-LiDARs. Thus, this proposed distance-based scheme is simple yet effective.

\parab{Cyber-physical association.}
In order to close the sensing-perception-control loop, we need to know the association between the entities tracked in our system and the vehicles in the physical world. To learn the association, we need to know the positions in both the perception system and the physical world. For positions in the physical world, vehicles can equip GPS\cite{} or GNSS\cite{} to track their positions(longitude and latitude) in the geographical coordinate system. As mentioned previously, \sysname detects and tracks the positions of all the vehicle instances in the scene. Because \sysname knows the mounting position of the LiDARs through GPS, we can convert  

\parab{Motion Estimation.}
% The last step of our perception module is \textit{motion estimation}. The motion estimation procedure estimates the four different components of the current motion state (detailed above) of the detected objects: (1) the location of a reference point of the vehicle, (2) the oriented bounding box of the vehicle, (3) the instant heading direction, and (4) the motion vector over a time window.
The last step of our perception module is \textit{motion estimation}. The motion estimation procedure estimates the three different components of the current motion state (detailed above) of the detected objects: (1) the oriented bounding box of the vehicle, (2) the instant heading direction, and (3) the motion vector over a time window. This data is directly fed to \sysname's planning module and used to generate trajectory plans for each vehicle. The collected LiDAR data is very time-sensitive with regards to trajectory (path) planning; our proposed algorithm, therefore, aims to complete the motion estimation in real-time while maximizing the accuracy.
% \pradipta{Is the location estimated part of the motion estimation? From reading it seems to be part of the tracking/association phase. Please correct me if I am wrong. If I am right, we should remove it here. Other wise we should add a para or line about it here.}
% \christina{Yes, it is obtained from tracking/association. I removed it.}

\ramesh{As with other sections, this is a very nice start. Please follow the comments I have given in the other sections to re-write the section. In particular, for this audience we need to help them understand what is novel relative to prior work, and what kinds of trade-offs we have made.}

% The perception module in \sysname outputs a reference point, a bounding box, heading direction, and motion vectors for each vehicle. By referring the position and the bounding box, the planning module gets a rough size of the vehicle and localizes it at the same time. Other than localization, motion information is acquired from heading direction and motion vector. In this paper, we use the term, \textit{heading direction}, to infer an instantaneous heading direction at the time. On the other hand, \textit{motion vector} means a continuous heading direction and velocity over the time. Both information are complimentary, and will give us more understanding of the scene.

% http://codextechnicanum.blogspot.com/2015/04/find-minimum-oriented-bounding-box-of.html
\parag{Bounding box estimation.} Our motion estimation starts with bounding box estimation. As implemented in \cite{pclbbox}, a minimum oriented bounding box of a given vehicle is extracted by using eigenvectors and covariance matrix of the point cloud. Based on the extracted bounding box, our algorithm estimates three surface normals (i.e., front direction, side direction, and upper direction) of the bounding box; these are fed to the next step to select the correct normal vectors as a heading direction of the vehicle.

\parag{Heading direction estimation.} After the bounding box estimation, our algorithm selects one of three surface normals estimated in the bounding box estimation step to represent the heading direction of each vehicle. To filter out the heading direction of the vehicle at time $t$, our algorithm fetches a point cloud of the vehicle at time $t-1$ and compares it with the point cloud at $t$; this gives us a vehicle's moving direction from time $t-1$ to $t$. To this, we simply calculate the vector ($\overrightarrow{dv}_t$) between the vehicle's reference points (centroid) at time $t$  and at time $t-1$: $\overrightarrow{dv}_t = \overrightarrow{c_t} - \overrightarrow{c_{t-1}}$, where $\overrightarrow{c_t}$ and $\overrightarrow{c_{t-1}}$ are the 3D position vectors for the vehicle centroid at time $t$ and $t-1$, respectively. Next, we compare the direction of $\overrightarrow{dv}_t$ with the three surface normals of the vehicle and select the one with the most similarity with $\overrightarrow{dv}_t$. This method works under the assumption that the vehicle's moving direction from $t-1$ to $t$ is not much different from the vehicle's instant heading direction at $t$.

To get an accurate $\overrightarrow{dv}_t$, we first run ICP algorithm to align the point cloud of the vehicle at time $t-1$ with the point cloud of the vehicle at time $t$. Next, we use the original point cloud at $t-1$ and the aligned point cloud to robustly calculate $\overrightarrow{dv}_t$.
\pradipta{From the meeting, if I remember correctly, the point cloud here is only for the vehicle; not the entire frame. Right? If so, we need to make it clear.}
\christina{Yes. I simply changed to "point cloud of the vehicle". Do we need more explanation?}
\pradipta{Should be fine I guess. But there is a slight disconnect in the write up then bcoz all of a sudden you are talking about vehicle point cloud instead of the whole point cloud. Ramesh will have better idea about this.}
% It is important to get an accurate $dv_t$ between two given point clouds. Thus, we run ICP algorithm to align those two point clouds. By running ICP, we first obtain a transformation matrix from point cloud at $t-1$ to $t$. Then, we transform the point cloud at $t-1$ under the obtained transformation matrix. Lastly, we gain $dv_t$ between the point clout at $t-1$ and transformed point cloud. Because we calculates $dv_t$ from two aligned centroid points, more robust estimation can be achieved.

\parag{Motion vector estimation.} For the last step in our motion estimation, our algorithm tracks a motion vector. We can decompose the motion vector into two sub-components; direction and magnitude of the vector. Direction of the motion vector indicates an averaged heading direction over a given time window, $w$, and we interpret it to a heading trend within the time window \pradiptas{What do you mean here?}. Magnitude of the vector is nothing but the average speed over the time window $w$. Our algorithm estimates the direction of the motion vector by simply averaging the estimated heading direction over $w$. To get the magnitude of the motion vector, our algorithm fetches another point cloud of the vehicle which is $w$ frames ahead and runs ICP to align them. Similar to the heading vector estimation above, we calculate a displacement vector $\overrightarrow{dv}_t$ for the vehicle from time $t-w$ to time $t$ and set $|\overrightarrow{dv}_t|$ as the magnitude of the motion vector.
\christina{I mean the direction of the vector is somehow averaged heading direction. Can you help to make it more clear?}
\pradipta{But I thought the displacement vector direction is the motion vector direction. Is it not? How are you averaging the direction otherwise?}
We notice that our proposed motion estimation is vulnerable to noisy data from sensor faults and such noisy data is quite common in real-world data collection. To filter out such noises, we adopt Kalman filtering. \sysname maintains a separate Kalman filter model for each detected vehicle. Instead of outputting the instantaneous motion vector, our algorithm feeds the newly estimated motion vector to the Kalman filter and outputs a less noisy motion vector.

% \ramesh{Point out that this is one way of doing it. The point about how current autonomous driving has the same components is good.}
% \fawad{Addressed.}


==> design_controller.tex <==
\section{\sysname Planning}
\label{s:planner}

\fawad{I think I'll add a diagram here to show how different sub-modules work in the controller.}
\sysname's controller module uses positions, bounding boxes and motion vectors along with a drivable space map from the perception module to control \sysname-compatible vehicles. The control module consists of the three sub-modules \ie the centralized planner at the edge for motion-planning, and the local low-level controller along with a PID controller at the vehicle which convert those paths to low-level vehicle controls (\eg steering wheel angle, throttle, and brake).


\parab{Goals and Requirements. } The controller must ensure collision-free driving for all \sysname-compatible vehicles with low latency in all deployment scenarios (\secref{sec:deployment}). The controller must support user-imposed traffic policies \eg prioritizing emergency vehicles, reducing traffic congestion \etc.

\ramesh{the second sentence is good, but comes out of the blue. We might want to figure out whether we want to justify this requirement either here or earlier in the introduction or the arch section.}

\parab{Control for Autonomous Driving Today. } Autonomous vehicles today use on-board planning and control modules to plan motion and follow collision-free paths to reach their destinations. Since every vehicle plans for itself, work in industry and academia has focused on decentralized motion planning algorithms ($A^{*}$~\cite{Astar}, Safe Interval Path Planning (SIPP)~\cite{SIPP}, and Dijkstra~\cite{Dijkstra}). Centralized algorithms (\eg Conflict Based Search (CBS)~\cite{CBS}) for multi-robot/agent planning exist but, in practice, they have been used in more controlled environments like warehouses and are known to have large tail latencies~\cite{cbslatency, SIPP}. To this end, \sysname uses a decentralized low-latency algorithm, SIPP, in a centralized manner for motion planning.

\ramesh{we might want to add a citation for the tail latencies.}
\fawad{Addressed.}

% \textit{Challenges. }
\parab{SIPP. }
Planning in static environments is a well-studied problem that can be solved efficiently. Planning algorithms discretize space into a 2D occupancy grid and plan a path for a given robot from a one location (source) to another (destination). Planning in dynamic environments adds an extra dimension \ie time, to the search space and this increases computational complexity. SIPP is a graph-search algorithm for dynamic environments that is based on the following intuition. Although the \textit{time steps} ($t_{1}, t_{2}, ...., t_{n}$) that a given location in the occupancy grid is safe for robot occupation is unbounded and infinitely large; the number of \textit{time intervals} ($[t_{1}, t_{n}]$) at which that location is safe is bounded and generally small. A safe \textit{time interval} ($[t_{1}, t_{n}]$) in one in which the location is safe for occupation throughout the interval, but not safe one step before ($t_{0}$) and one step after ($t_{n+1}$) the interval. To scale, for every location in the 2D occupancy grid, SIPP discretizes time into contiguous safe and unsafe \textit{time intervals} or states. Squares with static obstacles \eg the sidewalk are unsafe eternally whereas others like the road have multiple safe and unsafe states. This allows SIPP to compactly represent each location with a few states. With this representation, SIPP solves the graph-search problem using $A^{*}$ search.

\ramesh{the above description is good, but you might want to add more academic language: to scale, SIPP discretizes space and time etc. Give the intuition behind what enables it to scale, and then describe how the algorithm works.}
\fawad{Addressed.}

\parab{Centralized Planning with SIPP. }
\sysname uses SIPP in a greedy, sequential manner for centralized control. Consider the full-deployment scenario (\secref{sec:deployment}). In this, \sysname first plans for a single vehicle with SIPP using only the static environment. Then, it uses the SIPP-generated path for first vehicle as a dynamic obstacle for the second vehicle. This way, the second vehicle can avoid static obstacles and the first vehicle. The third vehicle uses both the first and second vehicles as dynamic obstacles and so on. This way, \sysname can plan for all vehicles in a centralized manner using sequential SIPP.

\sysname uses a greedy approach for planning as opposed to an optimal approach like CBS for two reasons: a) latency, and b) flexibility. Optimal approaches tradeoff planning time (latency) to ensure robots reach their destinations in the minimum amount of time. In our case, a lower planning time (to meet the 100~ms latency budget), guaranteed by a greedy approach, is more important. Second, an optimal approach achieves a single goal \ie minimum overall trip time. With a greedy approach, \sysname creates opportunities support different types of user-defined traffic policies. For instance, besides minimizing trip times, it can prioritize emergency vehicles, ensure fair waiting times for all vehicles, ameliorate traffic congestion on a given road \etc.
% \sysname uses a greedy approach as opposed to a more optimal approach like CBS for the following reasons. Optimal approaches tradeoff have higher planning times to ensure all robots reach their destinations in the minimum amount of time. In our  case of autonomous driving, a lower planning time (to meet the 100~ms latency budget) is more important than time to plan is more important    is more important than First, although, the greedy approach does not guarantee an optimal solution, it  the greedy approach ensures that we reach a solution faster. Optimal  Instead of a greedy approach, we could have used an We could have used a more optimal approach for planning (\eg Conflict Based Search) We use a greedy approach in \sysname (as opposed to an optimal approach like CBS)  
% 1. For latency
    % CBS run times are higher so we can only use it once. It will have to be updated and run every step which makes it very expensive
    % Even if the environment changes, we can run SIPP over and over again because it has a lower cost
% 2. For user defined traffic policies
%   
% As opposed to a greedy approach, \sysname could have used an optimal algorithm like Conflict Based Search. 

% A centralized controller, as opposed to decentralized controllers today, creates opportunities for cross-car optimizations and impose user-defined traffic policies (as we show later).

\ramesh{similar comment here. First say that we run SIPP in a greedy manner, planning for each vehicle in turn, while treating previously planned vehicles as obstacles. When you say this, people will expect a discussion of why you chose greedy: fast versus non-optimal.}
\fawad{Addressed but still thinking about how to improve it}

\parab{Challenges. }
SIPP solves a graph-search problem to plan a path for a vehicle from source to destination without any regard to real-world vehicle physics and traffic regulations. In doing so, it makes assumptions that do not hold true in the real-world. For instance it assumes that: a) vehicles can stop/start moving instantly, b) vehicles move with uniform speed, c) vehicles can move in all directions, d) vehicles occupy a single square on the occupancy grid, and e) the controller knows the location of every dynamic obstacle on the occupancy grid. To use SIPP in a realistic scenario, \sysname must relax these assumptions. 

Secondly, though SIPP is faster than other centralized algorithms, it takes upto 1~second to complete a single planning cycle. Moreover, this time increases with the number of vehicles that it must plan for. \sysname must enable SIPP to scale to a large number of vehicles and reduce the time for a single planning cycle.

\parab{\sysname's Approach. }
% Three contributions
% Splitting functionality / parallelism
To add support for real-world dynamics, \sysname must balance two competing constraints. \sysname's controller needs additional functionality to understands real-world dynamics. However, this functionality increases computational complexity and increases latency. To achieve both goals, \sysname divides the control module into two sub-modules and distributes the additional functionality between them. This includes a centralized planner resides at the edge and a low-level controller on-board every vehicle. The centralized planner runs the SIPP planning for all vehicles. It then sends a set of waypoints to the on-board low-level control module which converts them to the steer angle, throttle and brake. 

% Real-world dynamics
An out-of-the-box SIPP algorithm only uses robot positions as inputs for planning. To add support for real-world scenarios, \sysname's centralized planner makes use of the motion vectors and bounding boxes of vehicles from the perception component. The centralized planner uses motion vectors to model motion and the bounding boxes to model the realistic size of every vehicle in SIPP. Similarly, the low-level control module, converts the output (designed for a robot that can start/stop instantly) from the planner to a realistic path that vehicle can follow. To do this, it uses the set of waypoints and vehicle dynamics (\eg braking force and acceleration).

% Latency requirement
Lastly, \sysname makes optimizations to SIPP that enable it to run a planning cycle within 10~ms for low-latency planning. This way \sysname can run the centralized planner at LiDAR frame rate. As we discuss later, this makes \sysname more robust to unexpected changes in the environment (\eg unexpected driver, pedestrian or cyclist behavior).

% these waypoints to  Then, it sends    Then, it adds functionality to \sysname adds functionality to the controller that enable it to understand real-world dynamics. It splits this into two sub-modules: a) a centralized planner, and b) a local low-level control module. 

% First, \sysname uses SIPP planning at LiDAR frame rate instead of single-shot planning. Second, \sysname adds functionality to the controller that enable it to understand real-world dynamics of vehicles and road regulations. It splits this functionality between the edge (centralized controller) and the vehicle (local planner).

\ramesh{The LIDAR and single shot planning comes out of the blue; there is nothing in the prior text that prepares the reader for this. At this point, the reader is expecting some description of how you relax the assumptions. Also, it is unclear what problem functionality splitting solves.}
\fawad{I changed the entire approach because I missed out on many points. Please check it now}
% in SIPP to help it understand the real-world dynamics of a vehicle \eg its size and momentum. Last, \sysnam 
% whereas dynamic object   
% are used, \sysname controls multiple     a planning module along with a control module to control the motion of the vehicle. The planning module performs two functions: a) it plans a collision-free path for a vehicle from source to destination (path-planning) and b) it plans the motion of the vehicle to follow that path (motion-planning). The control module converts that motion to low-level control signals that the vehicle can understand. 

\begin{algorithm}[t]
  \caption{Centralized Planner}
  \label{algo:controller}
\SetKwFunction{CalculateDrivableSpace}{CalculateDrivableSpace}
\SetKwFunction{QueryPerception}{QueryPerception}
\SetKwFunction{MotionEstimation}{MotionEstimation}
\SetKwFunction{MotionAdaptiveBuffer}{MotionAdaptiveBuffer}
\SetKwFunction{AddDynamicObstacles}{AddDynamicObstacles}
\SetKwFunction{SippPlanning}{SippPlanning}
\SetKwFunction{RecoveryMode}{RecoveryMode}
\SetKwFunction{AddStaticObstacles}{AddStaticObstacles}
\SetKwFunction{GenerateIntervals}{GenerateIntervals}
\SetKwFunction{PriorityFunction}{PriorityFunction}
\SetKwFunction{Append}{Append}
\SetKwFunction{SendOverNetwork}{SendOverNetwork}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{\sysname-compatible objects $V_{C}$ \\ Non-compatible objects $V_{E}$ \\ Stitched point cloud $S$}
% ${Vehicle poses $P$, bounding boxes $B$, motion vectors $M$ and stitched point cloud $S$} % P for the set of point clouds and G for the set of gps tags
\Output{Vehicle trajectories $W$ for $V_{C}$}
\BlankLine
$P_{C}, M_{C}, B_{C} \leftarrow $ \QueryPerception ( $V_{C}$ ) \\ % Query perception for ego-vehicles
$P_{E}, M_{E}, B_{E} \leftarrow $ \QueryPerception ( $V_{E}$ ) \\ % Query perception for non-ego vehicles
$S_{D} \leftarrow $ \CalculateDrivableSpace {$S$} \\
$C. $ \AddStaticObstacles { $S_{D}$ } \\
% \ForEach { $v_{i}$ in $V_{E}$, $p_{i}$ in $P_{E}$, $m_{i}$ in $M_{E}$, $b_{i}$ in $B_{E}$ }
\ForEach { $v_{i}$ in $V_{E}$ } %, $p_{i}$ in $P_{E}$, $m_{i}$ in $M_{E}$, $b_{i}$ in $B_{E}$ }
{
    $t_{i} \leftarrow$ \MotionEstimation { $p_{i}$, $m_{i}$ } \\
    $d_{i} \leftarrow$ \MotionAdaptiveBuffer { $t_{i}$, $b_{i}$, $m_{i}$ } \\
    $C. $\AddDynamicObstacles { $d_{i}$ } \\
}
% $C. $\GenerateIntervals { } \\
$V^{'}_{C} \leftarrow $ \PriorityFunction { $V_{C}$ }\\
\ForEach { $v_{i}$ in $V^{'}_{C}$ } %, $p_{i}$ in $P_{E}$, $m_{i}$ in $M_{E}$, $b_{i}$ in $B_{E}$ }
{
    $w_{i} \leftarrow$ $C .$\SippPlanning { $p_{i}$, $g_{i}$ } \\
    % $W .$\Append{ $w_{i}$ } \\
    \SendOverNetwork { $v_{i}$ , $w_{i}$ } \\
    $d_{i} \leftarrow$ $C .$\MotionAdaptiveBuffer { $w_{i}$ } \\
    $C. $\AddDynamicObstacles { $d_{i}$ } \\
    % $d_{i} \leftarrow$ \MotionAdaptiveBuffer { $t_{i}$, $b_{i}$, $m_{i}$ } \\
    % $C. $\LoadDynamicObstacle { $d_{i}$ } \\
}
\end{algorithm}

\begin{algorithm}[t]
  \caption{Local Controller}
  \label{algo:planner}
\SetKwFunction{ReceiveTrajectory}{ReceiveTrajectory}
\SetKwFunction{ValidControlCycle}{ValidControlCycle}
\SetKwFunction{ValidTrajectory}{ValidTrajectory}
\SetKwFunction{RecoveryMode}{RecoveryMode}
\SetKwFunction{HasWaitCycle}{HasWaitCycle}
\SetKwFunction{GetWaitPoint}{GetWaitPoint}
\SetKwFunction{GetBrakingDistance}{GetBrakingDistance}
\SetKwFunction{ApplyBrake}{ApplyBrake}
\SetKwFunction{MoveToWaypoint}{MoveToWaypoint}
\SetKwFunction{SelectWaypoint}{SelectWaypoint}
\SetKwFunction{ApplyControl}{ApplyControl}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{Centralized planned trajectory $t$}
\Output{Low-level control signal $S$}
\BlankLine
$w \leftarrow$ \ReceiveTrajectory { } \\
\If  { $!$ \ValidControlCycle {$w$}  }
     {
        $w \leftarrow$ \RecoveryMode { } \\
     }
    
\eIf { \HasWaitCycle {$w$} }
     {
        $d_{s}, p_{s} \leftarrow$ \GetWaitPoint { $w$ } \\
        $d_{b} \leftarrow$ \GetBrakingDistance { $v$ } \\
        \eIf { $d_{b}$ $\leq$ $d_{s}$  }
        {
            $S \leftarrow$ \ApplyBrake { } \\
        }
        {
            $S \leftarrow$ \MoveToWaypoint { $p_{s}$ } \\
        }
     }
     {
        $p \leftarrow$ \SelectWaypoint { $w$ } \\
        $S \leftarrow$ \MoveToWaypoint { $p$ } \\
     }
\ApplyControl {$S$} \\
\end{algorithm}

\subsection{Centralized Planner}
The centralized planner, which resides at the edge, takes perception data and uses it to plan paths for all \sysname-compatible vehicles. It then sends these paths to all vehicles over the network. The planner generates paths for every vehicle at 10~Hz. The local low-level controllers on-board every vehicle convert these path to control signals (steer, throttle, and brake) that the vehicle can understand.

% \sysname uses the real-time scene understanding from the perception module to plan safe and efficient paths for \sysname-compatible vehicles. We call this component the \textit{centralized controller}. This component runs at the edge. 
%The edge runs trajectory planning for all \sysname-compatible vehicles on the road. 
% Self-driving vehicles today have a similar component today, however, this component is decentralized component so it plans a trajectory for a single vehicle. 

The perception module sends perception data about dynamic and static objects to the centralized controller. Dynamic objects include \sysname-compatible objects (vehicles with \sysname's low-level controller) and non-compatible objects (vehicles without \sysname's low-level controller, cyclists and pedestrians \etc). The centralized planner receives the position, bounding box, and motion vector (lines 1 and 2 of \algoref{algo:controller}) of every dynamic object from the perception module. Static objects include drivable area, the sidewalk, buildings, and traffic lights \etc For this, the planner receives a stitched 3D point cloud $S$ of the scene. It uses this to divide the scene into static obstacles and drivable space (line 3 of \algoref{algo:controller}).

\ramesh{does the term non-compatible also encompass cyclists and pedestrians?}
\fawad{Yes, addressed.}

The planner uses SIPP to plan every \sysname-compatible vehicle's motion. The planner converts the stitched point cloud $S$ into a 2D occupancy grid $S_{D}$ (with drivable and non-drivable blocks) and feeds it to SIPP (lines 3 and 4 of \algoref{algo:controller}). In a single agent scenario \ie only a single vehicle with no dynamic object, this occupancy grid would be enough for SIPP to plan a collision-free path. But in a realistic scenario, there are a number of dynamic obstacles which include both \sysname-compatible and non-compatible objects. \sysname needs to make SIPP aware of the locations of the objects at every instant in time in order to plan collision free paths. \sysname knows paths for all compatible objects because it plans paths for them. However, it has no way of knowing trajectories for non-compatible objects.

% an   The inputs to SIPP are: a) source and destination locations of the agent/car, and b) the set of obstacles in the environment. The set of obstacles consist of persistent static obstacles \eg the side-walk or a building and dynamic obstacles \eg traffic participants like other vehicles and pedestrains. Using these, SIPP plans the shortest non-collision path for the vehicle from source to destination.

To surmount this challenge, \sysname estimates the motion of all non-compatible vehicles\footnote{Like vehicles, we can estimate the motion of pedestrains as well. In this paper, we focus only on vehicles and the extension to pedestrains for future work.} and then feeds these estimates to SIPP (lines 5-9 of \algoref{algo:controller}). To do motion estimation for a non-compatible vehicle $v_{i}$, \sysname uses its motion vector $m_{i}$ and position estimate $p_{i}$ to forecast its trajectory $t_{i}$ over the next $X$ steps. To incorporate the vehicle's actual dimensions, \sysname uses the bounding boxes of every vehicle. However, this is not enough to relax the instant start/stop assumption of the SIPP algorithm or compensate for errors in perception/motion estimation.

To help alleviate the instant start/stop assumption and make the planner robust to perception errors, we form a motion adaptive buffer $d_{i}$ around the vehicle's trajectory $t_{i}$ (line 7 of \algoref{algo:controller}). The motion adaptive buffer wraps a dynamic bounding box around every position of the estimated trajectory $t_{i}$ for the vehicle $v_{i}$. The dynamic bounding box ensures safe driving distance between that vehicle and \sysname-compatible vehicles. This dynamic bounding box is a function of the vehicle bounding box $b_{i}$ and its motion vector $m_{i}$. At rest, the dynamic bounding box is the smallest and grows as the vehicle moves faster. Then, the planner feeds this to SIPP as a dynamic obstacle (line 8 of \algoref{algo:controller}). The planner uses the same technique for all non-compatible vehicles $V_{E}$ as well. 
% Finally, the controller combines the motion adaptive buffered trajectories of all vehicles and 

\ramesh{this notion of a motion adaptive box is interesting and could use a separate graphic as well as careful justification (perhaps it can be part of an ablation study)?}
\fawad{Please check now, I tried to justify it more and will add a figure too}

Next, the planner plans paths for all \sysname-compatible vehicles sequentially. The sequential order in which paths are planned allows for user-defined traffic policies. For instance, to prioritize an emergency vehicle at an intersection, SIPP will plan for it first and then use it as a dynamic obstacle for all other vehicles. So, the planner sorts \sysname-compatible vehicles $V^{'}_{C}$ based on a user-defined policy (line 10 of \algoref{algo:controller}). After this, the planner feeds the current position $p_{i}$ and goal $g_{i}$ of every compatible vehicle $v_{i}$ to SIPP. SIPP generates a set of collision-free way-points $w_{i}$ to take the vehicle from it position $p_{i}$ to its destination $g_{i}$ (line 13 of \algoref{algo:controller}). The planner sends these set of way points to the vehicle's on-board local low-level control module over the network (line 13 of \algoref{algo:controller}) using their cyber-physical association. Like a non-compatible vehicle, the planner forms a motion adaptive buffer around the current vehicle's trajectory and feeds it to SIPP as a dynamic obstacle for the next vehicle. At the end, the planner plans and sends paths to all compatible vehicles.



\ramesh{this notion of a policy being translated to the order in which your plan for vehicles is good. We might want to think a little bit about giving examples of practical policies, and how they can be translated into planning ordering. We don't have to go too deep into this, but we should be able to show the existence of 1 or 2 practical policies that can be implemented this way.}

% For every point in the estimated trajectory $t_{i}$, the motion adaptive filter wraps a bounding box around that   
% If SIPP assumptions about the world were true, controller could feed the trajectory $t_{i}$ of the vehicle $v_{i}$ to SIPP as dynamic obstacle. However, in the real-world, there can be errors in perception, or motion estimation and 

% For this, it extrapolates the vehi Given the present position estimate $p_{i}$, the motion estimation module extrapolates it using the magnitude and direction of the motion vector $m_{i}$ (line 6 of \algoref{algo:controller}). It uses the magnitude and direction of the the motion vector $m_{i}$ to determine position ov    estimates the motion of non-compatible vehicles and 
% Given an occupancy grid with static obstacles,  is a graph-search algorithm that finds the shortest path from source to destination in a given graph.  


% the centralized: a) stitched 3D  The centralized controller receives perception information about all the position, bounding box, and motion vector for every vehicle (both \sysname-compatible and non-compatible) along with a stitched point cloud from the perception module (\algoref{algo:controller}).  uses perception data (positions, bounding boxes, motion vectors and a drivable space map) from the perception module to generate trajectories for all \sysname-compatible vehicles. 
%% - Path planning
% \sysname uses the real-time scene understanding from the perception module to plan a safe and efficient path for vehicles to follow on the road. We call this component \textit{trajectory planning}. This component runs at the edge and it is a part of the planning module. The edge runs trajectory planning for all vehicles on the road. This creates opportunities for cross-car optimizations. Self-driving vehicles today have a similar component today, however, this component is decentralized component so it plans a trajectory for a single vehicle.

% \ramesh{For each component, say where it runs. Also, for path planning, say that the infrastructure has to do this for each car. This is an interesting point, because it permits cross-car optimizations unlike decentralized autonomous driving decisions made by each car.}
% \fawad{Addressed.}
%% - Delivery of low-level control signals
% \fawad{we might need a closed-loop component somewhere here}
\subsection{Local Planner}
Every \sysname-compatible vehicle has an on-board local low-level controller and PID controller that receives the set of planned way-points from the centralized planner over the network (\algoref{algo:planner}). The local controller translates these to low-level control signals (throttle, steer, and brake) that can be directly applied to each vehicle. The local controller runs every 2-3~ms in the vehicle. 

The local controller receives the planned trajectory $w$ from the centralized planner every 100~ms (line 1 of \algoref{algo:planner}). The planner may fail to plan a path for a vehicle or there might be a network failure. For robustness, the low-level controller checks if it has received the trajectory within a latency budget and if received path is valid (line 2 of \algoref{algo:planner}). If either of these are not true, it goes into recovery mode (line 3 of \algoref{algo:planner}). In recovery mode, the controller uses the last valid planned trajectory for the vehicle. The trajectory that the controller receives inform it of the vehicle's planned path for the next $X$ steps. It would have sufficed to send the vehicle its position for just the next 100~ms but this redundancy helps relax SIPP's instant start/stop assumption and introduces robustness.

\ramesh{The previous paragraph is important from a networking perspective. This idea is similar to soft state that permits robustness; see the Clark paper in the 551 readings.}

Given the planned trajectory $w$, the controller determines whether the vehicle has to wait at any point along it path (line 5 of \algoref{algo:planner}). We call this the wait cycle. If there is a wait cycle, it finds the position $p_{s}$ associated with the wait cycle and the distance of the vehicle from it $d_{s}$ (line 6 of \algoref{algo:planner}). Next, the controller calculates the braking distance $d_{b}$ (distance to bring the vehicle to a stop) of the vehicle using its current velocity $v$ (line 7 of \algoref{algo:planner}). If the braking distance is less than or equal to the distance from the stopping point (line 8 of \algoref{algo:planner}), the controller generates a signal $S$ to apply brakes (line 9 of \algoref{algo:planner}). Without this, vehicles would apply brakes at the spatial position of the wait cycle and hence overshoot it. With this maneuver, \sysname ensures that vehicles can adhere to SIPP's collision-free planned paths. On the other hand, if the vehicle is far away from the stopping point, then the controller generates a signal $S$ to continue moving the vehicle towards the stopping point (line 11 of \algoref{algo:planner}). We calculate braking distance using a standard equation~\cite{brakingdistance}.% and multiply it with a safety factor for robustness.

\ramesh{I couldn't find where wait cycle was previously defined.}
\fawad{Addressed.}

If there is no wait cycle in the entire trajectory $w$, the controller selects the next suitable way-point $p$ (line 14 of \algoref{algo:planner}) and generates a signal to move the vehicle towards that way-point (line 15 of \algoref{algo:planner}). Finally, the local controller applies the control signal $S$ to the vehicle (line 17 of \algoref{algo:planner}).


% As mentioned above, SIPP assumes that any vehicle can stop/start moving instantly. 
% After planning paths, \sysname sends them to all vehicles. %To do this, first, \sysname translates the path planned for each vehicle into low-level control (throttle and steering) signals. 
% To do this, first, \sysname associates the cyber presence of every vehicle in the perception module with its physical presence (network ID). This component lies at the edge inside the network module. Next, \sysname uses the network module to send the planned paths to all vehicles. %Current autonomous vehicle pipelines do  This component does not perform cyber-physical associations. %The first component (translation from path to signals) lies in the control module at the edge. 
% \sysname clients on the vehicles receive these trajectories. Besides this, the network module also transports data from sensors to the edge for perception. Self-driving vehicles pipelines today do not contain the network module. Then, these clients translate the planned trajectory into low-level control (throttle and steering) signals. The vehicle then uses these signals in closed feedback loop to drive the vehicle. This component lies in the control module at the vehicle. Current autonomous driving pipelines also contain a similar component.

% \fawad{Added a high-level planning layer that will reside at the cloud}
% Lastly, since the long time-scale path planning is relatively less latency-sensitive, it can be placed at the edge, the cloud or the car. This component draws safe and efficient paths for all vehicles from their origin to destinations. 

==> discussion.tex <==
\section{Discussions \& Future Work}
\label{sec:discussions}

\parab{Cyber-Physical Association}
To close the sensing-perception-control loop, we need to establish a \sysname-to-vehicle communication. We assume that the vehicles controlled by \sysname need to be equipped with some kinds of radio interface, such as WiFi, to receive the control commands. Each vehicles controlled by \sysname is assigned a unique NID(network id, such as a MAC/IP Address). \sysname can use the unique NID to send control message to the corresponding vehicle.

Each tracked vehicle in \sysname also receives a TID(tracking ID). Each vehicle in the LiDAR point cloud is consistently tracked by \sysname and receives the same TID. Because \sysname's planner and controller works with the instances detected in the LiDAR point cloud, they produce control commands based on the TIDs. To communicate the control commands to the corresponding vehicle in the physical world, \sysname needs to establish the association between TIDs and the NIDs.

Prior works (\cite{foresight}), \cite{roadmap} and \cite{roadview}) have explored thoroughly about how to combine a vehicle's visual feature(\eg color, shape, liscence plates, \etc) and electronic features(\eg GPS) at a given timestamp. Each vehicle will publish(through the network interface) its own feature vector and its NID, and at the same time receive feature vectors generated by other vehicles. At each timestamp, each vehicle measures the feature of its visual neighbors and perform feature matching between the set of visual features(through camera) and the received features(through network). Because each vehicle broadcast both its NID and its own features to its neighbors, this allows each vehicle to be discovered and matched by its neighbors.


% To learn the association, we need to know the positions in both the perception system and the physical world. For positions in the physical world, vehicles can equip GPS\cite{} or GNSS\cite{} to track their positions(longitude and latitude) in the geographical coordinate system. As mentioned previously, \sysname detects and tracks the positions of all the vehicle instances in the scene. Because \sysname knows the mounting position of the LiDARs, it can performs a trajectory matching between the GPS/GNSS sensor trajectories and the \sysname tracking trajectories. 

% Discussion and Future work
% - Real implementation
% - Scaling to large settings
% - Computational tradeoffs
% - Low latency
% - What would need to happen for deployment?https://www.overleaf.com/project/5eab1c82e1d472000137c95c

==> evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

Our evaluations show that \sysname: achieves frame rate processing and less than 100~ms tail latency both in real-world experiments (\secref{sec:eval-realworld}) and in simulation (\secref{s:simul-results:-laten}); achieves accuracy comparable to prior work (\secref{sec:eval-microbenchmark}); can be safer than autonomous driving  (\secref{s:bett-traff-manag}); and permits high-throughput traffic management (\secref{s:high-thro-traff}).

%% Outline for eval section
%% - Methodology (implementation, metrics, CarLA)
%% - end-to-end experiment
%% - CarLA end-to-end experiment (Fawad)
%% - perception microbenchmarks
%% - planning microbenchmarks

\subsection{Methodology}
\label{sec:eval-methodology}

%We conduct experiments on both a real-world testbed and a photorealistic autonomous vehicle simulator~\cite{Carla}.

\parab{Implementation.} We implemented \sysname's perception and planning on the Robot Operating System (ROS~\cite{quigley2009ros}). ROS provides inter-node (ROS modules are called \textit{nodes}) communication using publish-subscribe, and natively supports points clouds and other data types used in perception-based systems. \sysname runs as a ROS node that subscribes to point clouds, processes them as described in \secref{sec:design}, and publishes the results. The centralized planner builds on top of an open-source SIPP implementation~\cite{sipp_impl}, runs as a ROS node, subscribes to the perception results, and publishes trajectories for each vehicle. Perception requires 6909 lines of C++ code, and planning 3800.

% \weiwu{TODO: Che the testbed description for the updated hardware and lidar}
\parab{Real-world Testbed.} 
% \remove{Our testbed consists of three 64-beam Ouster~\cite{Ouster} LiDARs (two with $90^\circ$ and one with a $45^\circ$ field of view). The testbed also includes an edge computing unit with an Intel i9-10900KF CPU (20 core, 3.7GHz) and a GeForce RTX 3080 GPU;} 
Our testbed consists of four Ouster LiDARs~\cite{Ouster} (an OS-1 64, an OS-0 128, and two OS-0 64). Three of these have a field of view of $90^\circ$ while the last one has a $45^\circ$ field of view. \sysname is designed to accommodate this sensor heterogeneity. The testbed also includes an edge computing unit with an AMD 5950x CPU (16 cores, 3.4 GHz) and a GeForce RTX 3080 GPU; \sysname run on this. The LiDARs and the edge computing unit connect through Ethernet cables and an Ethernet switch (using an off-the-shelf Wi-Fi access point).

To demonstrate the use cases described in \secref{s:use_cases}, the centralized planner runs on the same edge computing unit as \sysname.
To transmit perception results and trajectories, \sysname uses in-vehicle Raspberry Pi 3 over Wi-Fi (as a proxy for 5G).

\parab{Simulation.} In our testbed, the trajectories derived from the centralized planner cannot be used to control vehicles, since vehicular control systems are proprietary. So, we complement our evaluations with a simulator which incorporates vehicular control. The simulator also helps us explore scaling \sysname. We use CarLA~\cite{Carla}, an industry-standard photo-realistic simulator for autonomous driving perception and planning. It contains descriptions of virtual urban and suburban streets, and, using a game engine, can (a) simulate the control of vehicles in these virtual worlds, and (b) produce LiDAR point clouds of time-varying scenes within these virtual worlds. Unless otherwise noted, our simulation based evaluations focus on intersections; several challenge scenarios for autonomous driving focus on intersections~\cite{nhsta2013,carlachallenge}. 

%ROS allows us to seamlessly bridge our \sysname implementation to either the simulator or the testbed. CarLA publishes point clouds using ROS, and Ouster also include ROS support in its SDK; \sysname subscribes to these over ROS. Conversely, \sysname publishes trajectories over ROS; a \sysname CarLA in-vehicle controller (\secref{s:planner}, \secref{s:local-controller}) subscribes to these, as does the Raspberry Pi in our implementation.

% The on-vehicle compute unit can join the ROS network and subscribes to the control commands.

% All components in the testbed are running in a single ROS network. We are using Ouster's provided ROS SDK to extract point clouds from the LiDARs' packets and publish to the corresponding ROS topic. We run \sysname-ROS package on the edge computing device and let \sysname's perception component subscribe to the point cloud topics. The ROS node running on each vehicle's Rasperberry Pi subscribes from the control topic which contains control commands publised by \sysname's planner. 

% \parab{Simulator Evaluation} For safety reason, we cannot have a large deployment of \sysname in the real world. To extensively evaluate \sysname's accuracy and capability to handle complicated scenario, we used CARLA~\cite{Carla} simulator to generates datasets and run different scenarios. With CARLA, we simulated 4 LiDARs at 4 corners of a intersection and published the LiDAR point clouds to the corresponding ROS topic. \sysname-ROS package's perception component subscribes from the topics and publish the perception results in another ROS topic. Similar to the real-world testbed setup, \sysname's planner will subscribe to the perception result topic and publish the control command. We implemented a CARLA low-level controller that subscribes these commands and converts to the actual vehicle controls(steering, throttle and break).

\parab{Metrics.} We quantify end-to-end performance in terms of the 99th percentile of the latency (\textbf{\textit{p99 latency}}) between when a LiDAR generates a frame, and when the vehicle receives the trajectory corresponding to that frame. To quantify accuracy of individual perception components, we use metrics described in prior work (defined later). We quantify planning efficacy by the rate of safety violations, or of undesirable outcomes such as deadlock.

\parab{Comparison.} Relative to autonomous driving, \sysname's perception has a more comprehensive scene understanding and can jointly plan for multiple vehicles at a time. To quantify this, we compare it against autonomous driving.

% \parab{Visualizations.} For many of our experiments, we have generated videos to complement our textual descriptions. These are available at an anonymous YouTube channel. \footnote{\url{https://www.youtube.com/channel/UCpb947_nEBAv_oikE7KsC-A}}

% We use the standard measures of tracking goodness, MOTA and MOTP\cite{mot_metric}, to evaluate how well \sysname can detect and track vehicle's positions in the scene. To measure the accuracy of the heading estimation, we calcualate the cosine similarity between the ground truth heading and the estimated heading direction. We also compare the magnitude component of the estimated heading vector(\ie the estimated speed) the ground truth speed.
% \weiwu{For the heading vector, I think we can choose between similarity or degree. Degree might be better because people can easily understand that. But we need to convert the real world result to be degree too(which doesn't look good). }

\subsection{Real-world Experiment}
\label{sec:eval-realworld}

% \begin{figure}[t]
%   \centering
  
%   \caption{Fused LiDAR frame from real-world deployment. The centers of the concentric circles represent LiDAR positions. Our two vehicles are also visible in the frame}
%   \label{fig:real-world-frame}
% \end{figure}
 
%\weiwu{This \figref{fig:end_to_end_latency} is actually hard to get it clear. The perception time is too large comparing to the other two. }

% \parab{Setup.}

%We ran \sysname for 5 minutes using our real-world testbed with 2 vehicles driving. We measures the end-to-end latency by calculating the time difference between the timestamp that \sysname received the point clouds and the timestamp that vehicles received the control command.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.8\columnwidth]{figs/fig_end_to_end_breakdown_mobicom.png}
%   \caption{End-to-end latency from real-world experiment.}
%   \label{fig:end_to_end_latency}
% \end{figure}
\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\columnwidth]{figs/fig_e2e_latency.pdf}
  \caption{Per-component end-to-end latency (left y-axis) along with the number of traffic participants (right y-axis) from a deployment of \sysname at a busy intersection in the real-world for over 30 minutes. A p99 latency of 91~ms suggests that \sysname stays within the 100~ms latency budget (dotted line) for autonomous driving.}
  \label{fig:end_to_end_latency}
\end{figure}

\parab{Deployment.}
% \remove{We deployed our testbed on a sidewalk along a major street in a large metropolitan area. For this experiment, we deployed three LiDARs along the side of the road, separated from one another by 20~m.} 
We deployed our testbed at a busy four-way intersection with heavy pedestrian and vehicular traffic in a large metropolitan area. For this experiment, we deployed the four LiDARs at the corners of the intersection (\figref{fig:intersection_example}(a)). These LiDARs connected to the edge compute device (described above) using Ethernet cables. The edge compute connected to Raspberry Pis on the vehicles through Wi-Fi (to proxy 5G). We collected data for nearly 30 minutes; we measured and report the end-to-end latency for every frame.

% \remove{Ideally, we would have liked to deploy the LiDARs at an intersection, but that would have involved disrupting traffic to establish wired connectivity across the intersection. We argue that our street-side deployment stresses \sysname at least as much as a deployment at an intersection would have, if not more. In our deployment, cars travel faster (speed limit: 45 mph); at an intersection, some cars are stationary or slow moving, so tracking, motion estimation and heading estimation algorithms need not be invoked on them.}

% For this experiment, we deployed our testbed atop a parking structure. Student volunteers drove two vehicles that were visible to the LiDARs at various times during the experiment. \sysname processed,\footnote{See YouTube channel for video} in real-time, frames from the three LiDARs, generated trajectories, transmitted them to the Raspberry Pis on the vehicles, which timestamped them. 

\parab{Results.}
\figref{fig:end_to_end_latency} shows the end-to-end latency for each frame, for over 30 minutes (approximately 18,000 frames), broken down by component.
% \remove{The y-axis is in \textbf{\textit{log scale}}.} 
The average end-to-end latency is 57~ms and p99 latency is 91~ms.
This shows that \sysname operates under the 100~ms latency budget set for autonomous driving by industry players like Udacity~\cite{udacity}, Mobileye\cite{mobileye}, and Tesla~\cite{tesla}. Moreover, \sysname processed LiDAR input at full frame rate. This is encouraging, and suggests that it is possible to achieve end-to-end performance with \sysname comparable to those in today's autonomous driving. \textit{Lastly, unlike autonomous driving pipelines today which control only a single vehicle, \sysname can control 10s of vehicles simultaneously within the 100~ms latency budget.}
%\weiwu{Thanks for updating the result. But it does have a few frames exceed 100ms, need to zoom in}

On average, at any given frame, \sysname detects 18 traffic participants (vehicles, pedestrians and cyclists) at the intersection during our experiment. As our experiment progressed, the traffic at the intersection steadily increased as shown by the dotted line in \figref{fig:end_to_end_latency} (representing the running average of traffic participants for 600~frames or 60~seconds). Because \sysname's latency depends on the number of traffic participants, this contributed to the slow increase in end-to-end latency towards the end of the experiment.

%\weiwu{To self: update the result with the 15min run}

From this graph, we also observe that: network latency is small \ie the average is 9~ms whereas p99 is 17~ms. The same is true for planning latency for which the average is 11~ms and p99 is 26~ms. Planning latency scales with the number of vehicles. As the number of vehicles increase through the course of the experiment, planning latency also increases. However, overall, perception latency (37~ms average and p99 of 60~ms) dominates, which motivates the careful algorithmic and implementation choices in \secref{sec:design}.

% In the real-world deployment, perception latency was higher (average of 37~ms and p99 of 60~ms) than in our CarLA-based evaluations (\secref{s:simul-results:-laten}) for two reasons. First, in our deployment, perception latency was affected by object \textit{size}. Our LiDARs were mounted at lower heights (2~m) than one might expect in a roadside deployment (to mimic which, our LiDARs in CarLA were mounted at 11~m). As a result, the point clouds corresponding to individual objects are larger, and several components that scale with the number of points of an object (like clustering, and heading vector estimation) take more time in our experiments. In practical deployments, point cloud size may not affect performance; because LiDARs scans are radial, the number of points representing an object drops off quickly with distance from the sensor. Second, in CarLA, we could only simulate 

% \weiwu{I think we can also mention another reason we are slower than carla is that we are having a more dynamic intersection than we can possibly simulate in Carla. The number of detected traffic participant at its 99th percentile is 29 and the 75th is 21. This will definitely make the latency larger.}

%\weiwu{I think the paragraph above is still valid, even the latency is not as high as the last submission. The p99 latency of perception is around 37ms}
%\figref{fig:end_to_end_latency} shows that the latency contributed by network communication and \sysname's controller is negligibly small compared to perception. We notice that the perception latency of the real-world experiment is significantly larger than the latency observed in microbenchmark evaluation of \secref{sec:eval-microbenchmark}. The reason behind that is we are able to deploy the LiDARs at the height of 11m(on the top of light poles), but we cannot make the same deployment in the real world experiment. Due to safety reasons, we can only mount our LiDARs at a height around 2m. Because of this, vehicles are closer to the LiDARs. This causes that each vehicle has much more points, and thus significantly slowdowns the components like background substraction, clustering and heading vector estimation.

\subsection{Latency Breakdown}
\label{s:simul-results:-laten}

\parab{Setup.}
To explore the total latency with more vehicles, and to understand the breakdown of latency by component, we designed several scenarios in CarLA with increasing numbers of vehicles traversing a four-way intersection. In these scenarios, CarLA (a) generates LiDAR data and (b) controls vehicles based on received trajectories; the results use the same \sysname code used in the real-world experiment. To control vehicles, we set the steer, brake and throttle values of a vehicle, exposed through the CarLA API.

At this intersection, both streets have two lanes in each direction. We varied the number of vehicles from 2 to 14, to understand how \sysname's components scale. To justify this range of the number of vehicles, we use the following data: the average car length is 15~ft~\cite{car_length}, and the width of a lane is 12~ft~\cite{lane_width}. Allowing for lane markers, medians, and sidewalks, let us conservatively assume that the intersection is 60~ft across. Suppose the intersection has traffic lights. Then, if traffic is completely stalled or moving very slowly, at most 4 cars can be inside the intersection per lane, resulting in a maximum of 16 cars (\ie the maximum capacity of the intersection is 16). If cars are stalled, \sysname does not incur much latency since it doesn't have to estimate motion, heading, or plan for these, so we limit our simulations to 14 vehicles.\footnote{We have verified that, above 14 vehicles, end-to-end latencies actually drop.} On the other hand, if traffic is moving at 45~mph (or 66~fps) and cars maintain a 3-second~\cite{three_second} safe following distance, then at most one car can be within the intersection per lane, for a total of 4 cars.

% \ramesh{Please add citations for car length, lane width and the 3-second rule.}
%\ramesh{Please review above para.}

\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{c|c|c|c|c|c|c}
\hline
 & \multicolumn{6}{c}{\textbf{Number of Vehicles}} \\ \hline \hline
\textbf{Component} & \textbf{2} & \textbf{4} & \textbf{7} & \textbf{10} & \textbf{12} & \textbf{14} \\ \hline
\begin{tabular}[l]{@{}l@{}}BG Subtraction\end{tabular} & 7.5 & 8.9 & 9.9 & 9.9 & 11.0 & 18.7 \\ \hline
Stitching & 0.08 & 0.11 & 0.13 & 0.13 & 0.17 & 0.19 \\ \hline
Clustering & 4.3 & 5.8 & 11.2 & 13.0 & 22.2 & 20.5 \\ \hline
  \begin{tabular}[l]{@{}l@{}}Bounding
    Box\end{tabular} & 0.06 & 0.07 & 0.09 & 0.15 & 0.17 & 0.16 \\ \hline
Tracking & 0.1 & 0.15 & 0.21 & 0.28 & 0.37 & 0.38 \\ \hline
\begin{tabular}[l]{@{}l@{}}Heading Vector\end{tabular} & 8.8 & 12.9 & 24.0 & 28.8 & 41.9 & 52.6 \\ \hline
% \begin{tabular}[l]{@{}l@{}}Motion\\ Vector\end{tabular} & 0.002 & 0.002 & 0.004 & 0.005 & 0.010 & 0.010 \\ \hline
\textbf{Total} & \textbf{18.5} & \textbf{26.4} & \textbf{43.7} & \textbf{47.1} & \textbf{69.9} & \textbf{81.5} \\ \hline
\end{tabular}
%\christina{Numbers updated}
\caption{p99 per-frame latency (in milliseconds) for perception. We exclude latency numbers for motion vector estimation which are on the order of a few microseconds.}
\label{tab:latency-ours}
\end{table}

\parab{Breakdown for Perception.}
\tabref{tab:latency-ours} depicts the breakdown of 99-th percentile (p99) latency by component for perception, as well as the total p99 latency, as a function of the number of vehicles in the scene. In all our experiments, \sysname processed frames at the full frame rate (10~fps).

The total p99 latency for perception increases steadily up to 82~ms for 14 vehicles\footnote{For many of our experiments, including this one, we have generated videos to complement our textual descriptions. These are available at an \textit{\textbf{anonymous YouTube channel}}: \url{https://www.youtube.com/channel/UCpb947_nEBAv_oikE7KsC-A}.} from 19~ms for 2 vehicles. This highlights the dependency of perception on scene complexity (\secref{sec:perception}); many components scale with the number of participants. At 14 vehicles, \sysname exceeds the latency budget, since planning requires over 20~ms for 14 vehicles (see below). These numbers suggest that modest off-the-shelf compute hardware that we have used in our experiments might be sufficient, at least for traffic management at moderately busy intersections. This data dependency also suggests that deployments of \sysname will need to carefully provision their infrastructures based on historical traffic (similar to network planning and provisioning). 

The three most expensive components are background subtraction, clustering, and heading vector estimation. Background subtraction accounts for about 10~ms, but depends slightly on the number of vehicles; to be robust, it uses a filter (details omitted in \secref{s:fusion}) that is sensitive to the number of points (or vehicles). Clustering accounts for about 20~ms with 14 vehicles and is strongly dependent on the number of vehicles, since each vehicle corresponds to a cluster.

Heading vector estimation accounts for nearly 65\% of perception latency, even after GPU acceleration (\secref{s:tracking}). These results show the fact that heading vector estimation is not only dependent on the number of vehicles, but their dynamics as well. When we ran perception on 16 vehicles, p99 latency actually dropped; in this setting,  16 vehicles congested the intersection, so each vehicle moved very slowly. Heading vector estimation uses ICP between successive object point clouds; if a vehicle hasn't moved much, ICP converges faster, accounting for the drop.

\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{c|c|c|c}
\hline
\multicolumn{1}{c|}{\textbf{Optimization}} & \textbf{Before} & \textbf{After} & \textbf{Ratio} \\ \hline \hline
  BG subt before stitching & 67.7 & 10.0 & 6.7 \\ \hline
%   background subtraction & & & \\ \hline
  Exploiting LiDAR characteristics & 9.9 & 1.5 & 6.6 \\ \hline
%   in background subtraction & & & \\ \hline
  Heading vector GPU acceleration  & 1057.7 & 28.8 & 36.6 \\ \hline
%   GPU acceleration & & & 
%   \\ \hline
\end{tabular}
%\christina{Numbers updated}
\caption{Impact of optimizations on p99 latency}
\label{tab:unopt_opt}
\end{table}

Other components are negligible. Stitching is fast because of the optimization described in \secref{s:fusion}. Bounding box estimation is inherently fast. Track association is cheap because it tracks a single point per vehicle (the centroid of the bounding box). Motion estimation is very fast (on the order of microseconds) and relies on positions computed during stitching. Thus, careful design choices that leverage abstractions and quantities computed earlier in the pipeline can be crucial for meeting latency targets (\secref{s:tracking}).

\parae{Benefits of optimizations.} \tabref{tab:unopt_opt} quantifies the benefits of our optimizations. Stitching before background subtraction requires nearly 70~ms in total; reversing the order reduces this time by 6.7$\times$. By exploiting LiDAR characteristics (\secref{s:fusion}), \sysname can perform background subtraction in 1.5~ms per frame.\footnote{\tabref{tab:latency-ours} does not include this optimization, since it can only be applied to some LiDARs} A CPU-based heading vector estimation requires nearly 1~s which would have rendered \sysname infeasible; GPU acceleration (\secref{s:tracking}) reduces latency by 35$\times$.

\parab{Calibration Steps}. Finally, alignment (\secref{s:fusion}) of 4 LiDARs takes about 4 minutes. This includes not just the time to guess initial positions, but to run the ICP (on a CPU). Because it is invoked infrequently, we have not optimized it.

\parab{Planning.} \tabref{tab:latency_planning} depicts the p99 planning latency. As expected, there is a dependency on the number of vehicles, since \sysname individually plans for each vehicle. Planning latencies can be slightly non-monotonic (the planning cost for 12 vehicles is more than that for 14) because the planner's graph search can depend upon the actual trajectories of the vehicles, not just their numbers.

\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{c|c|c|c|c|c|c}
\hline
\textbf{Number of Vehicles} & 2 & 4 & 7 & 10 & 12 & 14 \\ \hline
\textbf{p99 Latency (ms)} & 2.4 & 5.1 & 11.9 & 17.1 & 28.7 & 24.2 \\ \hline
\end{tabular}
\caption{p99 per-frame planning latency in milliseconds.}
\label{tab:latency_planning}
\end{table}

%We varied the number of vehicles driving around the intersection and measured the latency of each sub-component of \sysname's perception pipeline(shown in \figref{fig:perception_latency_ours} and \tabref{tab:latency-ours}). Across the runs, we observed that the total latency scales with the number of vehicles. Up to 10 vehicles, the average latency required by the perception components is 36.02ms, with a 99th percentile tail latency at 47.34ms. Across all the sub-components, background subtraction, stitching, association, normal vector estimation and motion vector estimation are having relatively constant latency regardless the number of vehicles. The latency of clustering and heading vector estimation scales with the number of vehicles. Clustering needs to process more points as more vehicles enter the scene, and heading vector estimation runs per vehicle per frame.

%\weiwu{The filtering actually does increase a little bit as the number of vehicle increase, even though we mentioned that it scales with the number of LiDARs. This should be due to the radius based outlier remover that we used. The more vehicle that we see, the more points need be process by the remover.}
% \weiwu{Ramesh: do you think we should use a line plot to represent this table of latency \tabref{tab:latency-ours}? I can quickly change it. The problem will be how to represent the 99 perentile.}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.8\columnwidth]{figs/perception_latency_ours.png}
%   \caption{Tail latency per-frame latency in our perception}
%   \label{fig:perception_latency_ours}
% \end{figure}

\subsection{Accuracy}
\label{sec:eval-microbenchmark}

\parab{Perception Component Accuracy.}
Using real-world data and simulation traces described above, we show that \sysname's positioning, heading, velocity, and tracking accuracies are comparable to that reported in other work. (For our real-world traces, we manually labeled ground-truth positions).

\parae{Metrics.}
We report positioning error (in m), which chiefly depends upon the accuracy of alignment. Heading accuracy is measured using the average deviation of the heading vector, in degrees, from ground truth. For estimating accuracy of velocity estimation, we report both absolute and relative errors. Finally, we use two measures to capture tracking performance~\cite{mot_metric}: multi-object tracking accuracy (MOTA) and precision (MOTP). The former measures false positives and negatives as well as ID switches (\secref{sec:design}); the latter measures average distance error from the ground-truth track.

\parae{Results.}
\tabref{tab:accuracy_results} summarizes our findings. Positioning error is about 8-10~cm in \sysname, both in simulation and in the real world; the state of the art LiDAR SLAM~\cite{vloam} reports about 15~cm error. Our heading estimates are comparable to prior work that uses a neural network to estimate heading. Speed estimates are highly accurate, both in an absolute sense (error of a few cm/s) and in a relative sense (over 97\%). 

Finally, tracking is also highly accurate. In the real-world experiment, tracking was perfect. In simulation, with 10 vehicles concurrently visible, MOTA is still very high (over 99\%), and significantly outperforms the state-of-the-art neural network in 3D tracking~\cite{mono3dt}, for two reasons. The neural network solves a harder problem, tracking from a moving LiDAR. Our fused LiDAR views increase tracking accuracy; when using a single LiDAR to track, MOTA falls to 93\%. Finally, MOTP is largely a function of positioning error, so it is comparable to that value.
%\christina{Updated carla-perception results and corresponding texts}

%From the real-world experiment, we manually labeled frames using a point cloud viewer. With the labeled ground truth positions, we then extract the ground truth speed of vehicles by calculating the total distance that each vehicle travels in 1 second. We then compare the ground truths with \sysname's output(shown in \tabref{tab:realworld_accuracy}). In terms of tracking quality, \sysname achieves $100\%$ in MOTA and $0.12 m$ in MOTP in euclidean distance.

% \begin{table}[t]
% \centering
% \begin{small}
% \begin{tabular}{|c|c|c|}
% \hline
%                             & Vehicle 1 & Vehicle 2 \\ \hline
% Localization Error(m)       & 0.13      & 0.11      \\ \hline
% Heading Accuracy(cos. sim.) & 0.95      & 0.85      \\ \hline
% Speed Error(m/s)            & 0.09      & 0.10      \\ \hline
% Speed Accuracy(\%)          & 93.53     & 87.62     \\ \hline
% \end{tabular}
% \end{small}
% \caption{Perception Accuracy for real-world experiment.}
% \label{tab:realworld_accuracy}
% \end{table}



\parab{Alignment Accuracy.}
Although alignment is performed only once, its accuracy is crucial for \sysname; without accurate alignment, \sysname's perception components could not have matched the state of the art (\tabref{tab:accuracy_results}).

\parae{Comparison alternatives.}
To show the efficacy of \sysname's novel alignment algorithm, we compared it against two alternative ways of obtaining an initial guess for ICP: a standard feature-based approach for ICP initial guesses, SAC-IA~~\cite{rusu09:_fast_point_featur_histog_fpfh}; and using GPS for alignment. In this experiment, we use point clouds from our simulations and real-world experiments. The three approaches estimate initial guesses for the pose of three LiDARs, and feed those poses to ICP for building a stitched point cloud. In our evaluations, we report the average root mean square error (RMSE) between the stitched point cloud (\textit{after} running ICP on the initial guesses) for every approach against a ground truth.
%The ground truth is stitched point cloud for which we obtain the LiDAR poses either by hand alignment or through ground truth positioning in the simulator.

% that we generate either through simulation or by 
% For every stitched point cloud, we compute two metrics.
% First, we compute the average root mean square error (RMSE) between the stitched point clouds against a ground truth stitched point cloud.
% Second, we calculate the e
% For every stitched point cloud, we calculated the average root mean square (RMSE) against a 
% After ICP stitching, we report the average root mean square error (RMSE) and rotational error.
% The RMSE is the average distance between points 
% In \tabref{tab:alignment_accuracy}, we report the average root mean square error (RMSE) 

\parae{Results.} \tabref{tab:alignment_accuracy} shows that \sysname's alignment results in errors of a few cm, almost 2-3 orders of magnitude lower error than the competing approaches, which explains why we chose this approach. SAC-IA~\cite{rusu09:_fast_point_featur_histog_fpfh} does not take any inputs other than the point clouds, and estimates the transformation between two point clouds using 3D feature matching. However, this works well only when point clouds have a large amount of overlap. In our setting, LiDARs are deployed relatively far from each other, resulting in less overlap, SAC-IA is unable to extract matching features from multiple LiDAR point clouds. Using GPS for alignment provides a good initial guess for the relative \textit{translation} between the LiDARs. However, GPS cannot estimate the relative \textit{rotation} between LiDARs, so results in poor accuracy.

% Similarly, using GPS for initial alignment in ICP is also not feasible because it does not provide information about the relative rotation between the LiDARs.
% If LiDARs are installed with exactly identical rotations, then our evaluations show that GPS-based alignment gives similar RMSE results to 
% \sysname.
% However, practically it is highly unlikely to install LiDARs with exactly similar rotations. 
% However, practically, this would be very cubersome.
% this is not practically possible


% , the point cloud regions of the same physical location in the different LiDARs are having different point density. This might influence the feature matching mechanism used by SAC-IA. 


% All three algorithms estimate initial transformation matrices for the three LiDARs

% To show the efficacy of \sysname's novel alignment algorithm, we compared it against two baselines \ie SAC-AI~\cite{sac

% \tabref{tab:alignment_accuracy} compares the alignment accuracy of using different ways of estimating the initial alignment in the intersection scenario. 

% Using GPS position of each LiDAR also doesn't provide good initial alignment for ICP. The intuition is that GPS positions can only provide the translational offsets of the alignment, but not the relative rotation between the LiDARs. 

% Indeed, we experimented on fixing an identity rotation for every LiDARs in the Carla simulation, and feeding the GPS location as the initial guess to ICP, the alignment accuracy was similar to our robust alignment's result. But we want to note that in practice, LiDAR installers can intentionally tilt or rotate the LiDAR to achieve better coverage. 
 
\begin{table}[t]
\centering
\begin{footnotesize}
\begin{tabular}{l|c|c|c} \hline
  \textbf{Metric} & \textbf{Real} & \textbf{Sim} & \textbf{Prior} \\ \hline \hline
  \textbf{Positioning Error (m)} & 0.10 & 0.08 & 0.15~\cite{vloam}   \\ \hline
 \textbf{Heading Error ($^\circ$)} & 8.17 & 6.45 & 5.10~\cite{intentNet}   \\ \hline
 \textbf{Speed Error (m/s)} & 0.04 & 0.06 & --- \\ \hline
 \textbf{Speed Accuracy (\%)} & 98.80 & 97.49 &  ---  \\ \hline
\textbf{MOTA (\%)} & 100 & 99.54 & 84.52~\cite{mono3dt}    \\ \hline
 \textbf{MOTP (m)} & 0.12 & 0.08 & ---  \\ \hline
\end{tabular}
\end{footnotesize}
%\christina{Numbers updated}
\caption{Perception accuracies from real-world data and simulation. The last column provides accuracies reported for these by prior work, for calibration, where available.}
\label{tab:accuracy_results}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\footnotesize
\centering
% \begin{footnotesize}
\begin{tabular}{|cc|cc|}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{}}                           & \multicolumn{2}{c|}{RMSE (m)}                            \\ \cline{3-4} 
\multicolumn{2}{|c|}{}                                            & \multicolumn{1}{c|}{Average}            & Std Dev       \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{Simulation}} & \textbf{\sysname} & \multicolumn{1}{c|}{\textbf{0.03}} & \textbf{0.02} \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                            & SAC-IA        & \multicolumn{1}{c|}{39.2}         & 13.4         \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                            & GPS           & \multicolumn{1}{c|}{23.8}         & 11.1         \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{Real-world}}  & \textbf{\sysname} & \multicolumn{1}{c|}{\textbf{0.09}} & \textbf{0.04} \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                            & SAC-IA        & \multicolumn{1}{c|}{11.8}         & 13.9         \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                            & GPS           & \multicolumn{1}{c|}{13.0}         & 1.2          \\ \hline
\end{tabular}
% \end{footnotesize}
\caption{\sysname's novel alignment algorithm outperforms existing state-of-the-art initial alignment algorithms.}
\label{tab:alignment_accuracy}
\end{table}

% \begin{table}[]
%   \centering
%   \begin{small}
%     \begin{tabular}{|c|c|c|c|}
%       \hline
%             & \# LiDARs & \# Points & Align. Error(m) \\ \hline
%       Loc 1 & 4         & 261112    & 0.090           \\ \hline
%       Loc 2 & 4         & 267076    & 0.064           \\ \hline
%       Loc 3 & 5         & 342000    & 0.037           \\ \hline
%       Loc 4 & 4         & 268332    & 0.038           \\ \hline
%       \end{tabular}
%   \end{small}
%   \caption{Alignment error at different locations of the simulator.}
%   \label{tab:alignment_error}
% \end{table}

%\parab{Point Cloud Alignment.} We evaluated the accuracy of the point cloud alignment using point clouds taken in the simulator. The simulator gives us the ground truth alignment of the LiDARs. We calculated the distance of each point transformed by the ground truth alignment and the same point transformed by \sysname's estimated alignment. The accuracy of our alignment is the mean of the distances. We ran \sysname's alignment module in different locations inside the simulator and reported the alignment errors in \tabref{tab:alignment_error}. The alignment errors are less than 10cm in average. The latency cost of aligning 4 LiDAR frames is around 4 minutes. 

% \begin{table*}[ht]
% \centering
% \begin{small}
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
%  & \multicolumn{7}{c|}{\# of Vehicles} \\ \hline
% Sub-component & 1 & 2 & 3 & 4 & 5 & 7 & 10 \\ \hline
% \begin{tabular}[c]{@{}c@{}}Background\\ subtracion\end{tabular} & \begin{tabular}[c]{@{}c@{}}6.84\\ (8.67)\end{tabular} & \begin{tabular}[c]{@{}c@{}}6.56\\ (7.40)\end{tabular} & \begin{tabular}[c]{@{}c@{}}7.18\\ (8.52)\end{tabular} & \begin{tabular}[c]{@{}c@{}}7.80\\ (8.69)\end{tabular} & \begin{tabular}[c]{@{}c@{}}8.43\\ (10.09)\end{tabular} & \begin{tabular}[c]{@{}c@{}}8.63\\ (10.22)\end{tabular} & \begin{tabular}[c]{@{}c@{}}8.67\\ (10.56)\end{tabular} \\ \hline
% Stitching & \begin{tabular}[c]{@{}c@{}}0.03\\ (0.07)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.04\\ (0.06)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.05\\ (0.09)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.06\\ (0.11)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.07\\ (0.10)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.09\\ (0.13)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.09\\ (0.14)\end{tabular} \\ \hline
% Clustering & \begin{tabular}[c]{@{}c@{}}1.77\\ (3.36)\end{tabular} & \begin{tabular}[c]{@{}c@{}}2.23\\ (2.59)\end{tabular} & \begin{tabular}[c]{@{}c@{}}3.60\\ (4.85)\end{tabular} & \begin{tabular}[c]{@{}c@{}}4.53\\ (6.13)\end{tabular} & \begin{tabular}[c]{@{}c@{}}5.98\\ (7.83)\end{tabular} & \begin{tabular}[c]{@{}c@{}}8.74\\ (11.19)\end{tabular} & \begin{tabular}[c]{@{}c@{}}10.19\\ (12.51)\end{tabular} \\ \hline
% Association & \begin{tabular}[c]{@{}c@{}}0.03\\ (0.05)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.03\\ (0.05)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.04\\ (0.07)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.05\\ (0.09)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.05\\ (0.07)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.07\\ (0.10)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.09\\ (0.14)\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Bounding box\\ estimation\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.03\\ (0.05)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.05\\ (0.06)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.07\\ (0.08)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.09\\ (0.15)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.11\\ (0.15)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.16\\ (0.22)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.21\\ (0.33)\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Heading vector\\ estimation\end{tabular} & \begin{tabular}[c]{@{}c@{}}4.35\\ (8.58)\end{tabular} & \begin{tabular}[c]{@{}c@{}}5.95\\ (9.44)\end{tabular} & \begin{tabular}[c]{@{}c@{}}7.93\\ (12.61)\end{tabular} & \begin{tabular}[c]{@{}c@{}}9.81\\ (16.07)\end{tabular} & \begin{tabular}[c]{@{}c@{}}15.23\\ (20.27)\end{tabular} & \begin{tabular}[c]{@{}c@{}}18.26\\ (25.03)\end{tabular} & \begin{tabular}[c]{@{}c@{}}16.76\\ (29.40)\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Motion\\ estimation\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.001\\ (0.001)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.001\\ (0.001)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.001\\ (0.002)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.001\\ (0.002)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.002\\ (0.002)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.003\\ (0.006)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.003\\ (0.005)\end{tabular} \\ \hline
% \textbf{Total} & \textbf{\begin{tabular}[c]{@{}c@{}}13.05\\ (19.24)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}14.87\\ (19.06)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}18.87\\ (22.75)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}22.35\\ (28.12)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}29.88\\ (37.50)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}35.94\\ (44.99)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}36.02\\ (47.34)\end{tabular}} \\ \hline
% \end{tabular}
% \end{small}
% \caption{Average(99th percentile) per-frame execution time (m/s) in our optimized perception}
% \label{tab:latency-ours}
% \end{table*}

% \begin{table*}[t]
% \centering
% \begin{small}
%   \begin{tabular}{|c|c|c|c|c|c|c|c|}
%     \hline
%     Dataset & \# of Vehicle & MOTA(\%) & MOTP(m) & Heading Sim. & Heading Error(Deg.) & Speed Error(m/s) & Speed Accuracy(\%) \\ \hline
%     A       & 1          & 100       & 0.08     & 0.994        & 6.288               & 0.060            & 98.745          \\ \hline
%     B       & 2          & 100       & 0.12     & 0.993        & 6.773               & 0.065            & 98.744          \\ \hline
%     C       & 3          & 99.50     & 0.06     & 0.997        & 4.209               & 0.032            & 98.343          \\ \hline
%     D       & 4          & 98.62     & 0.07     & 0.995        & 5.333               & 0.074            & 97.037          \\ \hline
%     E       & 5          & 94.71     & 0.10     & 0.992        & 6.700               & 0.034            & 98.565          \\ \hline
%     F       & 7          & 99.28     & 0.11     & 0.991        & 7.163               & 0.104            & 95.021          \\ \hline
%     G       & 10         & 99.54     & 0.08     & 0.993        & 7.156               & 0.068            & 97.531          \\ \hline
%     \end{tabular}
% \end{small}
% \caption{Tracking accuracy(MOTA and MOTP) and heanding vector estimation accuracy(direction and speed) in micro-benchmark}
% \label{tab:accuracy_microbenchmark}
% \end{table*}

%\parab{Multi-object Tracking Accuracy}. \tabref{tab:accuracy_microbenchmark}'s 3rd and 4th columns show the tracking accuracy in terms of MOTA and MOTP. Across all these runs with different numbers of vehicles, \sysname performs well in both MOTA: all runs have a MOTA of 94\% or higher. Higher MOTA values means that \sysname has few number of false negative("Miss"), false positive("Ghost") and ID switching. In fact, \sysname has no ID switching, in average less than 7 missed tracking and in average less than 1 ghost tracking across all these runs. MOTP of the runs are also good. All runs have MOTP less than 0.12m. The low MOTP indicates that \sysname can precisely track the position of vehicles in the scene, regardless of the number of vehicles.

%\parab{Heading Vector Estimation.} Heading vector estimation consists of two components, \ie direction and speed. \tabref{tab:accuracy_microbenchmark}(5th column) shows that \sysname can estimate the heading direction with error less than 8 degrees across all the runs. The speed estimation is also accurate with error up to 0.074m/s. This indicates an accuracy of 97.037\% by taking account of the absolute ground truth speed(\tabref{tab:accuracy_microbenchmark} 6th and 7th column).

%\christina{We are evaluating motion vectors with $w=10$, not heading vectors. Heading vector size doesn't mean speed.}

% \begin{table*}[ht]
% \centering
% \begin{small}
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
%  & \multicolumn{7}{c|}{\# of Vehicles} \\ \hline
% Sub-component & 1 & 2 & 3 & 4 & 5 & 7 & 10 \\ \hline
% Stitching & \begin{tabular}[c]{@{}c@{}}24.20\\ (25.92)\end{tabular} & \begin{tabular}[c]{@{}c@{}}23.82\\ (25.90)\end{tabular} & \begin{tabular}[c]{@{}c@{}}24.29\\ (28.02)\end{tabular} & \begin{tabular}[c]{@{}c@{}}24.34\\ (28.27)\end{tabular} & \begin{tabular}[c]{@{}c@{}}24.15\\ (26.24)\end{tabular} & \begin{tabular}[c]{@{}c@{}}24.20\\ (25.82)\end{tabular} & \begin{tabular}[c]{@{}c@{}}24.64\\ (29.50)\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Background\\ subtraction\end{tabular} & \begin{tabular}[c]{@{}c@{}}19.36\\ (38.91)\end{tabular} & \begin{tabular}[c]{@{}c@{}}19.21\\ (21.10)\end{tabular} & \begin{tabular}[c]{@{}c@{}}22.17\\ (48.19)\end{tabular} & \begin{tabular}[c]{@{}c@{}}23.61\\ (34.38)\end{tabular} & \begin{tabular}[c]{@{}c@{}}24.65\\ (27.12)\end{tabular} & \begin{tabular}[c]{@{}c@{}}28.69\\ (34.02)\end{tabular} & \begin{tabular}[c]{@{}c@{}}30.86\\ (38.26)\end{tabular} \\ \hline
% Clustering & \begin{tabular}[c]{@{}c@{}}1.89\\ (6.17)\end{tabular} & \begin{tabular}[c]{@{}c@{}}2.38\\ (2.91)\end{tabular} & \begin{tabular}[c]{@{}c@{}}4.26\\ (9.72)\end{tabular} & \begin{tabular}[c]{@{}c@{}}5.34\\ (6.93)\end{tabular} & \begin{tabular}[c]{@{}c@{}}6.64\\ (8.20)\end{tabular} & \begin{tabular}[c]{@{}c@{}}9.80\\ (12.51)\end{tabular} & \begin{tabular}[c]{@{}c@{}}11.40\\ (13.97)\end{tabular} \\ \hline
% Association & \begin{tabular}[c]{@{}c@{}}0.11\\ (0.25)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.15\\ (0.24)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.24\\ (0.48)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.30\\ (0.47)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.37\\ (0.52)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.52\\ (0.74)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.66\\ (0.76)\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Bounding box\\ estimation\end{tabular} & \begin{tabular}[c]{@{}c@{}}3.01\\ (5.70)\end{tabular} & \begin{tabular}[c]{@{}c@{}}4.62\\ (5.24)\end{tabular} & \begin{tabular}[c]{@{}c@{}}7.96\\ (16.54)\end{tabular} & \begin{tabular}[c]{@{}c@{}}10.09\\ (12.89)\end{tabular} & \begin{tabular}[c]{@{}c@{}}12.62\\ (14.66)\end{tabular} & \begin{tabular}[c]{@{}c@{}}18.82\\ (21.59)\end{tabular} & \begin{tabular}[c]{@{}c@{}}23.36\\ (29.05)\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Heading vector\\ estimation\end{tabular} & \begin{tabular}[c]{@{}c@{}}107.10\\ (230.99)\end{tabular} & \begin{tabular}[c]{@{}c@{}}173.78\\ (244.43)\end{tabular} & \begin{tabular}[c]{@{}c@{}}271.05\\ (457.67)\end{tabular} & \begin{tabular}[c]{@{}c@{}}325.87\\ (547.39)\end{tabular} & \begin{tabular}[c]{@{}c@{}}473.68\\ (645.15)\end{tabular} & \begin{tabular}[c]{@{}c@{}}668.73\\ (934.72)\end{tabular} & \begin{tabular}[c]{@{}c@{}}751.97\\ (1057.72)\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Motion\\ estimation\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.002\\ (0.003)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.004\\ (0.004)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.005\\ (0.07)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.007\\ (0.012)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.008\\ (0.012)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.012\\ (0.015)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.018\\ (0.039)\end{tabular} \\ \hline
% \textbf{Total} & \textbf{\begin{tabular}[c]{@{}c@{}}155.69\\ (296.98)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}223.96\\ (294.07)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}329.98\\ (502.60)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}389.55\\ (612.13)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}542.12\\ (715.28)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}750.77\\ (1020.83)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}842.92\\ (1148.25)\end{tabular}} \\ \hline
% \end{tabular}
% \end{small}
% \caption{Average(99th percentile) per-frame execution time in unoptimized perception}
% \label{tab:latency_unopt}
% \end{table*}

% \begin{table}[]
% \centering
% \small
% \begin{tabular}{|c|c|c|c|}
% \hline
% \multicolumn{1}{|l|}{\textbf{}} & Unopt & Opt & Ratio \\ \hline
% Stitching & 29.50 & 0.14 & 207.51 \\ \hline
% Background Subtraction & 38.26 & 10.56 & 3.62 \\ \hline
% Heading Vector Estimation & 1057.72 & 29.40 & 35.98 \\ \hline
% \end{tabular}
% \caption{Tail latency of unoptimzed vs optimized perception with 10 vehicles}
% \label{tab:unopt_opt}
% \end{table}

% % \begin{figure}[t]
% %   \centering
% %   \includegraphics[width=0.8\columnwidth]{figs/perception_latency_unopt.png}
% %   \caption{Tail latency per-frame latency in unoptimized perception}
% %   \label{fig:perception_latency_unopt}
% % \end{figure}

% We implemented three optimizations in our perception to meet real-time latency: (1) We did background subtraction first (2) We do parallel subtraction and (3) We adopt GPU to do ICP for heading vector estimation. As shown in \ref{fig:perception_latency_unopt}, unoptimized perception faces latency bottleneck in heading vector estimation, background subtraction, and stitching, and it rationalize our optimizations above. Thanks to (1) background subtraction fisrt pipeline and (2) parallel subtraction, we are able to reduce the latency of subtraction and stitching by a factor of 6. GPU-ICP reduces the latency of heading vector estimation by a factor of 33. In summary, per-frame tail latency is reduced by a factor of 20.

\subsection{Safety}
\label{s:bett-traff-manag}

In this section, we demonstrate \sysname's use case to improving safety in autonomous driving.
\sysname has a comprehensive view of an intersection, so it can lead to increased safety. To demonstrate this, we implemented two scenarios in CarLA from the US National Highway Transportation Safety Administration (NHTSA) precrash typology~\cite{nhsta2013}; these are challenging scenarios for autonomous driving~\cite{carlachallenge}.

\parae{Red-light violation.}
A red truck and the ego-vehicle (yellow box) approach an intersection (\figref{fig:red_light_violation}). An oncoming vehicle (red box) on the other road violates the red traffic light. The red truck can see the violator and hence avoid collision, but the ego-vehicle cannot. 

\parae{Unprotected left-turn.}
The ego-vehicle (yellow box) heads towards the intersection (\figref{fig:unprotected_left_turn}). A vehicle (red bounding box) on the opposite side of the intersection makes an unprotected left-turn. The ego-vehicle's view is blocked by the trucks on the left lane.

\parae{Methodology and metrics.} In each scenario, \sysname augments the ego-vehicle's on-board perception. When comparing against autonomous driving, to ensure a more-than-fair comparison, we: (a) equip autonomous driving with ground-truth (perfect) perception; and (b) use an on-board SIPP planner in single-mode (plan only for the ego-vehicle) for autonomous driving. The alternative would have been to use an open-source stacks like Autoware~\cite{Autoware} which has its own perception and planning modules. However, in these experiments we are trying to understand the impact of augmenting a vehicle's perception with \sysname, so we chose a simpler approach that equalizes implementations.

For both scenarios, we vary speeds and positions of the ego-vehicle and oncoming vehicle to generate 16 different experiments. We then compare for what fraction of experiments each approach can guarantee safe passage.

\parae{Results.}
In both scenarios (\tabref{tab:end_to_end_experiments}), autonomous driving ensures safe passage in fewer than 20-40\% of the cases. \sysname achieves safe passage in all cases because it senses the oncoming traffic even though it is occluded from the vehicle’s on-board sensors\footnote{\label{youtube}Please see YouTube channel for videos.}. This gives the planner enough time to react and plan a collision avoidance maneuver (in this case, stop the vehicle). Of the two cases, the unprotected left-turn was the more difficult one for \sysname (as it is for autonomous driving, which fails more often in this case), yet it is still able to guarantee safe passage in all 16 cases. In the red-light violation scenario, \sysname senses the oncoming traffic early on and has enough time to react. However, in the unprotected left-turn, the ego-vehicle is traveling relatively fast and the oncoming traffic takes the left-turn at the last moment. Though \sysname has a smaller time to react, its motion-adaptive bounding box and stopping distance estimation ensure that the vehicle stops on time.

% \begin{figure}[t]
% \begin{minipage}{0.49\linewidth}
%     \centering
%  \includegraphics[width=0.85\columnwidth]{figs/fig_red_light_violation.pdf}
%     \caption{The orange truck obstructs ego-vehicle's (yellow box) view of red-light violator.}
%     \label{fig:red_light_violation}
% \end{minipage}
% \begin{minipage}{0.49\linewidth}
% \centering
%  \includegraphics[width=0.85\columnwidth]{figs/fig_unprotected_left_turn.pdf}
%     \caption{The orange truck obstruct the ego-vehicle's (yellow box) view of left-turning car.}
%     \label{fig:unprotected_left_turn}
% \end{minipage}
% \end{figure}
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{c|c|c}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{NHTSA}\\ \textbf{Scenario}\end{tabular}} & \multicolumn{2}{c}{\textbf{Safe Passage (\%)}} \\ \cline{2-3} 
                      & \textit{\sysname} & \textit{Autonomous Driving} \\ \hline \hline
Red-light Violation   & 100                     & 37                 \\ \hline
Unprotected Left-turn & 100                     & 18                 \\ \hline
\end{tabular}
\caption{With more comprehensive perception, \sysname can provide safe passage to vehicles in both scenarios.}
\label{tab:end_to_end_experiments}
\end{table}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.7\columnwidth]{figs/fig_traffic_lights.pdf}
%   \caption{\sysname enables traffic light free intersections and can reduce wait times by 5~x.}
%   \label{fig:traffic_light}
% \end{figure}

% \begin{minipage}[t]{0.24\textwidth}
%   \centering
%   \includegraphics[width=0.9\columnwidth]{figs/fig_traffic_lights.pdf}
%   \caption{\sysname enables traffic light free intersections and can reduce wait times by 5~x.}
%   \label{fig:traffic_light}
% % \end{minipage}
% \begin{figure}
%   \centering
%   \includegraphics[width=0.5\columnwidth]{figs/fig_packet_loss.pdf}
%   \caption{\sysname can ensure collision-free trajectories with up to 70\% packet-loss rates.}
%   \label{fig:packet_loss}
% % \end{minipage}
% \end{figure}

\begin{figure}[t]
\begin{minipage}{0.49\linewidth}
    \centering
 \includegraphics[width=0.99\columnwidth]{figs/fig_packet_loss.pdf}
    \caption{\sysname can ensure collision-free trajectories with up to 70\% packet-loss rates.}
  \label{fig:packet_loss}
\end{minipage}
\begin{minipage}{0.49\linewidth}
\centering
 \includegraphics[width=0.99\columnwidth]{figs/fig_traffic_lights.pdf}
   \caption{\sysname minimizes average wait times (seconds) for vehicles with traffic light free intersections.}
   \label{fig:traffic_light}
\end{minipage}
\end{figure}



\parab{Robustness to Packet Loss.}
In our implementation, the centralized planner transmits trajectories wirelessly to vehicles. It generates trajectories over a longer time horizon (\secref{s:centralized_planning}) to be robust to packet loss. To quantify its robustness, we simulated packet losses ranging from 0 to 100\% for in the red-light violation scenario (\figref{fig:red_light_violation}). For each loss rate, we measured the stopping distance between the ego-vehicle and the oncoming traffic which violates the red-light. Higher stopping distances are good (\figref{fig:packet_loss}). We repeated the experiment multiple times for each loss rate. As we increased the packet-loss, the stopping distance decreased because the ego-vehicle was operating on increasingly stale information. Even so, \sysname ensures collision-free passage for the ego-vehicle through the intersection till 70\% loss, with minimal degradation in stopping distance till about 40\% loss.

% \fawad{Added the following for traffic light free intersection}



% \begin{figure}
%   \centering
%   \includegraphics[width=0.5\columnwidth]{figs/fig_packet_loss.pdf}
%   \caption{\sysname can ensure collision-free trajectories with up to 70\% packet-loss rates.}
%   \label{fig:packet_loss}
% \end{figure}

% \begin{minipage}[t]{0.24\textwidth}
%   \centering
%   \includegraphics[width=0.9\columnwidth]{figs/fig_traffic_lights.pdf}
%   \caption{\sysname enables traffic light free intersections and can reduce wait times by 5~x.}
%   \label{fig:traffic_light}
% \end{minipage}
% \begin{minipage}[t]{0.24\textwidth}
%   \centering
%   \includegraphics[width=0.9\columnwidth]{figs/fig_packet_loss.pdf}
%   \caption{\sysname can ensure collision-free trajectories with up to 70\% packet-loss rates.}
%   \label{fig:packet_loss}
% \end{minipage}
% \end{figure*}

\subsection{High-Throughput Traffic Management}
\label{s:high-thro-traff}
In this section, we demonstrate \sysname's use case to alleviating traffic congestion.
Intersections contribute significantly to traffic congestion~\cite{AIMSurvey}; \textit{\textbf{traffic-light free intersections}} can reduce congestion and wait times.  A centralized planner, enabled by \sysname, because it centrally plans trajectories for all \sysname-capable vehicles, can plan collision-free trajectories at an intersection without traffic lights. We have verified this in simulations as well.\footnoteref{youtube}

\parab{Wait-time Comparison.}
A traffic-light free intersection can significantly reduce wait times at intersections, thereby enabling higher throughput. To demonstrate this, we compared \sysname's average wait times (using a centralized planner) at an intersection against three other approaches:
\begin{itemize}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex,leftmargin=*]
\item \textit{Static.} An intersection with static traffic lights.
\item \textit{Intelligent.} Intelligent traffic light control~\cite{intelligent_tl} which prioritizes longer queues.
\item \textit{Ideal-Coop.} A traffic-light free intersection where autonomous vehicles use centralized perception but on-board \textit{decentralized planning} (as described in \secref{s:augment_vehicle_perception}). This represents an idealized version of cooperative perception like AVR~\cite{AVR}, Autocast~\cite{autocast} and EMP~\cite{emp} because it assumes that every vehicle has complete perception of all other traffic participants.
\end{itemize}
% \textit{Static.} An intersection with static traffic lights.
% \textit{Intelligent.} Intelligent traffic light control which prioritizes longer queues.
% \textit{Ideal-Coop.} A traffic-light free intersection where autonomous vehicles use centralized perception but on-board \textit{decentralized planning}. This represents an idealized version of cooperative perception like AVR~\cite{AVR}, Autocast~\cite{autocast} and EMP~\cite{emp} because it assumes that every vehicle has complete perception of all other traffic participants.


For the first two approaches, we obtained policies from published best practices~\cite{sumo,fhwa,natco}. In all experiments, we placed four LiDARs at an intersection in CarLA. 

\parab{Results.}
Compared to \textit{Static} and \textit{Intelligent}, \sysname reduces average wait times for vehicles by up to 5$\times$ (\figref{fig:traffic_light}). \sysname performs better than even \textit{Intelligent} because it can minimize the stop and start maneuvers at the intersection (by preemptively slowing down some vehicles), and hence can increase overall throughput, leading to lower wait times.\footnoteref{youtube}

Interestingly, beyond about 6 vehicles, wait times for strategies that use traffic lights (\textit{Static} and \textit{Intelligent}) drop. Recall that our intersection has two lanes in each direction. As the number of vehicles increases, the probability that a vehicle can pass the intersection without waiting increases. For example, with \textit{Intelligent}, a vehicle waiting at an intersection can trigger a green light, so a vehicle arriving in the adjoining lane can freely pass. Even so, \sysname has lower wait times than other alternatives up to 10 vehicles (wait time comparisons are similar beyond this number, results omitted for brevity).

\figref{fig:traffic_light} shows infinite wait times for \textit{Ideal-Coop}. That is because, although one might expect that a decentralized planner might have comparable throughput to \sysname, we found that it \textbf{\textit{led to a deadlock}} (\secref{s:centralized_planning}) with as few as two vehicles (each vehicle waited indefinitely for the other to make progress, resulting in zero throughput).\footnoteref{youtube} Fundamentally, this occurs because, with \textit{Ideal-Coop}, vehicles lack global knowledge of planning decisions. Thus, deadlocks can happen at intersections without traffic lights even for more practical cooperative perception approaches which use on-board planners like AVR~\cite{AVR}, Autocast~\cite{autocast}, EMP~\cite{emp}.

% \begin{table}[t]
% \footnotesize
% \begin{tabular}{c|c|c|c|c}
% \hline
% \textbf{Vehicle Count} & \textbf{Static} & \textbf{Intelligent} & \textbf{Ideal-Coop} & \textbf{\sysname} \\ \hline \hline
% 2             & 26.0   & 16.5        & $\infty$           & 4.0      \\ \hline
% 3             & 33.7   & 15.7        & $\infty$           & 4.7      \\ \hline
% 4             & 28.3   & 17          & $\infty$           & 5.0      \\ \hline
% 5             & 33.0   & 21.6        & $\infty$           & 5.4      \\ \hline
% 6             & 34.3   & 23.7        & $\infty$           & 5.8      \\ \hline
% 7             & 20.3   & 17.9        & $\infty$           & 5.7      \\ \hline
% 8             & 21.8   & 16.1        & $\infty$           & 5.5      \\ \hline
% 9             & 29.9   & 18.0        & $\infty$           & 6.7      \\ \hline
% 10            & 31.0   & 17.4        & $\infty$           & 8.2 \\ \hline    
% \end{tabular}
% \caption{\sysname minimizes average wait times (seconds) for vehicles with traffic light free intersections. Conventional traffic light strategies (Static and Intelligent) have more wait times due to start/stop maneuvers. Cooperative perception techniques (Ideal-Coop) can result in deadlocks ($\infty$ wait time) due to lack of global views.}
% \label{tab:traffic_light}
% \end{table}


% To demonstrate this, at an intersection with multiple \sysname-capable vehicles, in the simulator, we compared the average wait times we compared three approaches: a) conventional traffic a) \sysname and, b) a system with \sysname's centralized perception but with on-board decentralized/ego-planning at every vehicle. In this experiment, we evaluated the ability of both approach to ensure collision-free passage for all vehicles. We verified that \sysname ensured collision-free passage for all vehicles (see video on YouTube channel). On the other hand, in the approach with decentralized planning, with a few as 2 vehicles in the intersection, the approach resulted in a deadlock. In case of a deadlock, the vehicles were stuck at the intersection because there was no tie-breaker rule for the right-of-way.

% This is not possible the presence of a centralized controller (\eg in today's autonomous vehicles). 

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.6\columnwidth]{figs/fig_packet_loss.pdf}
%   \caption{\sysname can ensure collision-free trajectories with up to 70\% packet-loss rates.}
%   \label{fig:packet_loss}
% \end{figure}



% For this, we used the Gilbert-Elliot~\cite{packetloss} model to estimate the probability of packet losses (in our case, this was 40\%). We dropped a planning message every frame with this probability. We witnessed bursts of packet losses. Even so, for all 16 setups in the red-light violation scenario, \sysname ensured collision-free passage to the ego-vehicle.




%\parab{Traffic-free intersections.}


==> future_works.tex <==
\section{Future Work}
\label{s:future}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.95\columnwidth,trim={5cm 5cm 10cm 10cm},clip]{figs/cip_situ_aware.jpg}
  \caption{An example of CIP-enabled situational awareness through a real-time outdoor augmented reality system. 3D points (and bounding boxes) belonging to the moving pedestrian and the truck are captured by road-side LiDARs, and then sent and projected to an AR headset. In this example, the static background (\eg buildings, and parked vehicles) are not highlighted.
  }
  \label{fig:ar_situ_aware}
\end{figure}

Future work can seek to extend the current \sysname implementations in the following ways.
% \begin{itemize}[nosep,wide]

\parab{Optimizations:} \sysname's perception and the centralized planning modules are relatively unoptimized; they execute perception and planning for every participant in every frame. It can avoid tracking and estimating heading for stationary vehicles and pedestrians (\eg those waiting at the intersection). It can also avoid planning for such vehicles. Future work can explore these, and other optimizations (parallelizing tracking and heading estimation).

\parab{Edge Provisioning and Auto-scaling.} \sysname's perception and the centralized planning modules are sensitive to the number of participants. To deal with this, future work can explore provisioning strategies which take historical traffic into account to provision edge compute to meet p99 latency goals. Alternatively, future work can also explore auto-scaling strategies: scaling-out edge compute when p99 latencies start to increase. 


\parab{Large-scale Deployment.} Beyond intersections, \sysname can, in theory, enable a future world \textit{without autonomous driving}; cars would not have on-board perception and planning, but would simply follow \sysname-generated trajectories. This can eliminate the need for expensive sensors~\cite{qzvehiclecost,reutersvehiclecost}, power-hungry on-board compute~\cite{lin18:_archit_implic_auton_drivin}, and expensive high-definition maps~\cite{3dmapcost}. To achieve this vision, infrastructure needs to be installed everywhere, which will require much work: cost/benefit economic analyses, public-private partnerships to install infrastructure, regulatory approvals, buy-in from vehicle owners \etc 

\parab{Pedestrian Situational Awareness.} \sysname's perception can provide situational awareness for pedestrians. 
Perception outputs from \sysname can be used to generate audio cues to  alert visually-impaired pedestrians about oncoming vehicles.
For more immersive applications, \sysname's perception outputs can be fused in real-time with AR/MR headsets for outdoor augmented reality applications.
In such a scenario, \sysname's perception results can be streamed to, and accurately positioned in AR/MR headsets that pedestrians use (as illustrated in \cref{fig:ar_situ_aware}).
% illustrates a demo in which pedestrians wore AR/MR headsets that accurately track their head pose, and \sysname's perception outputs were streamed and rendered to the headset in real-time. 
In this example, although the truck was partially blocked by other vehicles, \sysname's perception (generated from road-side mounted LiDARs) enables a \textit{virtual-see-through} capability on the pedestrian's AR headset.
% \end{itemize}

==> intro.tex <==
\section{Introduction}
\label{sec:intro}

Technological changes have often spurred architectural shifts that have fundamentally altered the placement of functionality across a network. Some of these architectural shifts change the way the network itself works or is managed. A good example is software-defined networking (SDN), which de-couples the network's control plane from its data plane. Other architectural shifts change the design of applications and systems that use the network. For example, the advent of cloud computing inspired a class of cloud-enabled mobile applications that offload compute and storage for enhanced user experience. 

\parab{What is \sysname?}
In this paper, we explore an impending architectural shift in how autonomous vehicles use the network, a shift that resembles SDN. Today, autonomous vehicles use expensive sensors (like LiDARs) and run a software stack with three components (\figref{fig:netd_arch}(a)): \textit{perception} for scene understanding, trajectory \textit{planning}, and actuator \textit{control} to realize planned trajectories (\secref{sec:background}). This stack runs on-board the vehicle (\secref{sec:background}); if today's autonomous vehicles use the network at all, it is for over-the-air upgrades, and analytics uploads.

The drop in prices of sensors~\cite{sslidars,memslidar,huawei_lidar}, the increased deployment of edge computing~\cite{nvidiaedge,ibmedge,edgegartner}, and the rollout of 5G-based vehicular connectivity~\cite{amazon_edge,Qualcomm5g,5g} suggest an architectural shift that we call \sysname, in which components in the network remotely ``drive'' vehicles. \sysname \textit{decouples perception and planning from control\footnote{Control effects actuators using sub-millisecond control loops, so must remain in-vehicle.}} and offloads them to road-side infrastructure (\figref{fig:netd_arch}(b)). \sysname's perception component fuses data from multiple infrastructure-mounted sensors to develop scene understanding, and its planning component generates trajectories for all vehicles in view of the sensors. It continuously transmits, over wireless, these trajectories back to vehicles, which simply follow these planned trajectories (\secref{sec:architecture}).

% Source for this figure: https://docs.google.com/drawings/d/1kdvaR-D6rY5hBKQKm-tiCHll9FoDNA6UmvDqLW2ALOI/edit?usp=sharing
\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\columnwidth,frame]{figs/NetDriving_arch.pdf}
  \caption{(a) Autonomous vehicles run perception, planning and control on-board. (b) \sysname decouples perception and planning, placing these on edge-compute infrastructure, from control. (c) This decoupling is analogous to the control/data separation in SDN.}
  \label{fig:netd_arch}
\end{figure}

\parab{Resemblance to SDN.}
This resembles the decoupling of control and data planes in SDN (\figref{fig:netd_arch}(c)). In SDN, the logically-centralized control plane programs switches to direct traffic flows. Armed with a global view of the network, it can enable higher network utilization~\cite{B4,SWAN} and provide better abstractions for controlling network traffic~\cite{pyretic}.

Similarly, \sysname ``programs'' vehicle trajectories. Armed with a more complete view than a single vehicle, it can potentially ensure higher safety, better vehicular traffic throughput using long-desired transportation innovations (\eg platooning~\cite{platooning2011} and traffic-light free intersections~\cite{traffic-light-free}), and maybe even better abstractions for customizable traffic policies. This is because: (a) \sysname's perception fuses multiple sensors, it can see more than sensors mounted on a single vehicle\footnote{Sensors used for perception have line-of-sight limitations. A vehicle may not be able to see those oncoming vehicles in the opposite lane that are obstructed by the vehicle in front of it (\secref{sec:background}).}, resulting in increased safety; (b) because the planner can jointly plan trajectories for multiple vehicles.

\parab{A Key Challenge.} In addition to identifying and describing this architectural shift (\secref{s:de-coupl-perc}), this paper takes a first step towards addressing a basic technical question underlying the design of \sysname: can it match the performance and accuracy expected of today's autonomous vehicles? Today, autonomous vehicles must process sensor data at frame rates and produce trajectories with a tail latency of less than 100~ms~\cite{lin18:_archit_implic_auton_drivin, udacity, mobileye}. If \sysname cannot meet these requirements, it simply cannot be a viable alternative, since violations of these performance requirements can compromise safety. It is not immediately obvious that \sysname can meet these requirements, since it must be able to process multiple sensors concurrently, and generate trajectories for tens of vehicles or more at a time. This is challenging to do because these sensors  produce voluminous data (several hundred Gbps) and accurately extracting scene understanding and planning trajectories from these within a tight latency budget requires algorithmic innovations and the judicious use of hardware acceleration.

\parab{How \sysname Addresses the Challenge.}
\sysname's perception component (\secref{sec:perception}) generates near real-time instantaneous \textit{composite views} by stitching together LiDAR frames from multiple roadside sensors, then extracts dynamic objects, tracks them, and estimates their heading and motion vectors from successive composite views. Aside from using known techniques for some of these tasks, it uses novel robust techniques for sensor alignment and for estimating the heading of a vehicle of another participant (and accelerates the latter using a GPU because it is the bottleneck).

\sysname's planning component (\secref{s:planner}) jointly plans trajectories for multiple vehicles using the output of perception. It builds upon prior work in distributed robotic motion planning~\cite{SIPP}, but adapts it significantly to support vehicles of different sizes as well as \sysname-oblivious participants (\eg pedestrians or legacy vehicles), and adds vehicle kinematic constraints (like stopping distances) and driving experience constraints (like safe driving distances), without compromising correctness and performance.

Evaluations on a testbed as well as on a photorealistic autonomous vehicle simulator~\cite{Carla} show that: \sysname achieves its performance objectives end-to-end, being able to process frames from 3 LiDARs at 10~fps with a 99-th percentile tail latency under 100~ms; its perception component can track vehicles to centimeter-level accuracy (comparable to SLAM~\cite{ORB-SLAM2}-based positioning); and its planner results in fewer safety violations than today's autonomous vehicle designs and even alternative designs that rely on infrastructure-based perception, and can demonstrate safe traffic-light free intersections.

\parab{Contributions.} The paper makes the following contributions:
\begin{itemize}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex,leftmargin=*]
\item A new architecture for self driving vehicles which offloads perception and planning to the network edge.
\item A novel, fast, pipeline for perception using composite views obtained from multiple roadside sensors.
\item A fast planner for jointly planning trajectories of multiple vehicles while taking practical constraints into account.
\item An end-to-end implementation that satisfies tail latency, throughput, and accuracy requirements of autonomous vehicles.
\end{itemize}

\sysname is inspired by recent and planned roadside deployments of advanced sensors, and a large body of work on augmenting connected autonomous vehicle perception using infrastructure-based sensors (\secref{sec:related_work}). To our knowledge, no prior work has even considered combining infrastructure-based perception and planning~---~\sysname demonstrates the end-to-end viability of such a capability.

% Introduction:
% - Architectural innovation driven by functional de-coupling
%   - Control-data separation in networks
%   - Other examples
% - Position: de-coupling sensing and actuation can have significant benefits for autonomous driving


==> intro_new.tex <==
\section{Introduction}
\label{sec:intro}

Autonomous driving has made rapid strides in the past few years, and full autonomy may be feasible by 2030~\cite{Litman2015AutonomousVI}. An autonomous vehicle's software stack consists of three components~\cite{paden2016survey,pendleton2017perception}: perception, planning, and control (\figref{fig:netd_arch}).

% autonomous driving technologies such as adaptive cruise control and auto-steering are starting to be widely available in newer vehicles. By some estimates~\cite{Litman2015AutonomousVI}, full autonomy may be available at a price premium by the 2030s, and will get progressively cheaper in the subsequent decades. 

%\parab{A brief introduction to autonomous driving.}

% Source for figure:
% https://docs.google.com/drawings/d/1Pg3iyiMpIJOLya6yZ3YwoCiSJr-JAOj-dPGkFWEHduI/edit


% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.9\columnwidth]{figs/fig_autonomous_driving_stack.pdf}
%   \caption{Self-driving stack}
%   \label{fig:av_stack}
% \end{figure}

\begin{mydescription}
\item[Perception] extracts a vehicle's surroundings, using one or more 3D depth-perception sensors (\eg radars, stereo cameras, and LiDARs). A LiDAR, for example, sends millions of light pulses 10 or more times a second in all directions, whose reflections enable the LiDAR to estimate the position of points on objects or surfaces in the environment. The output of a LiDAR is a 3D \textit{point cloud} that contains points with associated 3D positions (also true of stereo cameras). The perception module extracts an abstract scene description consisting of static and dynamic objects, from these point clouds. Static objects include road surfaces, lane markers~\cite{lanedetection}, and safe drivable space~\cite{drivablespace}. The module also identifies and tracks dynamic objects (vehicles, pedestrians, and cyclists).
\item[Planning] uses the abstract scene description from the perception component to plan and execute a safe path for the vehicle, while satisfying performance and comfort objectives~\cite{paden2016survey} (\eg smooth driving, minimal travel time \etc). Planning executes at the timescale of 100s of milliseconds and its output is a \textit{\textbf{trajectory}}~---~a sequence of way-points, together with the precise arrival times at those way-points.
\item[Control] takes a trajectory and converts it, at millisecond timescales, to actuator (\eg throttle, steering, brake) signals.
\end{mydescription}
 %Finally, it estimates the vehicle's own position, using SLAM (Simultaneous Localization and Mapping)~\cite{slam_part1,slam_part2} algorithms. 

% understand the scene around it, detect drivable space, and localize itself (\figref{fig:av_stack}). First, the module segments the scene it sees through its sensors into static and dynamic objects. For this, it can use semantic segmentation tools~\cite{DeepLab}, background subtraction~\cite{Octree}, and ground-plane extraction~\cite{groundplane} \etc. Then, it extracts the road surface, detects lane markers~\cite{lanedetection} and safe drivable space~\cite{drivablespace}. To localize the vehicle, the perception module matches \textit{features} in its point cloud with those in SLAM (Simultaneous Localization and Mapping)~\cite{slam_part1,slam_part2} generated \textit{3D maps}~\cite{CarMap}. The map contains the positions of the matched features, using which the vehicle can triangulate its own position.

% and are constructed from LiDARs or 
% cameras (multi-view stereo~\cite{colmap}).

% These maps are dense reconstructions of the physical world 
% around the vehicle and enable it to see beyond it's sensors' range.
% SLAM uses cameras~\cite{ORB-SLAM2} or LiDARs~\cite{LOAM} along 
% with other sensors (GPS) to precisely localize a vehicle by 
% tracking static features in its surroundings.   
% \ramesh{Do they use SLAM, or SLAM-generated maps? Also, consider whether this detail is important from the perspective of the story. Do we use SLAM anywhere else? If we only plan to make a passing reference, may introduce it there.}
% \fawad{I think it might be important because we will have a localization experiment later on and then we need to compare our approach with what autonomous vehicles have now.}

% 2.2 Control
\parab{\sysname: Infrastructure-directed Autonomous Driving.} Sometimes roadside compute and sensing infrastructure can \textit{augment} autonomous driving. In our approach (\sysname):

%\begin{itemize}[topsep=0pt,itemsep=-1ex,partopsep=0ex,parsep=1ex,leftmargin=*]
\begin{itemize}[nosep,wide]
\item \textit{\textbf{roadside}} LiDARs\footnote{Roadside LiDAR deployments exist in several places~\cite{roadlidar1,roadlidar2,roadlidar3}.} have an unobstructed view of the roadway and continuously perceive intersection dynamics. \sysname feeds LiDAR outputs to its stack running on \textit{\textbf{edge compute}} (\figref{fig:netd_arch}) at or near the intersection.
\item \sysname's perception module produces a continuously updated abstract scene description from the LiDARs.
\item Its planning module plans trajectories for all autonomous vehicles, then transmits trajectories wirelessly (\eg over \textbf{\textit{5G}}) to the autonomous vehicle, which feeds that trajectory to its control module (\figref{fig:netd_arch}).
\end{itemize}

Thus, \textit{when \sysname infrastructure is available, autonomous vehicles use \sysname's trajectories, else they use trajectories generated by their on-board planner}. \sysname is fast becoming technically feasible because LiDARs are becoming cheaper~\cite{sslidars,huawei_lidar}, and  5G~\cite{5g,Qualcomm5g,Ericsson} and edge computing~\cite{ibmedge} are seeing rapid ongoing deployment.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.70\columnwidth]{figs/NetDriving_arch4.pdf}
  \caption{Autonomous vehicles run perception, planning and control on-board.  \sysname augments autonomous driving; it runs perception and planning on edge-compute infrastructure, and transmits trajectories directly to the vehicle's control module.}
  \label{fig:netd_arch}
\end{figure}

\sysname can help improve \textbf{\textit{safety}} and traffic \textbf{\textit{throughput}} at intersections. Annually, in the US, about 2.5 million accidents occur at intersections, which contribute to 50\% of all serious accidents and 25\% of fatalities~\cite{intersection-accidents}. As such, intersections are a focus area for the US Federal Highway Administration (FHWA)~\cite{intersection_safety} with programs that improve current intersection designs and explore safer alternatives. Intersection safety is a challenge problem for autonomous vehicles as well~\cite{carlachallenge} because of line-of-sight limitations~\cite{AVR}. In addition, wait times at intersections in major metropolitan areas can be significant, and higher traffic throughput can result in reduced wait times. A recent report~\cite{intersection-wait} estimates that drivers in California spend, on aggregate, 2.7M hours in a 24-hour period waiting at intersections!

\sysname has two properties to address these problems:

%\begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=0ex,parsep=1ex,leftmargin=*]
\begin{enumerate}[nosep,wide]
\item LiDARs mounted at each corner of an intersection above car heights can get a comprehensive view of all vehicles and traffic participants at an intersection (\figref{fig:netd_arch}). This improved perspective can help overcome safety issues caused by line-of-sight limitations. Consider \figref{fig:sys_overtaking}, which illustrates a common and deadly safety issue at intersections: \textit{\textbf{red-light violations}}, which account for 700-800 fatalities in the US annually~\cite{intersection-accidents}. In this figure, the yellow vehicle's view of the red-light violator (the blue car) is blocked by a red truck. This scenario is known to be challenging for autonomous vehicles~\cite{carlachallenge} as well. \sysname, because it notices the blue car, can generate a trajectory for the yellow vehicle to cause it to slow down, and avoid a collision. 
\item Because it \textit{jointly} plans trajectories for all autonomous vehicles, at an intersection, \sysname can increase traffic throughput and even enable \textbf{\textit{traffic-light free intersections}}~\cite{traffic-light-free}. To see why, consider the same scenario as in \figref{fig:sys_overtaking}, but now suppose that all vehicles are autonomous. Also suppose there are no traffic lights at the intersection. Then, as the vehicles arrive, \sysname can develop trajectories that slow down the blue car or speed up the red truck and the yellow car (or both), so that all cars can safely traverse the intersection. More important, joint trajectory planning is \textit{necessary} to achieve this capability. If \sysname had only offloaded perception to infrastructure (which provides comprehensive views of traffic analogous to cooperative perception in AVR~\cite{AVR}, EMP~\cite{emp}, VI-Eye~\cite{vieye}, and VIPS~\cite{vips}), and left it to vehicles to plan trajectories based on its scene description, traffic can  \textit{deadlock} (\secref{s:high-thro-traff}), resulting in \textit{\textbf{zero throughput}}.
\end{enumerate}

%\ramesh{Please update \figref{fig:sys_overtaking}.}

% For example, \sysname could instruct the oncoming vehicle in \figref{fig:sys_overtaking} to slow down enough to allow the blue vehicle to pass (\secref{s:planner}). Doing so might help both vehicles make progress faster than if the blue vehicle waited for the oncoming vehicle pass, thereby increasing throughput. More generally, \sysname can enable long-desired transportation innovations, such as \textit{traffic-light free intersections}~\cite{traffic-light-free}\footnote{Much work in transportation research focuses on traffic management at intersections, since these are potential choke points in traffic flow (the same reason that much networking research focuses on router designs).}. At an intersection without traffic lights, \sysname can jointly plan the trajectories of all vehicles so that they may safely pass through the intersection with lower wait times (or higher overall throughput). %\ramesh{Revisit last sentence after getting results of experiments.}

% In \figref{fig:sys_overtaking}, a blue vehicle wishes to pass a stationary red vehicle but there is an oncoming vehicle in the opposite lane. This scenario is challenging for autonomous vehicles~\cite{Carla} and for human drivers. In \sysname, roadside LiDARs convey (\figref{fig:sys_overtaking}) point-clouds to \sysname's perception component running on edge compute\footnote{We assume that because LiDARs are statically deployed on infrastructure, they have wired connectivity. Wirelessly streaming compressed LiDAR data can ease deployment, but we have left this to future work.}. This component analyzes the scene, and 

% In this paper, we explore a \textit{\textbf{different point in the design space}} of autonomous driving, an approach we call \sysname. In \sysname, components in the network remotely ``drive'' vehicles (\figref{fig:netd_arch}(b)), hence the name. Three technology trends motivate \sysname. \textit{\textbf{5G}}, the fifth generation of cellular network technology~\cite{5g,Qualcomm5g,Ericsson}, promises gigabit speeds and latency as low as 1~ms. Vehicle manufacturers are standardizing 5G technologies like CV2X~\cite{QualcommCV2X} and LTE Direct~\cite{LTEDirect} for cooperative perception, path-planning, and control. At the same time, \textit{\textbf{edge-computing}} is moving computational resources (both CPU and GPU~\cite{nvidiaedge}) closer to data sources to support latency-critical applications~\cite{ibmedge}. By some estimates, edge-servers will handle 75\% of the processing workloads handled by the cloud today~\cite{edgegartner}. 
% Finally, \textit{\textbf{LiDAR prices}} are falling dramatically due to competition and improved technology and manufacturing. A typical 64-beam LiDAR~\cite{Ouster,Velodyne} today costs a few thousand dollars. In the next few years LiDARs will likely cost a few hundred dollars~\cite{sslidars,huawei_lidar}.

% \sysname \textit{decouples perception and planning from control\footnote{Control effects actuators using sub-millisecond control loops, so must remain in-vehicle.}} and offloads them to road-side infrastructure. \sysname's perception component fuses data from multiple infrastructure-mounted sensors to develop scene understanding, and its planning component generates trajectories for all vehicles in view of the sensors. It  continuously transmits, over wireless, these trajectories back to vehicles, which simply follow these planned trajectories.

% \parab{How \sysname works.}
% These trends motivate \sysname's design, in which LiDARs are cheap enough to mount ubiquitously on roadside light poles; edge-compute infrastructure can process LiDAR data in near real-time; and 5G can convey the results of that processing to vehicles in milliseconds. Thus, \sysname offloads \textit{perception and planning} to roadside infrastructure (\figref{fig:netd_arch}(b)); control remains on-board because it involves tight sub-millisecond feedback loops.

% % Source for figure: https://docs.google.com/drawings/d/1eW5kuEXE6dO-kTs-xECv2STZYocAbkAxDfSgDs0zPsk/edit
% % Overview of NetDriving
% % - use a picture/scenario to maybe take one of the CarLA challenge problems (the single lane overtaking one)

% % \ramesh{Put figure before parab; otherwise heading doesn't show up correctly.}
% % \parab{Overview of \sysname.}
% % Show that today's approaches would find difficult
% % \fawad{I think we can comment out the following paragraph which shows how today's approaches will tackle this problem. It might be sufficient to just say how autonomous vehicles will tackle it} \ramesh{Sounds good, but autonomous vehicles might do roughly the same without AVR. Also, perhaps pick an intersection challenge from CarLA if there is one? Make sure to point out that this is from the CarLA challenge, not something we're making up.}
% In \figref{fig:sys_overtaking}, a blue vehicle wishes to pass a stationary red vehicle but there is an oncoming vehicle in the opposite lane. This scenario is challenging for autonomous vehicles~\cite{Carla} and for human drivers. In \sysname, roadside LiDARs convey (\figref{fig:sys_overtaking}) point-clouds to \sysname's perception component running on edge compute\footnote{We assume that because LiDARs are statically deployed on infrastructure, they have wired connectivity. Wirelessly streaming compressed LiDAR data can ease deployment, but we have left this to future work.}. This component analyzes the scene, and outputs an abstract scene description containing vehicles and pedestrians, their velocities and heading. Using these, \sysname's planner determines that the oncoming vehicle is far enough away for the blue vehicle to pass safely. It generates a trajectory for the blue vehicle, and transmits the trajectory over wireless to the vehicle (this is where \sysname needs 5G's low latency), whose control component effects the trajectory. %To address this challenge, prior work has proposed other approaches such as directly sharing sensor readings between vehicles~\cite{AVR}, discussed in \secref{sec:related_work}.

% \parab{Why consider \sysname?} \figref{fig:sys_overtaking} highlights two advantages of \sysname. First, well-placed infrastructure sensors can perceive more of the environment than in-vehicle sensors; in our example, a LiDAR mounted on the blue vehicle cannot see the oncoming vehicle because of the line-of-sight limitations. This can potentially \textit{\textbf{increase safety}}, because \sysname generates vehicle trajectories based on more complete information than in autonomous driving.

% https://docs.google.com/drawings/d/1ZGnU4q1_y-GV4lyx4Rle0qpW7wb_FYLNA4ZLAnlxue0/edit
% Second, \sysname can \textbf{\textit{increase traffic throughput}}. If every vehicle were \sysname capable, then \sysname's planner could jointly plan safe trajectories for all vehicles in the scene and optimize roadway utilization. For example, \sysname could instruct the oncoming vehicle in \figref{fig:sys_overtaking} to slow down enough to allow the blue vehicle to pass (\secref{s:planner}). Doing so might help both vehicles make progress faster than if the blue vehicle waited for the oncoming vehicle pass, thereby increasing throughput. More generally, \sysname can enable long-desired transportation innovations, such as \textit{traffic-light free intersections}~\cite{traffic-light-free}\footnote{Much work in transportation research focuses on traffic management at intersections, since these are potential choke points in traffic flow (the same reason that much networking research focuses on router designs).}. At an intersection without traffic lights, \sysname can jointly plan the trajectories of all vehicles so that they may safely pass through the intersection with lower wait times (or higher overall throughput). %\ramesh{Revisit last sentence after getting results of experiments.}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.6\columnwidth]{figs/red_violation_intro.pdf}
  \caption{In \sysname, roadside LiDARs transmit data over a wired network to an edge cluster. \sysname's perception extracts vehicles and their motion information, and its planning component determines that the blue vehicle can safely pass the stalled vehicle. \sysname wirelessly delivers a trajectory designed for the blue vehicle, whose control component executes the trajectory.}
  \label{fig:sys_overtaking}
%   \fawad{Note to self: replace this with a figure that shows infra sensors as well}
\end{figure}

% \parab{Deployment considerations.} \sysname departs significantly from existing autonomous driving designs, so its full deployment will take time.\footnote{However, if/when \sysname is fully deployed, it can simplify autonomous driving: vehicles will no longer need expensive sensors thereby reducing cost~\cite{qzvehiclecost,reutersvehiclecost}, nor power-hungry on-board compute~\cite{lin18:_archit_implic_auton_drivin}, nor expensive high-definition maps~\cite{3dmapcost}.}
% \sysname can, however, be \textit{incrementally} deployed, with initial deployments in areas with high traffic congestion: streets downtown, intersections, ports \etc. In these areas, \sysname can improve traffic flow without compromising safety. For example, at a busy intersection, a \sysname deployment might consist of four LiDARs mounted at light poles. As cars approach, they switch to following trajectories generated for them by \sysname (as for the blue car in \figref{fig:sys_overtaking}). In such a setting, \sysname is safer than autonomous driving and can effect safe passage of vehicles without traffic lights (as we show in \secref{s:bett-traff-manag}). Even in these deployments, much work is necessary; cost/benefit economic analyses, public-private partnerships to install infrastructure, regulatory approvals, buy-in from vehicle owners, \etc. We have left these to future work; we focus on understanding technical feasibility and potential benefits.

%We have left to future work to consider partial deployment strategies, perform an economic analysis of these deployment strategies, explore how to form public-private partnership to install infrastructure \etc In this paper, we focus on the feasibility of \sysname: we design and implement perception and planning components that meet performance requirements for autonomous vehicles described above, namely, to be able to process LiDAR frames at full frame rate and within 100~ms.


% Technological changes have often spurred architectural shifts that have fundamentally altered the placement of functionality across a network. Some of these architectural shifts change the way the network itself works or is managed. A good example is software-defined networking (SDN), which de-couples the network's control plane from its data plane. Other architectural shifts change the design of applications and systems that use the network. For example, the advent of cloud computing inspired a class of cloud-enabled mobile applications that offload compute and storage for enhanced user experience. 

%\parab{What is \sysname?}
%In this paper, we explore an impending architectural shift in how self-driving vehicles use the network, a shift that resembles SDN. Today, self-driving vehicles use expensive sensors (like LiDARs) and run a software stack with three components (\figref{fig:netd_arch}(a)): \textit{perception} for scene understanding, trajectory \textit{planning}, and actuator \textit{control} to realize planned trajectories (\secref{sec:background}). This stack runs on-board the vehicle (\secref{sec:background}); if today's self-driving vehicles use the network at all, it is for over-the-air upgrades, and analytics uploads.

%The drop in prices of sensors~\cite{sslidars,memslidar,huawei_lidar}, the increased deployment of edge computing~\cite{nvidiaedge,ibmedge,edgegartner}, and the rollout of 5G-based vehicular connectivity~\cite{amazon_edge,Qualcomm5g,5g} suggest an architectural shift that we call \sysname, in which components in the network remotely ``drive'' vehicles. \sysname \textit{decouples perception and planning from control\footnote{Control effects actuators using sub-millisecond control loops, so must remain in-vehicle.}} and offloads them to road-side infrastructure (\figref{fig:netd_arch}(b)). \sysname's perception component fuses data from multiple infrastructure-mounted sensors to develop scene understanding, and its planning component generates trajectories for all vehicles in view of the sensors. It continuously transmits, over wireless, these trajectories back to vehicles, which simply follow these planned trajectories (\secref{sec:architecture}).


% \parab{Resemblance to SDN.}
% This resembles the decoupling of control and data planes in SDN (\figref{fig:netd_arch}(c)). In SDN, the logically-centralized control plane programs switches to direct traffic flows. Armed with a global view of the network, it can enable higher network utilization~\cite{B4,SWAN} and provide better abstractions for controlling network traffic~\cite{pyretic}.

% Similarly, \sysname ``programs'' vehicle trajectories. Armed with a more complete view than a single vehicle, it can potentially ensure higher safety, better vehicular traffic throughput using long-desired transportation innovations (\eg platooning~\cite{platooning2011} and traffic-light free intersections~\cite{traffic-light-free}), and maybe even better abstractions for customizable traffic policies. This is because: (a) \sysname's perception fuses multiple sensors, it can see more than sensors mounted on a single vehicle\footnote{Sensors used for perception have line-of-sight limitations. A vehicle may not be able to see those oncoming vehicles in the opposite lane that are obstructed by the vehicle in front of it (\secref{sec:background}).}, resulting in increased safety; (b) because the planner can jointly plan trajectories for multiple vehicles.

\parab{\sysname Challenge.} \sysname has stringent bandwidth, latency,  accuracy and robustness requirements, and it must be possible to meet these requirements on commodity hardware deployed on edge computing infrastructure.

%\begin{itemize}[topsep=0pt,itemsep=-1ex,partopsep=0ex,parsep=1ex,leftmargin=*]
\begin{itemize}[nosep,wide]
\item LiDARs generate data at 10 frames per second. At 30~MB per frame, this translates to a \textit{\textbf{raw data rate of nearly 10~Gbps}} for four LiDARs at an intersection. LiDARs can have wired network connections so the network is unlikely to be a bottleneck, but extracting scene understanding from voluminous data can stress compute.
\item \sysname must produce trajectories within a tight latency (time taken to run a single frame from each LiDAR through its perception and planning) constraint. Industry players like Udacity~\cite{udacity}, Mobileye~\cite{mobileye, shalevshwartz2018formal}, and Tesla~\cite{tesla} argue that autonomous vehicles must make decisions \textit{\textbf{with a tail latency of less than 100~ms}}. Other work exploring autonomous driving also suggests the same constraint~\cite{lin18:_archit_implic_auton_drivin}.
\item \sysname generates scene descriptions which consist of objects, their tracks, positions, heading, and speed. The accuracy of these must \textbf{\textit{match or exceed the SOTA}}.
\item \sysname transmits trajectories wirelessly, and this must be robust to packet losses.
\end{itemize}

\begin{table}[t]
  \footnotesize
  \centering
  \begin{tabular}{c|c|c||c|c|c} \hline
      \textbf{Strategy} & \textbf{Prcp} & \textbf{Plan} & \textbf{Perf} & \textbf{Sfty} & \textbf{Tput} \\ \hline \hline
      AVR~\cite{AVR} & V2V & OB & \questmk & \crossmk & \crossmk \\ \hline
      EMP~\cite{emp} & V2I & OB & \questmk & \crossmk & \crossmk \\ \hline
      VIPS~\cite{vips} & I-V & OB & \questmk & \crossmk & \crossmk \\ \hline
      VI-Eye~\cite{vieye} & I-V & OB & \crossmk & \crossmk & \crossmk \\ \hline
      Autocast~\cite{autocast} & V2V & OB & \checkmk & \checkmk & \crossmk \\ \hline
      \sysname & I & I & \checkmk & \checkmk & \checkmk \\ \hline
  \end{tabular}
  \caption{\textbf{Prcp} and \textbf{Plan} refer to perception and planning respectively.
  V2V, I-V, and I in \textbf{Prcp} refer to vehicle-to-vehicle, infrastructure-to-vehicle and infrastructure cooperative perception respectively.
  OB and I in \textbf{Plan} refer to on-board and infrastructure planning respectively.
  \textbf{Perf} refers to achieving 100~ms end-to-end tail latency. A \textbf{?} in this column suggests that the work has partially benchmarked performance (\eg only perception) and this is within 100~ms. \textbf{Sfty} indicates whether the work has demonstrated safety in evaluations, and \textbf{Tput} indicates whether the work has demonstrated throughput in evaluations. We show that, in certain cases, cooperative perception can result in deadlock, resulting in poor throughput.}
  \label{tab:comprel}
\end{table}

It is not immediately obvious that \sysname can meet these requirements; for instance, the most accurate 2D and 3D object detectors on the KITTI leaderboard~\cite{geiger2013vision} incur a processing latency of 60-300~ms!


% This is challenging to do because these sensors produce voluminous data (several hundred Gbps) and accurately extracting scene understanding and planning trajectories from these within a tight latency budget requires algorithmic innovations and the judicious use of hardware acceleration.

% \parab{How \sysname Addresses the Challenge.} \sysname's stack is qualitatively different from those of open-source autonomous driving stacks like Autoware~\cite{Autoware} and Baidu's Apollo~\cite{BaiduSpecs} (\tabref{tab:stack_comparison}), and exploits domain-specific properties. It does not require pre-built HD maps for positioning, but estimates positions of vehicles and traffic participants using \textit{composite views} obtained from outputs of individual static LiDARs. Instead of operating on every LiDAR separately, \sysname combines point clouds from multiple LiDARs early on in its processing pipeline. This early fusion enables robust and cheap \textit{3D object detection} (unlike other stacks that detect obstacles or use 2D camera-based object detection). \sysname's object detector outputs tight bounding boxes for participants; this abstraction is used extensively to accurately, yet cheaply, track and estimate the motion of vehicles (\secref{sec:perception}). \sysname also uses a novel, GPU-accelerated, heading detection algorithm; simpler approaches have large errors in the tail.

% Its planner (\secref{s:planner}) jointly plans trajectories for multiple vehicles using perception outputs. It adapts prior work in distributed robotic motion planning~\cite{SIPP} to support vehicles of different sizes as well as \sysname-oblivious participants (\eg pedestrians or legacy vehicles), to be robust to packet loss, and adds vehicle kinematic constraints (like stopping distances) and driving experience constraints (like safe driving distances). Other stacks use comparable planners, but only plan for the ego vehicle (\tabref{tab:stack_comparison}).

\parab{Contributions.} To address these challenges, we make the following contributions:
%\begin{itemize}[topsep=0pt,itemsep=-1ex,partopsep=0ex,parsep=1ex,leftmargin=*]
\begin{itemize}[nosep,wide]
\item \sysname incorporates a novel stack for perception and planning, which is qualitatively different from existing autonomous driving stacks (\secref{sec:perception}).
\item Its perception pipeline fuses multiple LiDAR outputs using a novel alignment algorithm whose accuracy is significantly higher than prior work (\secref{s:fusion}).
\item Accurate alignment enables fast and cheap implementation of object extraction, tracking, and speed estimation, all centered around a single bounding box abstraction computed early in the pipeline (\secref{s:part-extr}).
\item Cheap algorithms for heading estimation are inaccurate, so \sysname develops a more accurate GPU-offload heading estimator to meet the latency constraint (\secref{s:tracking}).
\item \sysname adapts an existing single-robot motion planner to jointly plan trajectories for multiple vehicles, to account for real-world non-idealities, and wireless packet loss (\secref{s:planner}).
\end{itemize}
  %\ramesh{Revisit this list later.}




\begin{table*}[t]
  \begin{small}
  \centering
\begin{tabular}{l|p{1in}|p{1.5in}|p{1.5in}|p{1.5in}}\hline
                  & & \textbf{\sysname} & \textbf{Baidu Apollo}~\cite{BaiduSpecs} & \textbf{Autoware}~\cite{Autoware} \\ \hline\hline
      \multirow{4}{*}{Perception} & Mapping & \textit{\textbf{None}} & Pre-built HD-Map & Pre-built HD-Map \\ \cline{2-5}
      & Localization & \textit{\textbf{Live Fused Point Cloud}} (\secref{s:fusion}) & LiDAR scan matching fused with GPS-RTK and IMU & LiDAR scan matching \\ \cline{2-5}
                   & Object detection & \textit{\textbf{3D Object Detection}} (\secref{s:part-extr}) & Obstacle detection in 2D BEV projection & 2D object detection in camera, projected to 3D \\ \cline{2-5}
                   & Tracking and motion estimation & Kalman filter with matching, \textit{\textbf{Heading Estimation}} (\secref{s:tracking}) & Kalman filter with matching & Kalman filter with matching \\ \hline\hline
    Planning & & \textit{\textbf{Centralized Interval Planner}} (\secref{s:planner}) & Ego-planner using hybrid A$\star$ search & Ego-planner using conformal lattices \\ \hline               
    \end{tabular}
  \caption{\sysname uses a qualitatively different stack to meet throughput and latency requirements. Both perception and planning use different algorithms (highlighted in bold) than existing open-source stacks.}
  \label{tab:stack_comparison}
  \end{small}
\end{table*}

\parab{Summary of Results.}
Evaluations on a testbed, a deployment at a busy intersection in a large metropolitan city, and on a photorealistic autonomous driving  simulator~\cite{Carla} validate these contributions and demonstrate its superiority relative to today's autonomous driving and to cooperative perception (\secref{sec:evaluation}). \sysname achieves its performance objectives end-to-end, being able to process frames from 4 LiDARs at 10~fps with a 99-th percentile tail latency under 100~ms. Its perception component can track vehicles to centimeter-level accuracy (comparable to SLAM~\cite{LOAM}-based positioning). Its planner ensures safe passage in all red-light violation and unprotected left-turn scenarios, while autonomous driving can do so only 27\% of the time. It can reduce wait times 5$\times$ at intersections relative to intelligent traffic lights; in contrast, cooperative perception (\eg~\cite{AVR,autocast,emp}) can result in deadlock.

% \sysname is inspired by recent and planned roadside deployments of advanced sensors, and a large body of work on augmenting connected autonomous driving vehicle perception using infrastructure-based sensors (\secref{sec:related_work}). To our knowledge, no prior work has considered combining infrastructure-based perception and planning~---~\sysname demonstrates the end-to-end viability of such a capability.

\parab{Related Work.}
\sysname falls into a qualitatively different point in the design space relative to the most closely related prior work (\tabref{tab:comprel}); it is the first to explore completely moving perception and planning to the infrastructure. It is also the first to consider safety \textbf{\textit{and}} throughput. Several pieces of work have considered various forms of \textit{cooperative perception}. AVR~\cite{AVR} and Autocast~\cite{autocast} use vehicle-to-vehicle cooperative perception, EMP~\cite{emp} uses edge compute infrastructure, whereas Vi-Eye~\cite{vieye} and VIPS~\cite{vips} in addition uses infrastructure sensors. All of these approaches rely on \textbf{\textit{on-board planning}}. Of these, only Autocast~\cite{autocast} demonstrates end-to-end performance (including perception and planning) and safety, but does not evaluate throughput. In this paper, we show that even with comprehensive views of traffic (as with cooperative perception), on-board planning can result in zero throughput in some cases due to deadlock.

% There is a body of work that improve a vehicle's on-board (ego) perception by augmenting it with sensory data from surrounding vehicles (\eg AVR~\cite{AVR}, EMP~\cite{emp}, and Autocast~\cite{autocast}) or infrastructure sensors (VI-eye~\cite{vieye}). Because this alleviates the line-of-sight limitations of the 3D sensors, it enables safer driving and helps vehicles navigate challenging scenarios like \figref{fig:sys_overtaking}. Though this improves safety, it does not improve traffic efficiency because autonomous vehicles still use on-board planning. \sysname is an extreme point in this entire design space (\figref{fig:comprel}) because it moves both perception and planning from the ego vehicle to the infrastructure. By doing so, it enables the possibility of a centralized planner for all vehicles and thus in turn enables both safer, and more efficient autonomous driving. To our knowledge, no prior work has considered combining infrastructure-based perception and planning~---~\sysname demonstrates the end-to-end viability of such a capability.

% 3D sensors that are prone to line-of-sight limitations. As a result, they fail to navigate scenarios like \figref{fig:sys_overtaking}. There is a body of work that alleviates this problem through cooperative perception (vehicle-to-vehicle or vehicle-to-infrastructure)
% Source for figure:
% https://docs.google.com/presentation/d/1QO930yIamtt41R3ZG-UADbBcx9-ULgOd9yanbMKX3tg/edit#slide=id.p

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.7\columnwidth]{figs/fig_netdriving_design_space.pdf}
%   \caption{\add{\sysname explores an extreme space in the autonomous driving design space by offloading perception and planning to the infrastructure.}}
%   \label{fig:design_space}
% %   \fawad{Note to self: replace this with a figure that shows infra sensors as well}
% \end{figure}
% \ramesh{Note to self: Add section numbers to cells in \tabref{fig:stack_comparison}.}

% Introduction:
% - Architectural innovation driven by functional de-coupling
%   - Control-data separation in networks
%   - Other examples
%   - Position: de-coupling sensing and actuation can have significant benefits for autonomous driving




==> intro_sensys.tex <==
\section{Introduction}
\label{sec:intro}

% Outline
% Title: Fast Infrastructure-Based Cooperative (?) Perception Using LiDARs
% - Enables a new sensing capability
% - startups are starting to look at, albeit in more restrictive settings like parking garages etc.
% - edge compute and high bandwidth wireless etc.
% - use case
    % - to augment vehicular perception
    % - plan vehicles
    % - assist pedestrians in public space

% - requirements/challenges
% - brief summary of related work

% Enabling a new sensing capability
    % What is the sensing capability
        % Fast perception for large public spaces with multiple LiDARs
        % Ability to accurately monitor dynamic objects in large public spaces with low latency
        % By monitor, we mean accurately position, and estimate the motion of
        % Dynamics can be pedestrians, motorcyclists, and vehicles etc
    % How do you enable it
        % Using multiple 3D sensors mounted at public spaces
        % Edge compute

This paper introduces a novel sensing capability, \sysname, that uses multiple infrastructure-mounted LiDARs to enable real-time collaborative perception at large public spaces.
Using a set of LiDARs installed in public spaces (\eg intersections, plazas, and shopping malls \etc), \sysname identifies dynamic objects (\eg pedestrians, cyclists, vehicles), and tracks their motion in real-time (\figref{fig:deployment}).
To do this, \sysname continuously fuses 3D frames from multiple LiDARs into a single coordinate system to build a live 3D fused view.
Then, it utilizes this fused 3D frame to detect and track dynamic objects across consecutive frames in real-time.

% Why is this sensing capability possible now as opposed to before?
    % LiDAR prices are starting to come down, which enables deploying them widely in public spaces
    % Edge compute is starting to become more ubquitious which enables processing the intensive 3D data
    % Low latency 5G enables transfer of the 3D data or the processed results quickly

Three technology trends motivate \sysname.
In the next few years, with solid-state LiDARs~\cite{sslidars,memslidar,huawei_lidar}, the per-unit cost of LiDARs is expected to down to several hundred dollars.
This enables deploying them ubiquitously in public places to perceive the world in three dimensions, at scale.
Edge compute deployments~\cite{nvidiaedge,ibmedge,edgegartner,amazon_edge} will place powerful compute in proximity with these LiDARs.
Finally, 5G deployments~\cite{Qualcomm5g, 5g} enable high bandwidth and low latency wireless connections.
This enables seamless and low latency transport of 3D data.
Put together, these trends motivate \sysname, the capability to collaboratively perceive large public spaces with multiple LiDARs in real-time.


% Industry interest
    % Industry starting to look at similar capabilities but in more restrictive spaces
    % Seoul robotics uses this capability in parking garages as a means of last mile autonomy
These trends have also instilled interest in the industry in exploring similar capabilities, albeit in more restrictive spaces.
Seoul Robotics~\cite{seoulrobotics} offloads sensing, and computations from vehicles to the infrastructure to provide last mile autonomy for self-driving cars.
To do this, in restrictive places like parking lots and garages for malls and airports, Seoul Robotics installs a rich sensor suite consisting of LiDARs and cameras along with edge compute.
Using these sensors, their Level 5 Control Tower creates an obstructed view of the parking lot.
It then uses edge compute to run fast perception, and planning algorithms to process the 3D data, and guide vehicles to and out of their parking spaces.
\christina{What would be our novelty/contribution compared to this Seoul Robotics usecase? or we may need to emphasize any limitation on this case too.}
\fawad{This example further motivates the need for \sysname. Because their system is proprietary, there is no way for us to compare with it except say that it is used in restrictive spaces.}
% Why is this capability useful
    % For extending a vehicle's perception range (show an example)
    % For collaborative planning
    % To assist pedestrian in public spaces
The ability to do real-time perception from fused LiDAR views in large public spaces finds applications in a number of other use cases.
When shared with an autonomous vehicle, the perception results can be fused with the vehicle's on-board perception to improve its understanding of the environment.
By doing so, the vehicle can see beyond its sensor range, and enable it to make safer driving decisions.
At traffic intersections, real-time perception can be fed into a centralized planner located at the intersection.
% results can be fed to a centralized planner.
This centralized planner can jointly plan collision-free trajectories for all vehicles.
This enables a long sought after transportation goal \ie traffic light free intersections~\cite{traffic-light-free}, thus improving overall traffic throughput.
For pedestrians, such a capability will improve their situational awareness of their surroundings.


\begin{figure}[t]
  \centering
  \includegraphics[width=0.95\columnwidth]{figs/fig_deployment_diagram.pdf}
  \caption{\sysname deployment at an intersection with multiple LiDARs, and nearby edge compute.}
  \label{fig:deployment}
\end{figure}

% What are the requirements/challenges set by these use cases?
    % Output required by these use cases are a live scene understanding
    % Scene understanding constitutes: a) positions, b) motion vectors of dynamic objects
    % Requirements are: accuracy, and latency
    % accuracy must be cm-level
    % latency be must less than 100~ms (99th percentile)
    % Do so using existing hardware (COTS)

\parab{Challenges. }
The use cases described above set stringent latency and accuracy requirements for \sysname which must run on commodity hardware deployed on edge computing infrastructure.

\begin{itemize}[nosep,wide]

\item Autonomous vehicles must perceive the world, and make driving decisions at a frequency of 10~Hz with a tail latency less than 100~ms~\cite{udacity, mobileye, lin18:_archit_implic_auton_drivin}. 
To be applicable to autonomous driving, \sysname must also adhere to the same latency constraints. 
LiDARs generate data at 10 frames per second. 
At 30~MB per frame, with four LiDARs at an intersection, this translates to \sysname having to process data at a \textit{\textbf{raw rate of nearly 10~Gbps}}.
With COTS compute, this is not straightforward.

\item \sysname perception generates a scene description that consists of dynamic objects along with their positions, bounding boxes, heading vectors and motion vectors.
The accuracy of these must \textbf{\textit{match or exceed the state-of-the-art computer vision algorithms}}.
\end{itemize}

It is not immediately obvious that \sysname can meet these requirements; for example, the most accurate 2D and 3D object detectors on a popular autonomous driving benchmark~\cite{geiger2013vision} incur a processing latency of 60-300~ms.


% Contributions
    % Novel perception pipeline with:
        % Accurate alignment
        % Reuse of bounding boxes
        % Fast heading vector estimation
    % Demonstrate efficacy in use cases
\parab{Contributions. }
To address these challenges, \sysname incorporates a novel perception stack, in which we make the following contributions:

\begin{itemize}[nosep,wide]

\item To fuse 3D frames from multiple LiDARs, \sysname introduces a novel alignment algorithm whose accuracy is significantly higher than prior work (\secref{s:fusion}).

\item With an accurate 3D fused view, \sysname introduces fast and cheap implementations of algorithms for dynamic object extraction, tracking, and speed estimation. These are centered around a single bounding box abstraction which \sysname computes early on in the pipeline (\secref{s:part-extr}).

\item Cheap algorithms for heading estimation are inaccurate, so \sysname develops a more accurate GPU-offload heading estimator to meet the latency constraint (\secref{s:tracking}).

\item Finally, we demonstrate the effectiveness of this novel sensing capability by applying \sysname to two use cases in autonomous driving \ie improving safety, and improving traffic throughput.

\end{itemize}

% Recent work
    % Infrastructure-based perception
        % VI-Eye, and VIPS extend perception of a vehicle but leave processing to the vehicle
    % What else?
Recent work in autonomous driving has explored cooperative perception to extend a vehicle's sensing range in a bid to make safer driving decisions.
In these, some works have explored sharing raw or processed 3D frames amongst vehicles~\cite{AVR, autocast, emp}.
Whereas others, perhaps more related to \sysname, have explored augmenting a vehicle's perception with 3D frames from sensors mounted on road-side infrastructure~\cite{vieye, vips, he2022automatch}.
In these works, the focus is on 3D and 2D frame alignment, \ie accurately positioning the infrastructure sensor's frame with the vehicle's frame.
\sysname, on the other hand, further pushes the envelope by not only aligning multiple infrastructure LiDARs, but also enabling real-time perception on the fused 3D frames.
To the best of our knowledge, this is the first work to demonstrate such a capability.




==> optimization.tex <==
\section{Optimization}
\label{sec:optimization}

\subsection{GPU Accelerated ICP}

ICP becomes a bottleneck in \sysname's real-time processing pipeline. While using PCL's ICP implementation and maximum allowed number of iteration to be 100, registering a point cloud of 1500 points to another point cloud of 1500 points takes about 177ms. This has exceeded \sysname's latency requirement. While we can relaxed the the stopping criteria to allow the ICP to exit earlier and reduce the latency, this approach make compromise between accuracy and latency. 

The recent improvement in Graphic Processing Unit(GPU) enables fast computation of large amount of data in many fields. \sysname exploits the parallelizable structure of ICP and uses GPU to accelerate the ICP computation, while maintain the same level of accuracy of PCL's CPU implementation. Table \ref{tab:icp_time_compare} shows that \sysname ICP implementation is about 60-70x faster than PCL ICP implementation.

Parallel reduction kernel. Brute force but fast.

We transplanted PCL's ICP implementation to a GPU implementation written in CUDA. Each iteration of PCL's ICP implementation can be viewed as the following steps.
\begin{itemize}
    \item Correspondence Estimation between source and target cloud
    \item Transformation Estimation between source and target cloud
    \item Transform the source cloud by the estimated transform matrix
    \item Check whether the ICP has converge
\end{itemize}

\parab{Correspondence Estimation} By default, the correspondence estimation is achieved by nearest neighbor search. For each point $p$ in the source cloud, the nearest point of $p$ in the target cloud $q$ will be found, and ICP draws the correspondence between $p$ and $q$. We initially implemented the nearest neighbor search by PCL's GPU implementation of Octree. Because searching in an octree is a iterative process, it becomes a major bottleneck of our implementation. The parallelizable structure of the the nearest neighbor search enabled us to use parallel brute-force algorithm to calculate a pairwise distance matrix and perform reduction to find the nearest neighbor. \sysname uses a parallel brute-force distance calculation suggested by \cite{garcia2008fast} to get the distance matrix.  However, \cite{garcia2008fast} uses a modified insertion sort to find the nearest neighbor for each query point based on the distance matrix. The modified insertion sort is a linear reduction cuda kernel that scan through each row of the distance matrix to find the nearest neighbor, and the scan is not parallelizable within each row(but parallelizable across rows). Instead, \sysname further optimizes the nearest neighbor searching by employing CUDA's parallel reduction functionality that enables parallel searches for the nearest neighbor in each row.

\parab{Transformation Estimation} For each point in the source cloud, correspondence estimation finds the corresponding point in the target point cloud. PCL's implememtation firstly shuffle the points in target cloud such that the corresponding points have the same index in both source and target points array. Then PCL uses Eigen Library's Umeyama function to calculate the transformation matrix. Eigen Library's Umeyama implementation includes a demean operation(subtract the centroid from both source and target cloud), a matrix multiplication, and a SVD computation. \sysname implements CUDA kernels to perform the shuffle operation(since it's also highly parallelizable) and implements Umeyma algorithm with a CUDA demean kernel, a cuBLAS matrix multiplication function call and a fast CUDA SVD computation for $3x3$ matrix implemented by \cite{gao2018gpu}. 

\parab{Point Cloud Transformation} The last step of each iteration of ICP is to transform the source point cloud by the estimated transformation. PCL's ICP iteratively goes through each point of the point cloud and apply the transformation matrix. \sysname implemented a CUDA kernel to transform all the points in parallel.

\parab{Convergence Checking} \sysname adopt the same kind of heuristic as PCL's ICP to determine whether the ICP has been converge or not. The only difference between \sysname's and PCL's implementation is that \sysname uses a CUDA kernel and parallel reduction to calculate the Mean Squared Error(MSE) between the transformed sourced cloud and the target cloud. 

\begin{table}[h]
\begin{small}


\begin{tabular}{|l|l|l|l|}
\hline
& Benchmark 1 & Benchmark 2 & Benchmark 3 \\ \hline
PCL CPU ICP & 177.66 ms   & 256.57 ms   & 70.93 ms \\ \hline
\begin{tabular}[c]{@{}l@{}}\sysname\\ (PCL's GPU Octree)\end{tabular} & 10.25 ms    & 11.85 ms    & 4.27 ms     \\ \hline
\sysname & 3.33 ms     & 4.27 ms     & 1.35 ms \\ \hline
\end{tabular}
\caption{Average ICP align time per frame.}
\label{tab:icp_time_compare}
\end{small}
\end{table}

\subsection{Planning}

\subsection{Other Optimizations}

\parab{Adopting effective data structures.} There are several data structures that are useful in managing point cloud data. For example, \textit{octree} is one of common structures in 3D data where it recursively partitions a given 3D space into eight cubes. \textit{k-d tree} is another common trees which divides a space in to two parts at every levels. Both tree structures are especially useful in point cloud comparison and neighbor searching because those operations can efficiently understand relationships between points. Firstly, \sysname adopts octree for \textit{background filtering}. Our algorithm constructs two octrees for a background point cloud and a target point cloud respectively. Then, it detects a difference between two octrees to extract vehicles from the target point cloud. Also, \textit{clustering} can be advantaged by utilizing the k-d tree. The k-d tree helps DBSCAN algorithm to efficiently explore reachable neighbors from a query point. By simply adopting suitable data structures, we are able to minimize an execution time while keeping a same accuracy level. 

\parab{Reordering in the perception module.} We can further optimize our pipeline by a reordering. Because execution time in our perception module largely depends on the size of data as well, it is better to minimize the point cloud size. Based on this observation, we run \textit{background filtering} first to filter out all unnecessary background points and reduce the data size, then do \textit{stitching}. In this way, we are able to largely reduce the execution time in stitching.
\christina{If necessary, we can put how much we can reduce.}

==> optimization_sensys.tex <==
\subsection{Optimizations}
\label{s:optimizations}

In this section, we describe our optimizations to \sysname.

\parab{Background Subtraction. }
\sysname removes points belonging to static parts of the scene\footnote{Static parts of the scene (e.g., an object on the drivable surface) might be important for path planning. \sysname uses the static background point cloud to determine the drivable surface; this is an input to the planner (\secref{s:centralized_planning}). We omit this for brevity.}. This is: a) especially crucial for voluminous LiDAR data, and b) feasible in our setting because LiDARs are static. It requires a calibration step to extract a \textit{background point cloud} from each LiDAR~\cite{kashani2015review}, then creates a \textit{background fused frame} using the results from alignment; taking the intersection of a few successive point clouds and the aggregating intersections taken at a few different time intervals, works well to generate the background point cloud.

%\weiwu{Can we mention here something like "Background is subtracted for tracking vehicle, but the planner can still use the full point cloud(to be informed any obstacles) for path planning."}

\parab{Subtraction before Stitching. }
\sysname subtracts the background fused frame from each fused frame generated by stitching. We have found that a simple optimization can significantly reduce processing latency: first removing the background from each LiDAR frame (using its background point cloud), and then stitching points in the residual point clouds. Stitching scales with the number of points, which this optimization reduces significantly.

\parab{Leveraging LiDAR Characteristics. } Many LiDAR devices only output \textit{returns} from reflected laser beams. Generic background subtraction algorithm requires a nearest-neighbor search to match a return with the corresponding return on the background point cloud. Some LiDARs (like the Ouster), however, indicate \textit{non-returns} as well, so that the point cloud contains the output of every beam of the LiDAR. For these, it is possible to achieve fast background subtraction by comparing corresponding beam outputs in a point cloud and the background point cloud.

%\parae{A performance optimization.}

At the end of these two steps, the fused frame only contains points belonging to objects that are not part of the scene's background (\figref{fig:intersection_example}(d)).

\parab{Computing 3D Bounding Boxes. }
On the points in the fused frame remaining after background subtraction, \sysname uses a standard, fast, clustering algorithm
(DBSCAN)~\cite{ester1996density} to extract multiple clusters of points, where each cluster represents one traffic participant. Then, it uses an off-the-shelf algorithm~\cite{pclbbox}, which determines
a minimum oriented bounding box (\figref{fig:intersection_example}(d)) of a point cloud using principal component analysis (PCA). From these, we can extract the three surface normals of the object (\eg vehicle): the vertical axis, the axis in the direction of motion, and the lateral axis.


==> perception.tex <==
\section{\sysname Perception}
\label{sec:perception}

In the section, we describe the perception component of \sysname, beginning with an overview.

\subsection{Perception Overview}
\label{s:perception-overview}

\parab{Inputs and Outputs.} The input to perception is a continuous sequence of LiDAR frames from each LiDAR in a set of \textit{overlapping} LiDARs deployed roadside. To ground the discussion, consider four LiDARs deployed at an intersection. \figref{fig:intersection_example}(a) shows a view of this intersection and LiDARs are mounted on traffic light poles at the four corners. In what follows, and in our evaluations, we focus on traffic management at intersections, in part because intersections are known to significantly impact traffic flow, and intersection management for autonomous vehicles is an emerging area in transportation research~\cite{AIMSurvey}. \sysname generalizes to other settings (\eg a busy thoroughfare), since it assumes nothing more than static deployment of overlapping LiDARs.\footnote{Practical deployments of roadside LiDARs will need to consider coverage redundancy and other placement geometry issues, which are beyond the scope of this paper.}

The output of perception is a compact \textit{abstract scene description}: a list of bounding boxes of moving objects in the environment together with their motion vectors (\figref{fig:intersection_example}(e)). This forms the input to the planner (\secref{s:planner}), which also requires other inputs that we describe later.

\begin{figure*}
  \centering
  \begin{minipage}{0.19\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/intersection_example_a.pdf}
    {\small (a)}
  \end{minipage}
  \begin{minipage}{0.19\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/intersection_example_b.pdf}
    {\small (b)}
  \end{minipage}
  \begin{minipage}{0.19\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/intersection_example_c.pdf}
    {\small (c)}
  \end{minipage}
  \begin{minipage}{0.19\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/intersection_example_d.pdf}
    {\small (d)}
  \end{minipage}
  \begin{minipage}{0.19\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/intersection_example_e.pdf}
    {\small (e)}
  \end{minipage}
  \caption{(a) A bird's eye view of an intersection. LiDARs are mounted on the traffic light poles at each of the four corners of the intersection. (b) An individual frame from each of the 4 LiDARs. (c) A fused frame. (d) Point clouds of traffic participants at the intersection. (e) Bounding boxes and motion vectors for traffic participants, calculated over successive frames.}
  \label{fig:intersection_example}
\end{figure*}

\parab{Goal and Approach.} The goal of perception design is to obtain the outputs from each frame of the input (a) in under 100~ms (perception should leave some of the latency budget for planning and for wireless transmission, we discuss this in \secref{sec:evaluation}), (b) with centimeter-level accuracy for positioning of objects, comparable to those in today's autonomous vehicles.

This is challenging because a single frame of the 64-beam Ouster LiDAR we use is over 3~MB. At 10~fps, this corresponds to 240~Mbps, uncompressed. Extracting precise semantic information from multiple LiDARs, in our example 4 LiDARs, at 1~Gbps within a tight latency budget requires (a) careful algorithmic and implementation choices, (b) exploiting properties of the setting.

Perception employs \textit{sensor fusion} (it combines data from multiple sensors), and fusion systems face one important design choice
that impacts all other algorithmic and implementation choices: whether to fuse the raw data first before extracting semantic information (early fusion), or whether to extract semantic information from individual sensor and fuse the results (late fusion). 

Fusing raw LiDAR data frames can be computationally expensive because it requires determining the lowest error alignment between every pair of frames (discussed in detail below). However, a fused LiDAR frame from overlapping LiDARs may have more complete representations of objects than individual LiDAR frames. \figref{fig:intersection_example}(b) shows the view from each of the 4 LiDARs; in many of them, only parts of a vehicle are visible. \figref{fig:intersection_example}(c) shows a \textit{fused frame} which combines the 4 LiDAR frames into one; in this, all vehicles are completely visible.\footnote{This may not be immediately obvious from the figure. A LiDAR frame, or a fused frame is a 3D object, of which \figref{fig:intersection_example}(c) is a 2D projection.} Intuitively, for this reason, early fusion is likely to perform better than late fusion.

%\ramesh{In the eval section, it would be good to quantify the cost of alignment.}

Fortunately, in our setting, early fusion is cheap: since the LiDARs are static, we compute their relative alignments in an offline calibration step, and per-frame processing uses these pre-computed alignments.

\parab{Perception Stages.}
Given this approach, \sysname's perception proceeds in three stages: \textit{fusion}, which fuses multiple LiDAR views; \textit{participant extraction}, which extracts traffic participants (vehicles, pedestrians); and \textit{tracking}, which estimates motion vectors of these objects. Each of these stages consists of one or more sub-stages described in \tabref{tab:perception_stages}. In the subsequent sections, we describe three of these sub-stages (in bold) in some detail, and only briefly describe other sub-stages because they use slight adaptations of existing techniques. The table also identifies which sub-stages require per-frame processing and therefore may be critical for performance. Processing requirements for some stages scale with the number of LiDARs and for others with the number of participant. Being explicitly aware of these is important for bounding tail latency~---~we discuss this later in this section, and in \secref{s:simul-results:-laten}).

\begin{table}[t]
  \begin{small}
  \centering
  \begin{tabular}{|l|l|c|c|}
    \hline
    \textbf{Stage} & \textbf{Sub-Stage} & \textbf{Per-frame?} & \textbf{Scaling}\\
    \hline
    Fusion & \textit{\textbf{Alignment}} &  & L\\
          & Stitching & \ding{51} & L\\
          & Background subtraction & \ding{51} & L\\
    \hline
    Participant & Clustering & \ding{51} & P\\
    Extraction  & \textit{\textbf{Bounding box estimation}} & \ding{51} & P\\
     & Association &  & P\\
    \hline
    Tracking & Track association & \ding{51} & P\\
          & \textit{\textbf{Heading vector}} & \ding{51} & P\\
          & Motion estimation & \ding{51} & P\\
    \hline
  \end{tabular}
  \caption{Perception stages and sub-stages. Stages in bold are described in more detail than other stages. Some sub-stages are invoked every frame and are critical to performance. A sub-stage's performance may be determined by the number of LiDARs (\textbf{L}) or the number of participants (\textbf{P}).}
  \label{tab:perception_stages}
  \end{small}
\end{table}

\subsection{Fusion}
\label{s:fusion}

\parab{Point Cloud Alignment.}
Each frame of a LiDAR contains a \textit{point cloud}, a collection of points with 3D coordinates. These 3D coordinates are in the LiDAR's own frame of reference. Fusing frames from two different LiDARs is the process of converting all 3D coordinates of both point clouds into a common frame of reference. \textit{Alignment} computes the transformation matrix for this conversion.

If the precise 3D positions and 3D orientations (or \textit{pose}) of the LiDARs are known, the transformation matrix can be trivially computed from these. This is hard to do in practice. A strawman approach might use GPS to obtain the pose of the LiDAR; an installer can obtain this by placing a commodity GPS device while mounting the LiDAR. Even if GPS were perfect, this is not sufficient: we \textit{also} need to know the transformation between the GPS (geoidal) coordinate system, and the local coordinate system chosen by the LiDAR hardware to position the points. LiDAR hardware positions points with the LiDAR at the origin, but an \textit{unknown orientation}. We need to align the orientation with the geoidal coordinate system, and we know of no way of doing this accurately.

%\pradipta{Just curios: Is there any data available on how much small configuration error can impact some downstream for example tracking? That will be nice to put here.}\ramesh{Good question, saved for later.}

\parae{ICP and the importance of good initial guesses.}
Prior work has developed Iterative Closest Point (ICP)~\cite{chen91:_objec,bellekens2015benchmark} techniques that \textit{search} for the lowest error alignment. The effectiveness of these approaches depends upon the initial guess for LiDARs' poses. Poor initial guesses can result in local minima. Most uses of ICP attempt to align successive point clouds obtained from a LiDAR on a moving vehicle; in these cases, it is easy to obtain good initial guesses. In our setting, for the reason described above, we cannot use GPS to get good initial guesses either.

\parae{Initial guesses using minimal information.}
Instead, because fusion is such an important step for us and poor guesses can lead to bad alignment (as we have learned by trial and error), \sysname uses a technique to get good initial guesses for LiDAR poses from \textit{minimal information}~---~the distances on the ground between a reference LiDAR and all others; off-the-shelf laser rangefinders suffice for measuring these. We now describe this technique for two LiDARs $L_1$ and $L_2$. It generalizes easily, as we shall show, to multiple LiDARs. We present a simplified description of the algorithm here: \secref{s:find-init-guess} has the details.

The inputs to this algorithm are two point clouds $C_1$ and $C_2$ captured from the corresponding LiDARs at the same instant, and the distance $d$ on the ground between the LiDARs. The output of this algorithm is an initial guess for the pose of each LiDAR. (By definition, an initial guess does not need to be precise: we feed these guesses into ICP to obtain good alignments).

Without loss of generality, set LiDAR $L_1$'s $x$ and $y$ coordinates to be $(0,0)$ (\ie the base of the LiDAR is at the origin). Then, assume that $L_2$'s base is at $(d,0)$. We now have to determine: (a) the height of each LiDAR $z_i$, and (b) the roll (angle around the $x$ axis), pitch (angle around the $y$ axis) and yaw (angle around the $z$ axis) of each LiDAR.

To fix the first three, \sysname relies on fast \textit{plane-finding} algorithms~\cite{derpanis2010overview} that extract planes from a collection of points. These techniques output the equations of the planes. Assuming that the largest plane is the \textit{ground-plane} (a reasonable assumption for roadside LiDARs), \sysname aligns the $z$ axis of two LiDARs with the normal to the ground plane. In this way, it implicitly fixes the roll and pitch of the LiDAR. Moreover, after alignment, the height of the LiDARs $z_i$ is also known (because the $z$ axis is perpendicular to the ground plane).

It only remains to determine the yaw for each LiDAR. To do this, we use a simple trick illustrated in \figref{fig:yaw_example}. Consider a point cloud visible in the two LiDARs. \sysname searches for the combination of yaw settings for the two LiDARs (\figref{fig:yaw_example}(a) and (b)) until it finds a combination that results in the smallest angle between the two point cloud's orientations\footnote{The actual search algorithm is a little bit more complex, \secref{s:find-init-guess}.} (\figref{fig:yaw_example}(c)). We have found that ICP is robust to initial guesses for yaw that are within about 15-20$^\circ$ of the actual yaw, so \sysname discretizes the search space by this amount.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.8\columnwidth]{figs/alignment_planes.png}
%   \caption{\sysname finds the yaw for the two LiDARs by searching for that combination where two surfaces on the point clouds have the smallest angle.}
%   \label{fig:yaw_example}
% \end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\columnwidth,frame]{figs/alignment_car.png}
  \caption{\sysname finds the yaw for the two LiDARs by searching ((a) and (b) for that combination where two surfaces on the point clouds have the smallest angle (c).}
  \label{fig:yaw_example}
\end{figure}

\sysname repeats this procedure for every other LiDAR $L_i$ with respect to $L_1$, at the end of which it has initial guesses for the poses of every LiDAR. It feeds these into ICP to obtain an alignment.

\parae{Re-calibrating alignment.} Alignment needs to be performed only when installing the LiDARs. In practice, re-alignment may be necessary if a LiDAR is replaced or otherwise re-positioned.

\parab{Stitching and Background Subtraction.} LiDARs generate frames at 10~fps (or more). In \figref{fig:intersection_example}, when each LiDAR generates a frame, the fusion stage performs \textit{stitching} and \textit{background subtraction}. Both of these are standard operations in point-cloud processing. Stitching applies the coordinate transformation for each LiDAR generated by alignment, resulting in a fused frame (\figref{fig:intersection_example}(c)). Thus, \sysname generates fused frames at the LiDAR frame rate.

Background subtraction, which removes points belonging to static parts of the scene, is (a) especially crucial for voluminous LiDAR data and (b) feasible in our setting because the LiDARs are static. It requires a calibration step to extract a \textit{background point cloud} from each LiDAR~\cite{kashani2015review}, then create a \textit{background fused frame} using the results from alignment. A simple heuristic such as taking the intersection of a few successive point clouds and the aggregating intersections taken at a few different time intervals, works well to generate the background point cloud. \sysname subtracts the background fused frame from each fused frame generated by stitching.

\parae{A performance optimization.}
We have found that performing these sub-stages in the opposite order can significantly reduce processing latency: \sysname first removes the background from LiDAR frame (using its background point cloud), and then stitches points in the residual point cloud. At the end of this step, the fused frame only contains points belonging to objects that are not part of the scene's background. Both of these steps scale with the number of LiDARs ($L$ in \tabref{tab:perception_stages}), but both are parallelizable. In \secref{sec:evaluation} we quantify the compute latency of these steps. However, because we seek to bound tail latency, being explicitly aware of the factors that affect the compute latency is important for \sysname.

\subsection{Participant Extraction}
\label{s:part-extr}

The subsequent stages of \sysname all operate on fused frames generated by the fusion stage.

\parab{Clustering.} \sysname uses a standard, fast, clustering algorithm
(DBSCAN)~\cite{ester1996density} to extract multiple clusters of points, where each cluster represents traffic participant.

% A subtle point about clustering performance. The cost of clustering depends on the number of participants, but it also depends upon the number of points representing each participant (since clustering has to examine every point at least once). This latter quantity depends on the number of LiDARs; \eg in \figref{fig:intersection_example}(b), a frame fused from 3 of the 4 LiDARs is likely to have fewer points for a vehicle than the fused frame in \figref{fig:intersection_example}(c).

\parab{Bounding Box Esstimation.} This sub-stage in \sysname is important because it generates an abstraction of objects useful in subsequent processing stages. It estimates the 3D bounding box of the points in a single cluster from the previous stage (\figref{fig:intersection_example}(d)). \sysname uses the 3D bounding box in 3 different ways. It: (a) tracks objects using its centroid, (b) estimates heading direction from the axes of the bounding box, and (c) uses the dimensions of the box to represent spatial constraints for planning. In our experience, developing such a re-usable abstraction early in the processing pipeline is crucial for minimizing latency.

\sysname uses an off-the-shelf algorithm~\cite{pclbbox}, which determines
a minimum oriented bounding box of a point cloud using principal component analysis (PCA). From these, we can extract the three surface normals of the object (\eg vehicle): the vertical axis, the axis in the direction of motion, and the lateral axis.

\parab{Cyber-Physical Association.} \sysname needs a way to associate an object it sees in the LIDAR with a cyber endpoint (\eg an IP address), because its planning component sends customized trajectories to each vehicle. %This sub-stage does not need to be invoked per frame, so we have not implemented it. Prior work~\cite{foresight,roadmap,roadview} has explored correlating a vehicle's visual features (\eg color, shape, license plate information) with its electronic features (\eg a GPS trace). Real deployments can use such solutions, or develop the kind of infrastructure used in tollways: proximity sensing of a transponder located close to a toll camera.
To find right assignments between objects from LiDAR scene and cyber endpoint, we leverage GPS readings from vehicles. We first guess a transformation on how to convert a trajectory in LiDAR reference to a trajectory in GPS reference in a known vehicle. In run-time, whenever a new vehicles is found in \sysname, we converted $w$ seconds of GPS trajectory of the vehicle into our LiDAR reference, and find a corresponding LiDAR trajectory which has the closet euclidean distance. This sub-stage does not need to be invoked per frame.  
\christina{Revised}

\subsection{Tracking}
\label{s:tracking}

Tracking follows objects across multiple fused frames and determines their motion characteristics (heading and velocity).

\parab{Multi-Object Tracking.} This well-known problem in visual processing tries to match objects in one fused frame, with objects in the next. When applied on every pair of successive frames, this approach can track each object in the first frame across all successive frames. Early tracking algorithms used a simple, highly efficient idea: (a) for each object in a frame, predict its position in the next frame using, for example, a Kalman filter~\cite{kalman1960new}; (b) find the best match (\eg in a least-squares sense) the predicted positions against the actual positions of all objects.

%\ramesh{To footnote above add a reference to a recent tracking DNN.}

Although tracking in point clouds is a challenging problem~\cite{vaquero2017deconvolutional} in general,
the earlier simple approach works \textit{exceedingly well} in our setting, so \sysname uses this (for prediction and matching, it represents the position of the object by the centroid of its bounding box, \secref{s:part-extr}). The biggest challenge in tracking is occlusions: when one object occludes another in a frame, it may be mistaken for the other in subsequent frames (an \textit{ID-switch}). Because our fused frame includes perspectives from multiple LiDARs, ID-switches occur rarely (in our evaluations, \secref{sec:evaluation}).

\parab{Heading Vector Estimation.} The next step is, at each frame, to determine, for each object, its instantaneous \textit{heading} (direction of motion). This is one of the three surface normals of the bounding box of the vehicle; in this sub-stage, we develop an algorithm to determine this accurately. Most on-vehicle perception systems can obtain heading from SLAM or visual odometry (\secref{sec:related_work}), so little prior work has explored extracting heading from infrastructure LiDAR frames.

%\ramesh{Note to self: Add a brief discussion of prior work. Point out why we can be more accurate: because we do more work like alignment, tracking, etc.}
%\weiwu{I added a small discussion of the related work of heading estimation at related work section. The key difference is that we are using non-DNN techniques and non on-vehicle sensors. I want to point out that heading estimation for us is a harder task(comparing to getting heading from SLAM or similar techniques.)}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\columnwidth,frame]{figs/hv.pdf}
  \caption{The figure shows the points belonging to a car, in two successive frames $t$ and $t+1$. (a) Strawman approach for heading determination. (b) \sysname's approach.}
  \label{fig:heading}
\end{figure}

Estimating heading is non-trivial. Consider an object $A$ at time $t$ and time $t+1$. \figref{fig:heading}(a) shows the points belonging to that object. Since those points are already in the same frame of reference, a strawman algorithm is: (a) find the vector between the centroid of $A$ at time $t$ and centroid of $A$ at time $t+1$, (b) the heading direction is the surface normal (from the bounding box) that is most closely aligned with this vector (\figref{fig:heading}(a)).

We have found that this approach can be inaccurate: if $A$ has fewer points in $t+1$ than in $t$ (\figref{fig:heading}(b)), the computed centroid will be different from the true centroid. To overcome this, we (a) use ICP to find the transformation matrix between $A$'s point cloud in $t$ and in $t+1$, (b) ``place'' $A$'s point cloud from $t$ in frame $t+1$ (\figref{fig:heading}(b), lower), (c) then compute the vector between the centroids of these two (so that the centroid calculations are based on the same set of points). As before, the heading direction is the surface normal (from the bounding box) that is most closely aligned with this vector.

\parae{A performance optimization.} ICP is compute-intensive, even for small object point clouds. If there are multiple objects in the frame, \sysname needs to perform ICP for each of them. Thus, this sub-stage (as well as many others in \tabref{tab:perception_stages}) scale with the number of participants (P in \tabref{tab:perception_stages}). We have experimentally found this to be the bottleneck stage, so we developed a fast GPU-based implementation of this ICP, which reduces the overhead of this stage by over $35\times$ (\secref{s:simul-results:-laten}).

\parae{Scene complexity and tail latency.}
The computational overhead of many perception systems can depend on scene complexity (in our case, the number of participants). In our experiments, the GPU we use can scale heading vector estimation to about 20 participants before exhausting the latency budget. Practical deployments can use multiple GPUs to scale better, since it is parallelizable. Edge computing systems can provide auto-scaling mechanisms, but may also need to be provisioned to deal with this workload variability.

\parab{Motion Vector Estimation.} The motion vector of an object has two components: (a) a direction, which we compute as the average of the heading vectors for the object over a time window $w$, and (b) a magnitude, the instantaneous velocity, which we estimate from the difference in position of the centroids of the bounding box at the beginning of $w$ and the most recent bounding box, divided by the time duration of the window.

% \parag{Heading direction estimation.} After the bounding box estimation, our algorithm selects one of three surface normals estimated in the bounding box estimation step to represent the heading direction of each vehicle. To filter out the heading direction of the vehicle at time $t$, our algorithm fetches a point cloud of the vehicle at time $t-1$ and compares it with the point cloud at $t$; this gives us a vehicle's moving direction from time $t-1$ to $t$. To this, we simply calculate the vector ($\overrightarrow{dv}_t$) between the vehicle's reference points (centroid) at time $t$  and at time $t-1$: $\overrightarrow{dv}_t = \overrightarrow{c_t} - \overrightarrow{c_{t-1}}$, where $\overrightarrow{c_t}$ and $\overrightarrow{c_{t-1}}$ are the 3D position vectors for the vehicle centroid at time $t$ and $t-1$, respectively. Next, we compare the direction of $\overrightarrow{dv}_t$ with the three surface normals of the vehicle and select the one with the most similarity with $\overrightarrow{dv}_t$. This method works under the assumption that the vehicle's moving direction from $t-1$ to $t$ is not much different from the vehicle's instant heading direction at $t$.

% To get an accurate $\overrightarrow{dv}_t$, we first run ICP algorithm to align the point cloud of the vehicle at time $t-1$ with the point cloud of the vehicle at time $t$. Next, we use the original point cloud at $t-1$ and the aligned point cloud to robustly calculate $\overrightarrow{dv}_t$.
% \pradipta{From the meeting, if I remember correctly, the point cloud here is only for the vehicle; not the entire frame. Right? If so, we need to make it clear.}
% \christina{Yes. I simply changed to "point cloud of the vehicle". Do we need more explanation?}
% \pradipta{Should be fine I guess. But there is a slight disconnect in the write up then bcoz all of a sudden you are talking about vehicle point cloud instead of the whole point cloud. Ramesh will have better idea about this.}

% In this section, we detail our proposed vehicle tracking method based on infrastructure based LiDARs. After the object clustering step (see above), \sysname's perception module assigns an unique ID to each detected object in the scene. The main goal of this step is to identify inter-frame associations and detect same objects over the consecutive frames. Lack of semantic information poses an intrinsic challenge to multi-objects tracking in 3D point cloud as compared to 2D image data~\cite{vaquero2017deconvolutional}. Nonetheless, 3D data is often enriched with geometry information. Researchers often apply \textit{Kalman filtering}~\cite{kalman1960new} or \textit{Hungarian algorithm}~\cite{kuhn1955hungarian} on such geometric data for accurate and fast tracking~\cite{}; the performance of such methods are vulnerable to occluded objects or incomplete point clouds. Interestingly, \sysname do not suffer from such incomplete point cloud problem since we leverage stitched point clouds from multi-LiDARs that capture a more complete picture of the scene.
% \christina{Note-to-myself: Need to add kf tracking citations}

% \ramesh{please consider re-organizing the above paragraph according to the template discussed for alignment: A few sentences on the problem, A few on prior work, A few sentences describing why is the prior work falls short, and a few sentences that describe the key idea behind our approach.}
% \ramesh{the last sentence is good, but we need to discuss how stitched point clouds help. Do they let us design a cheaper algorithm? Or do they give higher accuracy when we use an existing algorithm?}
% \ramesh{To the algorithm description below, let's try to answer them contextual information: how similar or different is it from standard ways of doing tracking?}
% \ramesh{Also, in the rewrite, we should explicitly mention clustering in this section, otherwise readers will not be able to match the description in the overview to the tracking section.}

% % https://www.mathworks.com/help/fusion/ug/introduction-to-assignment-methods-in-tracking-systems.html
% \sysname adopts Kalman filtering to track objects and assign corresponding IDs with a simple distance-based scheme. Based on previous history of identified objects, our algorithm applies Kalman filtering to first calculate the expected/estimated positions of the tracked vehicles (\ie vehicles identified in earlier frames). On the other end, \sysname observes a set of vehicles in the current point cloud frame and outputs their clusters. For the purpose of ID assignment, we represent each vehicle by the centroid of the object's cluster in the point cloud; we use these also as the \textit{reference points} for each tracked vehicles. Now, let us denote the estimated positions of $u$ tracked objects as $e_1, e_2, ..., e_u$ and the observed positions of $v$ objects as $o_1, o_2, ..., o_v$, respectively. Lastly, we introduce a distance matrix $D$ where $D_{ij}$ is the Euclidean distance between $e_i$ and $o_j$. With this, the tracking problem is converted into a matching like problem; we use distance metrics to match the estimated locations with the observed locations. Our algorithm finds an assignments $A = \{a_{ij}\}$ that minimizes the summation of distance of assignments as follows:

% % \begin{flalign*}
% % &\textrm{Minimize}  \hspace{10mm} \sum_{i=0}^{n}\sum_{j=1}^{m}D_{ij}a_{ij} && \\
% % &\textrm{Subject to} \hspace{10mm} \sum_{i=0}^{m}a_{ij} = 0, \forall j &&\\
% % & \hspace{23mm} \sum_{j=0}^{n}a_{ij} = 0, \forall i &&
% % \end{flalign*}

% \begin{flalign*}
% &\textrm{Minimize}  \hspace{10mm} \sum_{i=1}^{u}\sum_{j=1}^{v}D_{ij}a_{ij} && \\
% &\textrm{Subject to} \hspace{10mm} \sum_{i=0}^{u}a_{ij} = 1, \forall j \in \{1, \cdots, v\} &&\\
% & \hspace{23mm} \sum_{j=0}^{v}a_{ij} = 1, \forall i \in \{1, \cdots, u\}  &&
% \end{flalign*}
% \pradipta{The equations did not seem right. I modified it based on my understanding. Please check.}
% \pradipta{The cost function seems bit weird to me. This will force to minimize the sum of distance. Then the solution will be all $a_{i0} = 1$ and $a_{0j} = 1$. To circumvent this, typically a large cost is added for the 0 assignment case. But even then the problem will be it will always try to assign a matching even though there is no correlation. I guess the best cost function would be to use $D_{i0}$ and $D_{0,1}$ to be a threshold distance for matching. Maybe you are already doing that. But please check.}
% \christina{Yes, I get your point. Our current implementation is using the distance threshold (5m) for the matching so maybe we need to add what you suggested? Also, other than that, I was wrong on the equation and the changed one makes sense!}
% \pradipta{I see. In that case, please update the equation and the description.}
% Here, $a_{ij} = 1$ implies estimated object $e_i$ is matched to observed object $o_j$. If an estimated object $e_i$ is not matched with any observed object, $a_{i0} = 1$. Similarly, if $o_j$ is not matched with any estimations, then $a_{0j} = 1$. The optimization function makes sure that the closest pair is matched together while the constraints ensures each estimation is associated with no more than one observation, vice versa.

% After solving this optimization, we should have correct ID assignment to each vehicles. We feed the output \ie a list of tracked object ID with their respective reference points ($o_j$) to the motion estimation and planning module.

% To close the sensing-perception-control loop, we need to establish a \sysname-to-vehicle communication. We assume that the vehicles controlled by \sysname need to be equipped with some kinds of radio interface, such as WiFi, to receive the control commands. Each vehicles controlled by \sysname is assigned a unique NID(network id, such as a MAC/IP Address). \sysname can use the unique NID to send control message to the corresponding vehicle.

% Each tracked vehicle in \sysname also receives a TID(tracking ID). Each vehicle in the LiDAR point cloud is consistently tracked by \sysname and receives the same TID. Because \sysname's planner and controller works with the instances detected in the LiDAR point cloud, they produce control commands based on the TIDs. To communicate the control commands to the corresponding vehicle in the physical world, \sysname needs to establish the association between TIDs and the NIDs.

% Prior works (\cite{foresight}), \cite{roadmap} and \cite{roadview}) have explored thoroughly about how to combine a vehicle's visual feature(\eg color, shape, liscence plates, \etc) and electronic features(\eg GPS) at a given timestamp. Each vehicle will publish(through the network interface) its own feature vector and its NID, and at the same time receive feature vectors generated by other vehicles. At each timestamp, each vehicle measures the feature of its visual neighbors and perform feature matching between the set of visual features(through camera) and the received features(through network). Because each vehicle broadcast both its NID and its own features to its neighbors, this allows each vehicle to be discovered and matched by its neighbors.

% A \textit{background point cloud} is a point cloud frame that represents the static background of a sensed region (such as roads, buildings, and traffic signs). \sysname compares a point cloud frame with a background point cloud to identify dynamics objects (such as cars and humans). In a real-world setting, it is challenging to find an empty scene without any dynamic objects to generate a background point cloud. A trivial approach can take an intersection of multiple consecutive frames; however, this may include temporary static objects such as a parked vehicle. 
% To this, we take an intersection of $P$ temporally isolated frames to completely filter out dynamic points and form a \emph{common frame}.  A single common frame is, yet, not a robust representation of the background point cloud; it might be missing a significant subset of background static points~\cite{kashani2015review} due to either temporary obstructions or LiDAR hardware issues. To solve this practical problem, we generate $Q$ temporally distributed common frames and aggregate them to form the final background point cloud. 

\iffalse
% \ramesh{Let's have two separate sections, one for perception and one for planning. The architecture section will discuss these at a high-level, so it is probably OK to do that.}

% \ramesh{In this section, we should have an overview subsection, followed by three subsections one each for the three main components that we discussed.}
% \ramesh{Here is the grouping we discussed today for the three main components, together with suggested new terminology. Please leave comments if you think there is better terminology that we should adopt. (a) \textit{\textbf{View fusion}}, which consists of \textit{alignment} and \textit{stitching}, (b) \textit{\textbf{Participant extraction}}, which consists of \textit{background subtraction}, \textit{point clustering} and \textit{participant association} and (c) \textit{\textbf{Tracking}}, which consists of \textit{track association}, \textit{motion estimation}, \textit{heading estimation}. }

\subsection{Infrastructure-based Perception}

In this section, we detail one of the main contributions of \sysname: Infrastructure LiDAR-based \emph{real time} perception; this component is key to our proposed decoupling (\secref{sec:architecture}) of the state-of-the-art autonomous driving stack. We propose a novel perception algorithm that combines 3D point clouds from multiple geographically-distributed static LiDARs and processes a unified point cloud in real-time to enable fine-grain localization and tracking for autonomous driving. Note that \sysname does not plan the LiDAR placement; \sysname assumes that a deploying authority will use an intelligent topology planner to deploy a sufficient (say, $N$) number of LiDARs in a road intersection.

\ramesh{make sure to update \figref{fig:av_stack} with the components of the perception pipeline, or create a new figure.}

% \sysname relies on 3D sensors deployed on road-side infrastructure for perception. Each 3D sensor generates 3D frames at different frame rates per second. \sysname continuously merges point clouds from all these sensors into a single, stitched, real-time 3D point cloud. We call this component \textit{point-cloud stitching}. It is a part of the perception module, and it runs at the edge. The current autonomous driving pipeline does not contain such capabilities.
% Commented out by Christina

\ramesh{Create a new sub section. Call it design overview or \sysname overview. We have already talked about the architecture in the previous section.}
\parab{Overall Architecture.} 
Let us assume that a set of $N$ LiDARs are deployed in a designated intersection; each LiDAR generates a 3D point-cloud frame at a constant rate of $f$ frames per seconds (\ie 1 frame in every $T = 1/f$ seconds) and transfers it to the perception module of \sysname. In every $T$ seconds, \sysname's perception module processes the most recent set of $N$ frames (1 from each LiDAR) to detect any moving objects (\eg a car or a pedestrian) and to output the motion information of the detected objects; this is further fed to \sysname's planner module (\figref{fig:sys_overtaking}) to generate desired path trajectories for autonomous vehicles. To estimate accurate motion information in real-time, \sysname executes a one-time initialization step\footnote{We may need to re-invoke the initialization step if there is a dramatic change in the surroundings such as the spawning of a new building.} followed by a set of five sequential steps in every sensing period ($T$) as follows.
% \pradipta{The Initialization is run once at the beginning right? Or Do you run it again after some time?}
% \christina{We can run it again to detect some dynamics in roads, if necessary. However, for now, we just can say it runs once at the beginning.}

\ramesh{What do you have below is a great start! However, the overview section needs to be short and crisp. First, instead of having six different components, which is hard for a reader to keep in mind, can we describe the system as having three top level components, each of which we have two or more sub components? What would those be?}
\ramesh{Second, for each sub component start with the "what" (see detailed comments below), and have a brief sentence that describes the "how" and how the "how" is a novel contribution.}
\ramesh{For example, this is how I would describe the initialization component in an overview section. I would pick a better name, such as \textit{calibration} or even \textit{alignment}. (It is not clear that the step needs to be done only once. It may need to be done for example if the Lidar has moved for any reason). Then, the text would be something like: The position of a point in a LiDAR's point cloud is described in that LiDAR's frame of reference. In order to detect objects from multiple LiDARs, \sysname needs to ensure that all LiDAR point clouds are positioned within a common coordinate frame of reference. The alignment step, performed once initially and again whenever a LiDAR is reconfigured, adapts prior work on point cloud registration to be robust to settings, such as ours, when the point clouds are captured from vastly different perspectives.}
\ramesh{Also, if we are claiming alignment to be a contribution, let's find a name to describe it.}

\parag{Initialization.} To efficiently detect the dynamic objects and extract the respective motion information, \sysname needs two basic information: (1) Pair-wise transformation matrices between LiDARs and (2) a background point cloud. In addition, \sysname needs to detect drivable Space to plan the autonomous vehicle trajectories. 

We need the pair-wise transformation matrix to fuse the 3D sensory data from multiple LiDARs into a unified point cloud. Each LiDAR point cloud is represented by its own (and independent) frame of reference (or coordinate system). To combine two LiDAR point clouds, we apply coordinate transformation from one's point cloud to the other; a pairwise transformation matrix is a key to this. Estimation of the transformation matrices takes several minutes and can be done offline as the LiDARs are static. To this, \sysname completes a \emph{Point Cloud Alignment} process as a part of the initialization (detailed below).

A \textit{background point cloud} is a point cloud frame that represents the static background of a sensed region (such as roads, buildings, and traffic signs). \sysname compares a point cloud frame with a background point cloud to identify dynamics objects (such as cars and humans). In a real-world setting, it is challenging to find an empty scene without any dynamic objects to generate a background point cloud. A trivial approach can take an intersection of multiple consecutive frames; however, this may include temporary static objects such as a parked vehicle. 
To this, we take an intersection of $P$ temporally isolated frames to completely filter out dynamic points and form a \emph{common frame}.  A single common frame is, yet, not a robust representation of the background point cloud; it might be missing a significant subset of background static points~\cite{kashani2015review} due to either temporary obstructions or LiDAR hardware issues. To solve this practical problem, we generate $Q$ temporally distributed common frames and aggregate them to form the final background point cloud. 
The background point cloud construction takes a significant amount of time and only needs to be updated after a dramatic change in the surroundings such as the spawning of a new building. Therefore, \sysname performs the \textit{Background Point Cloud Construction} as a part of the initialization.
% \pradipta{I am actually more confused now. You say that P frames should not be consecutive. But then what the reason behind first combing P
\pradipta{What are the typical values of P and Q?}
\pradipta{minor comment: can we come up with a meaningful name instead of "common frame"?}
% \pradipta{Please check. Also, Can you write 1-2 sentences on how does the aggregation helps?}
% \christina{Actually, I was wrong for describing how we get the background construction, so revised the writing. Please check and let me know when it confuses you.}
\ramesh{I noticed that we discuss point cloud alignment in more detail in a later section. Let's move the above paragraph to that section. The principle is that in this overview section, we should be discussing \textit{what} we do, not \textit{how} we do it}

Lastly, for the planner module to design trajectories, we need to inform the planner where vehicles can drive safely and legally.
\pradipta{Please write the drivable space extraction part here.}
\pradipta{Also, can we add an illustrative image for each of the steps?}
\christina{Yes, I think that is a good idea! I will make corresponding images and update the paper.}

% To extract the necessary motion information in real-time, \sysname performs an initialization (or pre-processing) step to perform three time-consuming (takes several minutes) and resource-heavy operations: (1) \textit{Point Cloud Alignment}, (2) \textit{Background Point Cloud Construction} and (3) \textit{Drivable Space Extraction}. The \emph{Point Cloud Alignment} process extracts pair-wise transformation matrix between the LiDARs; this is a key information required to fuse the 3D sensory data from multiple LiDAR into an unified point cloud. We propose a novel algorithm to extract the pairwise transformation matrices (detailed below). \sysname also needs to construct one frame of point cloud that only contains background points from Background Point Cloud Construction. The background point cloud will be used to filter out the background from each collected data. In real-world, however, it is not always easy to collect a point cloud from an empty scene without any vehicle. Thus, we spend some time constructing a robust background point cloud. Given an integer $i$ and $j$, we pick $i \times $j number of random frames such that there are $i$ number of sets of point clouds and each set has $j$ number of consecutive point clouds. Then, we extract common points in each set and merged these $i$ number of intersectioned point clouds into one frame of background point cloud. In this way, we can construct a robust background even under a dynamic situation. For the planner module to design trajectories, we need to let the planner know where vehicles can drive safely and legally.

\parag{Stitching.} After proper initialization, the first step of \sysname's perception module is to stitch the most-recent $N$
\ramesh{Shouldn't this be: the most recent frame from each of the $N$ different LiDARs?} frames from different LiDARs into one unified frame; we call this a \textit{stitched point cloud frame}. Each LiDAR's 3D frame is presented in its coordinate systems. \sysname applies a linear coordinate transformation to each frame with the respective transformation matrix (obtained from \textit{Point Cloud Alignment}) to aggregate them into the stitched point cloud frame. The stitched point cloud presents a full view of the scene; it aggregates information about everything detected by the LiDARs such as ground planes, buildings, and vehicles. We further detail the stitching process below.

\ramesh{Rewrite the previous paragraph to describe the what before the how. The last sentence gets close to the how.} 
\ramesh{Also, as you write, keep in mind that the why is also an important consideration. We should discuss why we do stitching, and what other options are possible. The Overview may not be the best place to do this, it might be better to describe the why closer to the how.}

\parag{Background filtering.} In the second step, \sysname's perception module filters out all points residing in the background and extracts only dynamics object (in our case mainly vehicles) by simply removing the overlapping points between the stitched point cloud and the background point cloud (obtained from the \textit{Background Cloud Construction}). This is sufficient in our setting as the LiDARs are fixed and the background points are mostly static; this is quite different from traditional autonomous vehicle systems with moving LiDARs.
% \pradipta{Do we assume that there is no other dynamic object other than vehicles?}
% \christina{There can be other objects. However, we haven't designed yet how to cope with them.}

\parag{Clustering.} After background filtering, the stitched point cloud only contains dynamic objects. Assuming there exists no dynamic object other than vehicles, \sysname's perception module performs a \textit{Density-based Spatial Clustering with Noise} (DBSCAN)~\cite{ester1996density} to extract multiple clusters where each cluster corresponds to a vehicle.
% \christina{Added a citation.}

\parag{Tracking/Association.} Following the clustering step, \sysname examines the clusters to associate vehicle identities; this is required to persistently track the same vehicles in-between frames. We propose a Kalman filtering~\cite{kalman1960new} based method to find the correct correspondences between the current set of detected vehicles and the vehicles detected in earlier frames and to perform a consistent tracking of individual vehicles. The tracking algorithm also outputs the location of a consistent reference point for each vehicle. This is further detailed later on.
% \christina{Added a citation.}

% \parag{Motion estimation.} In the last step, \sysname's perception module estimates the location and movement state of each vehicle. To this, \sysname estimates four different parameters to completely represent a vehicle's motion: (1) the location of a reference point of the vehicle, (2) the oriented bounding box of the vehicle, (3) the instant heading direction, and (4) the motion vector over a time window. The location of a reference point and the bounding box summarize the dimensions of a vehicle and the location (position and orientation) in the stitched 3D frame. In addition to the localization information, we need the heading direction and the motion vector to characterize the motion of each vehicle in the current stitched 3D frame. We use the term, \textit{heading direction}, to infer an instantaneous heading direction at the time. On the other hand, a \textit{motion vector} embodies the velocity and the heading direction of a vehicle averaged over a short period of time. How \sysname estimates these parameters is further explained in details below.

\parag{Motion estimation.} In the last step, \sysname's perception module estimates the movement state of each vehicle. With the estimated location of a reference point of the vehicle (obtained from \textit{Tracking/Association}), \sysname estimates three different parameters to completely represent a vehicle's motion: (1) the oriented bounding box of the vehicle, (2) the instant heading direction, and (3) the motion vector over a time window. The location of a reference point and the bounding box summarize the dimensions of a vehicle and the location (position and orientation) in the stitched 3D frame. In addition to the localization information, we need the heading direction and the motion vector to characterize the motion of each vehicle in the current stitched 3D frame. We use the term, \textit{heading direction}, to infer an instantaneous heading direction at the time. On the other hand, a \textit{motion vector} embodies the velocity and the heading direction of a vehicle averaged over a short period of time. How \sysname estimates these parameters is further explained in details below.
% \christina{Revised it to remove location estimation in this phase.}

% %% - Point-cloud stitching
% \fawad{Weiwu: please write down the details of the point cloud stitching algorithm here.}
% \sysname relies on 3D sensors deployed on road-side infrastructure for perception. Each 3D sensor generates 3D frames at different frame rates per second. \sysname continuously merges point clouds from all these sensors into a single, stitched, real-time 3D point cloud. We call this component \textit{point-cloud stitching}. It is a part of the perception module, and it runs at the edge. Current autonomous driving pipeline do not contain such capabilities.
% Commented out by Weiwu

% %% - Object detection and tracking
% \fawad{Christina: please write down all perception components here. Once you are done, please let me know}
% After generating the real-time stitched 3D map, the perception module uses it to understand condition of the road. In doing so, it segments the scene into static, and dynamic objects and then tracks the motion of the dynamic objects. One way of doing this is to segment the stitched point cloud. This component is also a part of the perception module. It runs at the edge, and we call it \textit{object detection and tracking}. Current autonomous driving pipelines contain similar components for tracking objects. However, they use monolithic (unstitched) point clouds from a single 3D sensor atop a vehicle rather than stitched point clouds.
% Commented out by Christina

\parab{Tracking.}
In this section, we detail our proposed vehicle tracking method based on infrastructure based LiDARs. After the object clustering step (see above), \sysname's perception module assigns an unique ID to each detected object in the scene. The main goal of this step is to identify inter-frame associations and detect same objects over the consecutive frames. Lack of semantic information poses an intrinsic challenge to multi-objects tracking in 3D point cloud as compared to 2D image data~\cite{vaquero2017deconvolutional}. Nonetheless, 3D data is often enriched with geometry information. Researchers often apply \textit{Kalman filtering}~\cite{kalman1960new} or \textit{Hungarian algorithm}~\cite{kuhn1955hungarian} on such geometric data for accurate and fast tracking~\cite{}; the performance of such methods are vulnerable to occluded objects or incomplete point clouds. Interestingly, \sysname do not suffer from such incomplete point cloud problem since we leverage stitched point clouds from multi-LiDARs that capture a more complete picture of the scene.
\christina{Note-to-myself: Need to add kf tracking citations}

\ramesh{please consider re-organizing the above paragraph according to the template discussed for alignment: A few sentences on the problem, A few on prior work, A few sentences describing why is the prior work falls short, and a few sentences that describe the key idea behind our approach.}
\ramesh{the last sentence is good, but we need to discuss how stitched point clouds help. Do they let us design a cheaper algorithm? Or do they give higher accuracy when we use an existing algorithm?}
\ramesh{To the algorithm description below, let's try to answer them contextual information: how similar or different is it from standard ways of doing tracking?}
\ramesh{Also, in the rewrite, we should explicitly mention clustering in this section, otherwise readers will not be able to match the description in the overview to the tracking section.}

% https://www.mathworks.com/help/fusion/ug/introduction-to-assignment-methods-in-tracking-systems.html
\sysname adopts Kalman filtering to track objects and assign corresponding IDs with a simple distance-based scheme. Based on previous history of identified objects, our algorithm applies Kalman filtering to first calculate the expected/estimated positions of the tracked vehicles (\ie vehicles identified in earlier frames). On the other end, \sysname observes a set of vehicles in the current point cloud frame and outputs their clusters. For the purpose of ID assignment, we represent each vehicle by the centroid of the object's cluster in the point cloud; we use these also as the \textit{reference points} for each tracked vehicles. Now, let us denote the estimated positions of $u$ tracked objects as $e_1, e_2, ..., e_u$ and the observed positions of $v$ objects as $o_1, o_2, ..., o_v$, respectively. Lastly, we introduce a distance matrix $D$ where $D_{ij}$ is the Euclidean distance between $e_i$ and $o_j$. With this, the tracking problem is converted into a matching like problem; we use distance metrics to match the estimated locations with the observed locations. Our algorithm finds an assignments $A = \{a_{ij}\}$ that minimizes the summation of distance of assignments as follows:

% \begin{flalign*}
% &\textrm{Minimize}  \hspace{10mm} \sum_{i=0}^{n}\sum_{j=1}^{m}D_{ij}a_{ij} && \\
% &\textrm{Subject to} \hspace{10mm} \sum_{i=0}^{m}a_{ij} = 0, \forall j &&\\
% & \hspace{23mm} \sum_{j=0}^{n}a_{ij} = 0, \forall i &&
% \end{flalign*}

\begin{flalign*}
&\textrm{Minimize}  \hspace{10mm} \sum_{i=1}^{u}\sum_{j=1}^{v}D_{ij}a_{ij} && \\
&\textrm{Subject to} \hspace{10mm} \sum_{i=0}^{u}a_{ij} = 1, \forall j \in \{1, \cdots, v\} &&\\
& \hspace{23mm} \sum_{j=0}^{v}a_{ij} = 1, \forall i \in \{1, \cdots, u\}  &&
\end{flalign*}
\pradipta{The equations did not seem right. I modified it based on my understanding. Please check.}
\pradipta{The cost function seems bit weird to me. This will force to minimize the sum of distance. Then the solution will be all $a_{i0} = 1$ and $a_{0j} = 1$. To circumvent this, typically a large cost is added for the 0 assignment case. But even then the problem will be it will always try to assign a matching even though there is no correlation. I guess the best cost function would be to use $D_{i0}$ and $D_{0,1}$ to be a threshold distance for matching. Maybe you are already doing that. But please check.}
\christina{Yes, I get your point. Our current implementation is using the distance threshold (5m) for the matching so maybe we need to add what you suggested? Also, other than that, I was wrong on the equation and the changed one makes sense!}
\pradipta{I see. In that case, please update the equation and the description.}
Here, $a_{ij} = 1$ implies estimated object $e_i$ is matched to observed object $o_j$. If an estimated object $e_i$ is not matched with any observed object, $a_{i0} = 1$. Similarly, if $o_j$ is not matched with any estimations, then $a_{0j} = 1$. The optimization function makes sure that the closest pair is matched together while the constraints ensures each estimation is associated with no more than one observation, vice versa.

After solving this optimization, we should have correct ID assignment to each vehicles. We feed the output \ie a list of tracked object ID with their respective reference points ($o_j$) to the motion estimation and planning module.

% Our algorithm set a position of objects to a centroid of the object's point cloud. The main idea to do association between these estimations and observations is to assign a nearest observation to an identified estimation. We introduce estimation positions as $e_1, e_2, ..., e_n$ , observed positions as $o_1, o_2, ..., o_m$, and a distance matrix $D_{ij}$ where $D_{ij}$ is an euclidean distance between $e_i$ and $o_j$.

% As mentioned above, detected objects are almost free from the occlusion problem because \sysname utilizes stitched point clouds from multi-LiDARs. Thus, this proposed distance-based scheme is simple yet effective.

\parab{Cyber-physical association.}
\weiwu{Placeholder}

\parab{Motion Estimation.}
% The last step of our perception module is \textit{motion estimation}. The motion estimation procedure estimates the four different components of the current motion state (detailed above) of the detected objects: (1) the location of a reference point of the vehicle, (2) the oriented bounding box of the vehicle, (3) the instant heading direction, and (4) the motion vector over a time window.
The last step of our perception module is \textit{motion estimation}. The motion estimation procedure estimates the three different components of the current motion state (detailed above) of the detected objects: (1) the oriented bounding box of the vehicle, (2) the instant heading direction, and (3) the motion vector over a time window. This data is directly fed to \sysname's planning module and used to generate trajectory plans for each vehicle. The collected LiDAR data is very time-sensitive with regards to trajectory (path) planning; our proposed algorithm, therefore, aims to complete the motion estimation in real-time while maximizing the accuracy.
% \pradipta{Is the location estimated part of the motion estimation? From reading it seems to be part of the tracking/association phase. Please correct me if I am wrong. If I am right, we should remove it here. Other wise we should add a para or line about it here.}
% \christina{Yes, it is obtained from tracking/association. I removed it.}

\ramesh{As with other sections, this is a very nice start. Please follow the comments I have given in the other sections to re-write the section. In particular, for this audience we need to help them understand what is novel relative to prior work, and what kinds of trade-offs we have made.}

% The perception module in \sysname outputs a reference point, a bounding box, heading direction, and motion vectors for each vehicle. By referring the position and the bounding box, the planning module gets a rough size of the vehicle and localizes it at the same time. Other than localization, motion information is acquired from heading direction and motion vector. In this paper, we use the term, \textit{heading direction}, to infer an instantaneous heading direction at the time. On the other hand, \textit{motion vector} means a continuous heading direction and velocity over the time. Both information are complimentary, and will give us more understanding of the scene.

% http://codextechnicanum.blogspot.com/2015/04/find-minimum-oriented-bounding-box-of.html
\parag{Bounding box estimation.} Our motion estimation starts with bounding box estimation. As implemented in \cite{pclbbox}, a minimum oriented bounding box of a given vehicle is extracted by using eigenvectors and covariance matrix of the point cloud. Based on the extracted bounding box, our algorithm estimates three surface normals (i.e., front direction, side direction, and upper direction) of the bounding box; these are fed to the next step to select the correct normal vectors as a heading direction of the vehicle.

\parag{Heading direction estimation.} After the bounding box estimation, our algorithm selects one of three surface normals estimated in the bounding box estimation step to represent the heading direction of each vehicle. To filter out the heading direction of the vehicle at time $t$, our algorithm fetches a point cloud of the vehicle at time $t-1$ and compares it with the point cloud at $t$; this gives us a vehicle's moving direction from time $t-1$ to $t$. To this, we simply calculate the vector ($\overrightarrow{dv}_t$) between the vehicle's reference points (centroid) at time $t$  and at time $t-1$: $\overrightarrow{dv}_t = \overrightarrow{c_t} - \overrightarrow{c_{t-1}}$, where $\overrightarrow{c_t}$ and $\overrightarrow{c_{t-1}}$ are the 3D position vectors for the vehicle centroid at time $t$ and $t-1$, respectively. Next, we compare the direction of $\overrightarrow{dv}_t$ with the three surface normals of the vehicle and select the one with the most similarity with $\overrightarrow{dv}_t$. This method works under the assumption that the vehicle's moving direction from $t-1$ to $t$ is not much different from the vehicle's instant heading direction at $t$.

To get an accurate $\overrightarrow{dv}_t$, we first run ICP algorithm to align the point cloud of the vehicle at time $t-1$ with the point cloud of the vehicle at time $t$. Next, we use the original point cloud at $t-1$ and the aligned point cloud to robustly calculate $\overrightarrow{dv}_t$.
\pradipta{From the meeting, if I remember correctly, the point cloud here is only for the vehicle; not the entire frame. Right? If so, we need to make it clear.}
\christina{Yes. I simply changed to "point cloud of the vehicle". Do we need more explanation?}
\pradipta{Should be fine I guess. But there is a slight disconnect in the write up then bcoz all of a sudden you are talking about vehicle point cloud instead of the whole point cloud. Ramesh will have better idea about this.}
% It is important to get an accurate $dv_t$ between two given point clouds. Thus, we run ICP algorithm to align those two point clouds. By running ICP, we first obtain a transformation matrix from point cloud at $t-1$ to $t$. Then, we transform the point cloud at $t-1$ under the obtained transformation matrix. Lastly, we gain $dv_t$ between the point clout at $t-1$ and transformed point cloud. Because we calculates $dv_t$ from two aligned centroid points, more robust estimation can be achieved.

\parag{Motion vector estimation.} For the last step in our motion estimation, our algorithm tracks a motion vector. We can decompose the motion vector into two sub-components; direction and magnitude of the vector. Direction of the motion vector indicates an averaged heading direction over a given time window, $w$, and we interpret it to a heading trend within the time window \pradiptas{What do you mean here?}. Magnitude of the vector is nothing but the average speed over the time window $w$. Our algorithm estimates the direction of the motion vector by simply averaging the estimated heading direction over $w$. To get the magnitude of the motion vector, our algorithm fetches another point cloud of the vehicle which is $w$ frames ahead and runs ICP to align them. Similar to the heading vector estimation above, we calculate a displacement vector $\overrightarrow{dv}_t$ for the vehicle from time $t-w$ to time $t$ and set $|\overrightarrow{dv}_t|$ as the magnitude of the motion vector.
\christina{I mean the direction of the vector is somehow averaged heading direction. Can you help to make it more clear?}
\pradipta{But I thought the displacement vector direction is the motion vector direction. Is it not? How are you averaging the direction otherwise?}
We notice that our proposed motion estimation is vulnerable to noisy data from sensor faults and such noisy data is quite common in real-world data collection. To filter out such noises, we adopt Kalman filtering. \sysname maintains a separate Kalman filter model for each detected vehicle. Instead of outputting the instantaneous motion vector, our algorithm feeds the newly estimated motion vector to the Kalman filter and outputs a less noisy motion vector.

% \ramesh{Point out that this is one way of doing it. The point about how current autonomous driving has the same components is good.}
% \fawad{Addressed.}

\fi


==> perception_new.tex <==
\section{Perception}
\label{sec:perception}

\sysname consists of two components (\tabref{tab:stack_comparison}): perception and planning. In this section, we describe the former. 

\subsection{Perception Overview}
\label{s:perception-overview}

\parab{Inputs and Outputs.} The input to perception is a continuous sequence of LiDAR frames from each LiDAR in a set of \textit{overlapping} LiDARs deployed roadside. Consider four LiDARs deployed at an intersection.\footnote{\sysname generalizes to other settings but we focus on traffic intersections~\cite{AIMSurvey}, a significant challenge in transportation research.}
% , a significant challenge in transportation~\cite{AIMSurvey}}.
% \sysname generalizes to other settings (\eg a busy thoroughfare), since it only assumes a static deployment of overlapping LiDARs.}  
\figref{fig:intersection_example}(a) shows a view of a busy intersection in a major metropolitan area.
%
At this intersection, we mounted LiDARs\footnote{Practical deployments of roadside LiDARs will need to consider coverage redundancy and other placement geometry issues, which are beyond the scope of this paper.} at the four corners (\secref{sec:evaluation}).

The output of perception is a compact \textit{abstract scene description}: a list of bounding boxes of moving objects in the environment together with their motion vectors (\figref{fig:intersection_example}(e)).
%
This forms the input to the planner (\secref{s:planner}), which also requires other inputs that we describe later.

\begin{figure*}
  \centering
  \begin{minipage}{0.19\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/bird_eye_view_intersection.png}
    {\small (a)}
  \end{minipage}
  \begin{minipage}{0.19\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/lidar_point_clouds.png}
    {\small (b)}
  \end{minipage}
  \begin{minipage}{0.19\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/stitched_point_cloud.png}
    {\small (c)}
  \end{minipage}
  \begin{minipage}{0.19\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/filtered_point_cloud.png}
    {\small (d)}
  \end{minipage}
  \begin{minipage}{0.19\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/extracted_participants.png}
    {\small (e)}
  \end{minipage}
  \caption{\sysname deployment at a busy intersection with heavy vehicular and pedestrian traffic in a large metropolitan city. (a) A top down view of the intersection (taken from Google Maps~\cite{google_maps}. We mounted four LiDARs near each of traffic light poles situated at the four corners of the intersection. (b) An individual frame from each one of the 4 LiDARs. (c) A fused frame. (d) Point clouds of traffic participants (dynamic objects) at the intersection. (e) Bounding boxes and motion vectors for traffic participants, calculated over successive frames.}
  \label{fig:intersection_example}
\end{figure*}

\begin{figure*}
  \centering
  \begin{minipage}{0.20\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/fig_alignment_base.pdf}
    {\small (a)}
  \end{minipage}
  \begin{minipage}{0.20\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/fig_alignment_input.pdf}
    {\small (b)}
  \end{minipage}
  \begin{minipage}{0.15\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/fig_alignment_bg_removed.pdf}
    {\small (c)}
  \end{minipage}
  \begin{minipage}{0.1725\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/fig_alignment_distance_offset.pdf}
    {\small (d)}
  \end{minipage}
  \begin{minipage}{0.24\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/fig_alignment_rotation_offset.pdf}
    {\small (e)}
  \end{minipage}
  \caption{An illustration of \sysname's point cloud alignment algorithm. (a) A top down view of a parking lot with two LiDARs shown by red ($L_{1}$) and blue ($L_{2}$) icons. (b) The inputs to initial guess algorithm are point clouds ($C_{1}$ and $C_{2}$) in the respective LiDAR's coordinate system along with the ground distance $d$ between them. (c) Figure (b) with background removed. (d) To fix the base coordinates, \sysname displaces $C_{2}$ by the ground distance $d$. (e) \sysname rotates both $C_{1}$ and $C_{2}$ by small yaw increments to find the combination with the lease distance between the point clouds.}
  \label{fig:alignment}
\end{figure*}

% \parab{Goal and Challenge.} Perception must obtain the outputs from each frame of the input (a) in under 100~ms (perception should leave some of the latency budget for planning and for wireless transmission, we discuss this in \secref{sec:evaluation}), (b) while achieving localization and tracking accuracy comparable to the state-of-the-art. This is challenging because a single frame of the 64-beam Ouster LiDAR we use is over 3~MB. At 10~fps, this corresponds to 240~Mbps, uncompressed. Extracting precise semantic information from multiple LiDARs, in our example 4 LiDARs, at 1~Gbps within a tight latency budget requires (a) careful algorithmic and implementation choices, (b) exploiting properties of the setting.

\parab{Approach.}
%
To address the challenges described in \secref{sec:intro}, \sysname's perception uses a three stage pipeline, each with three sub-stages (\figref{fig:perception_stages}).
%
\textit{Fusion} combines multiple LiDAR views into fused frames, and then subtracts the static background to reduce data.
%
\textit{Participant extraction} identifies traffic participants by clustering and estimates a tight 3D bounding box around each object.
%
\textit{Tracking} associates objects across frames, and estimates their heading and motion vectors.

This design achieves \sysname's goals using three ideas:
\begin{itemize}[nosep,wide]
\item \sysname exploits the fact that LiDARs are static to cheaply \textit{fuse} point clouds from multiple overlapping LiDARs into a single \textit{fused frame}.
%
Such a frame may have more complete representations of objects than individual LiDAR frames.
%
\figref{fig:intersection_example}(b) shows the view from each of the 4 LiDARs; in many of them, only parts of a vehicle are visible.
%
\figref{fig:intersection_example}(c) shows a \textit{fused frame} which combines the 4 LiDAR frames into one; in this, all vehicles are completely visible.\footnote{Not immediately obvious from the figure, but a LiDAR frame, or a fused frame is a 3D object, of which \figref{fig:intersection_example}(c) is a 2D projection.}

\item \sysname builds most algorithms around a single abstraction, the 3D bounding box of a participant (\figref{fig:intersection_example}(e)).
%
Its tracking, speed estimation, and motion vector estimation rely on the observation that the centroid of the bounding box is a convenient consistent point on the object for estimating these quantities.
%
This is especially true for fused LiDAR frames that provide comprehensive views of an object.

\item \sysname uses, when possible, cheap algorithms rather than expensive deep neural networks (DNNs). Only when higher accuracy is required does \sysname resort to expensive algorithms, but employs hardware acceleration to meet the latency budget; its use of a specialized heading vector estimation algorithm is an example.

\end{itemize}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\columnwidth]{figs/stages_ver2.pdf}
  \caption{Perception stages. Bold sub-stags described in detail.}
  \label{fig:perception_stages}
\end{figure} 


\parab{Qualitative Design Comparison.} \sysname's perception design is qualitatively different (\tabref{tab:stack_comparison}) from that of other popular open-source autonomous driving stacks, Baidu's Apollo~\cite{BaiduSpecs} and Autoware~\cite{Autoware}:

\begin{itemize}[nosep,wide]
\item These approaches~\cite{BaiduSpecs,Autoware} rely on a pre-built HD-map, and localize the \textit{ego-vehicle} (the one on which the autonomous driving stack runs) by matching its LiDAR scans against the HD map (Apollo additionally improves position estimates using multi-sensor fusion). In contrast, \sysname \textit{does not require a map} for positioning: all vehicle positions can be directly estimated from the fused frame.

\item Autonomous driving stacks use different ways to identify traffic participants. Apollo extracts obstacles on a 2D occupancy grid and infers participants from contiguous occupied grids. Autoware uses 2D object detector on images, then back-projects these to the 3D LiDAR view. In contrast, \sysname directly extracts the 3D point cloud associated with each participant. It does this cheaply using background subtraction because its LiDARs are static.

\item Autonomous driving stacks use Kalman filters to estimate motion properties\footnote{Vehicles use SLAM to estimate their own motion and heading.} (speed, heading) of other vehicles. For heading, \sysname uses a more sophisticated algorithm to ensure higher tail accuracy.
\end{itemize}

We now describe parts of \sysname's novel perception relative to autonomous driving stacks (bold text in \tabref{tab:stack_comparison}). 

\subsection{Accurate Alignment for Fast Fusion}
\label{s:fusion}











\parab{Point Cloud Alignment.}
Each frame of a LiDAR contains a \textit{point cloud}, a collection of points with 3D coordinates. These coordinates are in the LiDAR's own frame of reference. Fusing frames from two different LiDARs is the process of converting all 3D coordinates of both point clouds into a common frame of reference. \textit{Alignment} computes the transformation matrix for this conversion.

Prior work has developed Iterative Closest Point (ICP)~\cite{chen91:_objec,bellekens2015benchmark} techniques that \textit{search} for the lowest error alignment. The effectiveness of these approaches depends upon the initial guess for LiDARs' poses. Poor initial guesses can result in local minima. SAC-IA~\cite{rusu09:_fast_point_featur_histog_fpfh} is a well-known algorithm to quickly obtain an initial guess for ICP. As we demonstrate in \secref{sec:evaluation}, with SAC-IA's initial guesses, ICP generates poor alignments on full LiDAR frames.






\parae{Initial guesses using minimal information.}
Besides the 3D point clouds, SAC-IA requires no additional input. We have developed an algorithm to obtain good initial guesses (that enable highly accurate ICP alignments) using minimal additional input. Specifically, \sysname only needs the distances on the ground (using, for example, an off-the-shelf laser rangefinder) between a reference LiDAR and all others to get good initial guesses.\footnote{LiDAR GPS locations as input result in poor alignment (\secref{sec:evaluation}).} We now describe the algorithm for two LiDARs $L_1$ and $L_2$ (as shown in \figref{fig:alignment}(a)); the technique generalizes to multiple LiDARs. 


The inputs are two point clouds $C_1$ and $C_2$ (more generally, $N$ point clouds captured from the corresponding LiDARs at the same instant (\figref{fig:alignment}(b) and \figref{fig:alignment}(c)), and the distance $d$ on the ground between the LiDARs. The output is an initial guess for the pose of each LiDAR. We feed these guesses into ICP to obtain good alignments. The algorithm conceptually consists of three steps:

\begin{mydescription}

\item[Fixing the base coordinates.]
Without loss of generality, set LiDAR $L_1$'s $x$ and $y$ coordinates to be $(0,0)$ (\ie base at origin). Then, assume that $L_2$'s base is at $(d,0)$ (\figref{fig:alignment}(d)). 

\item[Estimating height, roll and pitch.]
In this step, we determine: the height of each LiDAR $z_i$, the roll (angle around the $x$ axis),  and pitch (angle around the $y$ axis). For these, \sysname relies on fast \textit{plane-finding} algorithms~\cite{derpanis2010overview} that extract planes from a collection of points. These techniques output the equations of the planes. Assuming that the largest plane is the \textit{ground-plane} (a reasonable assumption for roadside LiDARs), \sysname aligns the $z$ axis of two LiDARs with the normal to the ground plane. In this way, it implicitly fixes the roll and pitch of the LiDAR. Moreover, after alignment, the height of the LiDARs $z_i$ is also known (because the $z$ axis is perpendicular to the ground plane).

\item[Estimating yaw.]
Finally, to determine yaw (angle around the $z$ axis), we use a technique illustrated in \figref{fig:alignment}(e). In this technique, \sysname rotates both point clouds $C_{1}$ and $C_{2}$ with different yaw settings until it finds a combination that results in the smallest 3D distance\footnote{The 3D distance between two point clouds is the average distance between every point in the first point cloud to its nearest neighboring point in the second point cloud.} between the two point clouds. We have found that ICP is robust to initial guesses for yaw that are within about 15-20$^\circ$ of the actual yaw, so \sysname discretizes the search space by this amount. In case of \figref{fig:alignment}(e), \sysname calculates the initial guess for the yaw by rotating the blue point cloud ($C_{2}$). 
\end{mydescription}






\sysname repeats this procedure for every other LiDAR $L_i$ with respect to $L_1$, to obtain initial guesses for the poses of every LiDAR. It feeds these into ICP to obtain an alignment. 

\parae{Re-calibrating alignment.} Because alignment is expensive, it is run only once, when installing the LiDARs. Re-alignment may be necessary if a LiDAR is replaced or re-positioned. Alignment is performed infrequently but is crucial to \sysname's accuracy (\secref{sec:eval-microbenchmark}).

\parab{Using alignment: Stitching.} LiDARs generate frames at 10~fps (or more). In \figref{fig:intersection_example}, when each LiDAR generates a frame, the fusion stage performs \textit{stitching}. Stitching applies the coordinate transformation for each LiDAR generated by alignment, resulting in a fused frame (\figref{fig:intersection_example}(c)).











\subsection{Reusing 3D Bounding Boxes}
\label{s:part-extr}

\sysname's efficiency results from re-using the \textit{3D bounding box} of a participant (\figref{fig:intersection_example}(e)) in many processing steps. After stitching, \sysname extracts the bounding box by performing \textit{background subtraction} on the fused point cloud to extract points belonging to moving objects, then applies \textit{clustering} techniques to determine points belonging to individual objects, and run a \textit{bounding box estimation} algorithm. These use well-known algorithms, albeit with some optimizations; we describe these in \secref{s:other-details}.


\parab{Using the 3D Bounding Box.} \sysname uses the bounding box for many of its algorithms (\tabref{tab:bounding_boxes}). Accurate alignment enables low complexity algorithms that use the pre-computed bounding box geometry. These algorithms are key to achieving low latency perception without compromising accuracy.

\begin{itemize}[nosep,wide]
\item To associate objects across frames (\textit{tracking}), it uses a Kalman filter to predict the position of the \textit{centroid} of the 3D bounding box, then finds the best match (in a least-squares sense) between predicted positions and the actual positions of the centroids in the frame.
Although tracking in point clouds is a challenging problem~\cite{vaquero2017deconvolutional} for which research is exploring deep learning, a Kalman filter works \textit{exceedingly well} in our setting. The biggest challenge in tracking is occlusions: when one object occludes another in a frame, it may be mistaken for the other in subsequent frames (an \textit{ID-switch}). Because our fused frame includes perspectives from multiple LiDARs, ID-switches occur rarely (in our evaluations, \secref{sec:evaluation}).

\item To estimate \textit{speed} of a vehicle, \sysname measures the distance between the centroid of the bounding box in one frame, and the centroid $w$ frames in the past ($w$ is a configurable window size parameter), then estimates speed by dividing the distance by the time to generate $w$ frames.

\item \sysname needs to associate an object seen in the LIDAR with a cyber endpoint (\eg an IP address) so its planning component can send a customized trajectory to each vehicle. For this \textit{cyber-physical association} (\figref{fig:perception_stages}), \sysname uses a calibration step performed once. In this step, given a vehicle for which we know the cyber-physical association (\eg LiDAR installer's vehicle), we estimate the transformation between the trajectory of the vehicle seen in the LiDAR view with the GPS trajectory (details omitted for brevity). \sysname uses this to transform a vehicle's GPS trajectory to its expected trajectory in the scene, then matches actual scene trajectory to expected trajectory in a least-squares sense. To define the scene trajectory, we use the centroid  of the vehicle's bounding box.
  
\end{itemize}

\begin{table}[t]
\small
\begin{tabular}{ccc|c|c}
\hline
  \multicolumn{3}{c|}{\textbf{Centroid}} &
  \textbf{Axes} &
  \textbf{Dimension} \\ \hline \hline
  \multicolumn{1}{c|}{Tracking} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Speed \\ Estimation\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}Cyber-Phy\\ Association\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Heading \\ Estimation\end{tabular} &
  Planning \\ \hline
\end{tabular}
\caption{\sysname computes bounding boxes for traffic participants early on and reuses properties of the bounding boxes in multiple modules to ensure low latency.}
\label{tab:bounding_boxes}
\end{table}


In all of these tasks, the centroid of the bounding box  is an easily computed, consistent, point within the vehicle that aids these tasks. Moreover, because we have multiple LiDARs that capture a vehicle from multiple directions, the centroid of the bounding box is generally a good estimate of the actual centroid of the vehicle.

Besides these, \sysname (a) estimates heading direction from the axes of the bounding box (discussed in \secref{s:tracking}) and (b) uses the dimensions of the box to represent spatial constraints for planning (discussed in \secref{s:planner}). 

\subsection{Fast, Accurate Heading Vectors}
\label{s:tracking}

Planning also needs the \textit{motion vector} to predict trajectories for vehicles. To compute this, \sysname first determines, for each object, its instantaneous \textit{heading} (direction of motion), which is one of the three surface normals of the bounding box of the vehicle. It estimates the motion vector as the average of the heading vectors in a sliding window of $w$ frames. Most autonomous driving stacks can obtain heading from SLAM or visual odometry (\secref{sec:related_work}), so little prior work has explored extracting heading from infrastructure LiDAR frames.


\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\columnwidth,frame]{figs/hv.pdf}
  \caption{The figure shows the points belonging to a car, in two successive frames $t$ and $t+1$. (a) Strawman approach for heading determination. (b) \sysname's approach.}
  \label{fig:heading}
\end{figure}

\parae{A strawman approach.}
Consider an object $A$ at time $t$ and time $t+1$. \figref{fig:heading}(a) shows the points belonging to that object. Since those points are already in the same frame of reference, a strawman algorithm is: (a) find the vector between the centroid of $A$ at time $t$ and centroid of $A$ at time $t+1$, (b) the heading direction is the surface normal (from the bounding box) that is most closely aligned with this vector (\figref{fig:heading}(a)). We have found that the error distribution of this approach can have a long tail (although average error is reasonable). If $A$ has fewer points in $t+1$ than in $t$ (\figref{fig:heading}(b), upper), the computed centroid will be different from the true centroid, which can induce significant error.

\parae{\sysname's approach.}
To overcome this, we (a) use ICP to find the transformation matrix between $A$'s point cloud in $t$ and in $t+1$, (b) ``place'' $A$'s point cloud from $t$ in frame $t+1$ (\figref{fig:heading}(b), lower), (c) then compute the vector between the centroids of these two (so that the centroid calculations are based on the same set of points). As before, the heading direction is the surface normal (from the bounding box) that is most closely aligned with this vector.

\parae{GPU acceleration.} ICP is compute-intensive, even for small object point clouds. If there are multiple objects in the frame, \sysname must run ICP for each of them. We have experimentally found this to be the bottleneck, so we developed a fast GPU-based implementation of heading vector estimation, which reduces the overhead of this stage (\secref{s:simul-results:-laten}).

A typical ICP implementation has four steps: (1) estimate correspondence between the two point clouds, (2) estimate transformation between two point clouds, (3) apply the transformation to the source point cloud and (4) check for the ICP convergence. The first step requires a nearest neighbor search; instead of using octrees, we adapt a parallelizable version described in~\cite{garcia2008fast} but use CUDA's parallel scanning to find the nearest neighbor. The second step shuffles points in the source point cloud then applies the Umeyama~\cite{umeyama} algorithm for the transformation matrix. We re-implemented this algorithm using CUDA's demean kernel, and a fast SVD implementation~\cite{gao2018gpu}. For the third and fourth steps, we developed custom CUDA kernels.


\subsection{Other Details}
\label{s:other-details}

\parab{Background Subtraction.}
\sysname removes points belonging to static parts of the scene\footnote{Static parts of the scene (e.g., an object on the drivable surface) might be important for path planning. \sysname uses the static background point cloud to determine the drivable surface; this is an input to the planner (\secref{s:planner}). We omit this for brevity.}. This is: a) especially crucial for voluminous LiDAR data, and b) feasible in our setting because LiDARs are static. It requires a calibration step to extract a \textit{background point cloud} from each LiDAR~\cite{kashani2015review}, then creates a \textit{background fused frame} using the results from alignment; taking the intersection of a few successive point clouds and the aggregating intersections taken at a few different time intervals, works well to generate the background point cloud.


\parae{Optimization: background subtraction before stitching.}
\sysname subtracts the background fused frame from each fused frame generated by stitching. We have found that a simple optimization can significantly reduce processing latency: first removing the background from each LiDAR frame (using its background point cloud), and then stitching points in the residual point clouds. Stitching scales with the number of points, which this optimization reduces significantly.

\parae{Optimization: exploiting LiDAR characteristics.} Many LiDAR devices only output \textit{returns} from reflected laser beams. Generic background subtraction algorithm requires a nearest-neighbor search to match a return with the corresponding return on the background point cloud. Some LiDARs (like the Ouster), however, indicate \textit{non-returns} as well, so that the point cloud contains the output of every beam of the LiDAR. For these, it is possible to achieve fast background subtraction by comparing corresponding beam outputs in a point cloud and the background point cloud.


At the end of these two steps, the fused frame only contains points belonging to objects that are not part of the scene's background (\figref{fig:intersection_example}(d)).

\parab{Computing the 3D bounding box.}
On the points in the fused frame remaining after background subtraction, \sysname uses a standard, fast, clustering algorithm
(DBSCAN)~\cite{ester1996density} to extract multiple clusters of points, where each cluster represents one traffic participant. Then, it uses an off-the-shelf algorithm~\cite{pclbbox}, which determines
a minimum oriented bounding box (\figref{fig:intersection_example}(d)) of a point cloud using principal component analysis (PCA). From these, we can extract the three surface normals of the object (\eg vehicle): the vertical axis, the axis in the direction of motion, and the lateral axis.















\iffalse


\subsection{Infrastructure-based Perception}

In this section, we detail one of the main contributions of \sysname: Infrastructure LiDAR-based \emph{real time} perception; this component is key to our proposed decoupling (\secref{sec:architecture}) of the state-of-the-art autonomous driving stack. We propose a novel perception algorithm that combines 3D point clouds from multiple geographically-distributed static LiDARs and processes a unified point cloud in real-time to enable fine-grain localization and tracking for autonomous driving. Note that \sysname does not plan the LiDAR placement; \sysname assumes that a deploying authority will use an intelligent topology planner to deploy a sufficient (say, $N$) number of LiDARs in a road intersection.

\ramesh{make sure to update \figref{fig:av_stack} with the components of the perception pipeline, or create a new figure.}


\ramesh{Create a new sub section. Call it design overview or \sysname overview. We have already talked about the architecture in the previous section.}
\parab{Overall Architecture.} 
Let us assume that a set of $N$ LiDARs are deployed in a designated intersection; each LiDAR generates a 3D point-cloud frame at a constant rate of $f$ frames per seconds (\ie 1 frame in every $T = 1/f$ seconds) and transfers it to the perception module of \sysname. In every $T$ seconds, \sysname's perception module processes the most recent set of $N$ frames (1 from each LiDAR) to detect any moving objects (\eg a car or a pedestrian) and to output the motion information of the detected objects; this is further fed to \sysname's planner module (\figref{fig:sys_overtaking}) to generate desired path trajectories for autonomous vehicles. To estimate accurate motion information in real-time, \sysname executes a one-time initialization step\footnote{We may need to re-invoke the initialization step if there is a dramatic change in the surroundings such as the spawning of a new building.} followed by a set of five sequential steps in every sensing period ($T$) as follows.

\ramesh{What do you have below is a great start! However, the overview section needs to be short and crisp. First, instead of having six different components, which is hard for a reader to keep in mind, can we describe the system as having three top level components, each of which we have two or more sub components? What would those be?}
\ramesh{Second, for each sub component start with the "what" (see detailed comments below), and have a brief sentence that describes the "how" and how the "how" is a novel contribution.}
\ramesh{For example, this is how I would describe the initialization component in an overview section. I would pick a better name, such as \textit{calibration} or even \textit{alignment}. (It is not clear that the step needs to be done only once. It may need to be done for example if the Lidar has moved for any reason). Then, the text would be something like: The position of a point in a LiDAR's point cloud is described in that LiDAR's frame of reference. In order to detect objects from multiple LiDARs, \sysname needs to ensure that all LiDAR point clouds are positioned within a common coordinate frame of reference. The alignment step, performed once initially and again whenever a LiDAR is reconfigured, adapts prior work on point cloud registration to be robust to settings, such as ours, when the point clouds are captured from vastly different perspectives.}
\ramesh{Also, if we are claiming alignment to be a contribution, let's find a name to describe it.}

\parag{Initialization.} To efficiently detect the dynamic objects and extract the respective motion information, \sysname needs two basic information: (1) Pair-wise transformation matrices between LiDARs and (2) a background point cloud. In addition, \sysname needs to detect drivable Space to plan the autonomous vehicle trajectories. 

We need the pair-wise transformation matrix to fuse the 3D sensory data from multiple LiDARs into a unified point cloud. Each LiDAR point cloud is represented by its own (and independent) frame of reference (or coordinate system). To combine two LiDAR point clouds, we apply coordinate transformation from one's point cloud to the other; a pairwise transformation matrix is a key to this. Estimation of the transformation matrices takes several minutes and can be done offline as the LiDARs are static. To this, \sysname completes a \emph{Point Cloud Alignment} process as a part of the initialization (detailed below).

A \textit{background point cloud} is a point cloud frame that represents the static background of a sensed region (such as roads, buildings, and traffic signs). \sysname compares a point cloud frame with a background point cloud to identify dynamics objects (such as cars and humans). In a real-world setting, it is challenging to find an empty scene without any dynamic objects to generate a background point cloud. A trivial approach can take an intersection of multiple consecutive frames; however, this may include temporary static objects such as a parked vehicle. 
To this, we take an intersection of $P$ temporally isolated frames to completely filter out dynamic points and form a \emph{common frame}.  A single common frame is, yet, not a robust representation of the background point cloud; it might be missing a significant subset of background static points~\cite{kashani2015review} due to either temporary obstructions or LiDAR hardware issues. To solve this practical problem, we generate $Q$ temporally distributed common frames and aggregate them to form the final background point cloud. 
The background point cloud construction takes a significant amount of time and only needs to be updated after a dramatic change in the surroundings such as the spawning of a new building. Therefore, \sysname performs the \textit{Background Point Cloud Construction} as a part of the initialization.
\pradipta{What are the typical values of P and Q?}
\pradipta{minor comment: can we come up with a meaningful name instead of "common frame"?}
\ramesh{I noticed that we discuss point cloud alignment in more detail in a later section. Let's move the above paragraph to that section. The principle is that in this overview section, we should be discussing \textit{what} we do, not \textit{how} we do it}

Lastly, for the planner module to design trajectories, we need to inform the planner where vehicles can drive safely and legally.
\pradipta{Please write the drivable space extraction part here.}
\pradipta{Also, can we add an illustrative image for each of the steps?}
\christina{Yes, I think that is a good idea! I will make corresponding images and update the paper.}


\parag{Stitching.} After proper initialization, the first step of \sysname's perception module is to stitch the most-recent $N$
\ramesh{Shouldn't this be: the most recent frame from each of the $N$ different LiDARs?} frames from different LiDARs into one unified frame; we call this a \textit{stitched point cloud frame}. Each LiDAR's 3D frame is presented in its coordinate systems. \sysname applies a linear coordinate transformation to each frame with the respective transformation matrix (obtained from \textit{Point Cloud Alignment}) to aggregate them into the stitched point cloud frame. The stitched point cloud presents a full view of the scene; it aggregates information about everything detected by the LiDARs such as ground planes, buildings, and vehicles. We further detail the stitching process below.

\ramesh{Rewrite the previous paragraph to describe the what before the how. The last sentence gets close to the how.} 
\ramesh{Also, as you write, keep in mind that the why is also an important consideration. We should discuss why we do stitching, and what other options are possible. The Overview may not be the best place to do this, it might be better to describe the why closer to the how.}

\parag{Background filtering.} In the second step, \sysname's perception module filters out all points residing in the background and extracts only dynamics object (in our case mainly vehicles) by simply removing the overlapping points between the stitched point cloud and the background point cloud (obtained from the \textit{Background Cloud Construction}). This is sufficient in our setting as the LiDARs are fixed and the background points are mostly static; this is quite different from traditional autonomous vehicle systems with moving LiDARs.

\parag{Clustering.} After background filtering, the stitched point cloud only contains dynamic objects. Assuming there exists no dynamic object other than vehicles, \sysname's perception module performs a \textit{Density-based Spatial Clustering with Noise} (DBSCAN)~\cite{ester1996density} to extract multiple clusters where each cluster corresponds to a vehicle.

\parag{Tracking/Association.} Following the clustering step, \sysname examines the clusters to associate vehicle identities; this is required to persistently track the same vehicles in-between frames. We propose a Kalman filtering~\cite{kalman1960new} based method to find the correct correspondences between the current set of detected vehicles and the vehicles detected in earlier frames and to perform a consistent tracking of individual vehicles. The tracking algorithm also outputs the location of a consistent reference point for each vehicle. This is further detailed later on.


\parag{Motion estimation.} In the last step, \sysname's perception module estimates the movement state of each vehicle. With the estimated location of a reference point of the vehicle (obtained from \textit{Tracking/Association}), \sysname estimates three different parameters to completely represent a vehicle's motion: (1) the oriented bounding box of the vehicle, (2) the instant heading direction, and (3) the motion vector over a time window. The location of a reference point and the bounding box summarize the dimensions of a vehicle and the location (position and orientation) in the stitched 3D frame. In addition to the localization information, we need the heading direction and the motion vector to characterize the motion of each vehicle in the current stitched 3D frame. We use the term, \textit{heading direction}, to infer an instantaneous heading direction at the time. On the other hand, a \textit{motion vector} embodies the velocity and the heading direction of a vehicle averaged over a short period of time. How \sysname estimates these parameters is further explained in details below.



\parab{Tracking.}
In this section, we detail our proposed vehicle tracking method based on infrastructure based LiDARs. After the object clustering step (see above), \sysname's perception module assigns an unique ID to each detected object in the scene. The main goal of this step is to identify inter-frame associations and detect same objects over the consecutive frames. Lack of semantic information poses an intrinsic challenge to multi-objects tracking in 3D point cloud as compared to 2D image data~\cite{vaquero2017deconvolutional}. Nonetheless, 3D data is often enriched with geometry information. Researchers often apply \textit{Kalman filtering}~\cite{kalman1960new} or \textit{Hungarian algorithm}~\cite{kuhn1955hungarian} on such geometric data for accurate and fast tracking~\cite{}; the performance of such methods are vulnerable to occluded objects or incomplete point clouds. Interestingly, \sysname do not suffer from such incomplete point cloud problem since we leverage stitched point clouds from multi-LiDARs that capture a more complete picture of the scene.
\christina{Note-to-myself: Need to add kf tracking citations}

\ramesh{please consider re-organizing the above paragraph according to the template discussed for alignment: A few sentences on the problem, A few on prior work, A few sentences describing why is the prior work falls short, and a few sentences that describe the key idea behind our approach.}
\ramesh{the last sentence is good, but we need to discuss how stitched point clouds help. Do they let us design a cheaper algorithm? Or do they give higher accuracy when we use an existing algorithm?}
\ramesh{To the algorithm description below, let's try to answer them contextual information: how similar or different is it from standard ways of doing tracking?}
\ramesh{Also, in the rewrite, we should explicitly mention clustering in this section, otherwise readers will not be able to match the description in the overview to the tracking section.}

\sysname adopts Kalman filtering to track objects and assign corresponding IDs with a simple distance-based scheme. Based on previous history of identified objects, our algorithm applies Kalman filtering to first calculate the expected/estimated positions of the tracked vehicles (\ie vehicles identified in earlier frames). On the other end, \sysname observes a set of vehicles in the current point cloud frame and outputs their clusters. For the purpose of ID assignment, we represent each vehicle by the centroid of the object's cluster in the point cloud; we use these also as the \textit{reference points} for each tracked vehicles. Now, let us denote the estimated positions of $u$ tracked objects as $e_1, e_2, ..., e_u$ and the observed positions of $v$ objects as $o_1, o_2, ..., o_v$, respectively. Lastly, we introduce a distance matrix $D$ where $D_{ij}$ is the Euclidean distance between $e_i$ and $o_j$. With this, the tracking problem is converted into a matching like problem; we use distance metrics to match the estimated locations with the observed locations. Our algorithm finds an assignments $A = \{a_{ij}\}$ that minimizes the summation of distance of assignments as follows:


\begin{flalign*}
&\textrm{Minimize}  \hspace{10mm} \sum_{i=1}^{u}\sum_{j=1}^{v}D_{ij}a_{ij} && \\
&\textrm{Subject to} \hspace{10mm} \sum_{i=0}^{u}a_{ij} = 1, \forall j \in \{1, \cdots, v\} &&\\
& \hspace{23mm} \sum_{j=0}^{v}a_{ij} = 1, \forall i \in \{1, \cdots, u\}  &&
\end{flalign*}
\pradipta{The equations did not seem right. I modified it based on my understanding. Please check.}
\pradipta{The cost function seems bit weird to me. This will force to minimize the sum of distance. Then the solution will be all $a_{i0} = 1$ and $a_{0j} = 1$. To circumvent this, typically a large cost is added for the 0 assignment case. But even then the problem will be it will always try to assign a matching even though there is no correlation. I guess the best cost function would be to use $D_{i0}$ and $D_{0,1}$ to be a threshold distance for matching. Maybe you are already doing that. But please check.}
\christina{Yes, I get your point. Our current implementation is using the distance threshold (5m) for the matching so maybe we need to add what you suggested? Also, other than that, I was wrong on the equation and the changed one makes sense!}
\pradipta{I see. In that case, please update the equation and the description.}
Here, $a_{ij} = 1$ implies estimated object $e_i$ is matched to observed object $o_j$. If an estimated object $e_i$ is not matched with any observed object, $a_{i0} = 1$. Similarly, if $o_j$ is not matched with any estimations, then $a_{0j} = 1$. The optimization function makes sure that the closest pair is matched together while the constraints ensures each estimation is associated with no more than one observation, vice versa.

After solving this optimization, we should have correct ID assignment to each vehicles. We feed the output \ie a list of tracked object ID with their respective reference points ($o_j$) to the motion estimation and planning module.



\parab{Cyber-physical association.}
\weiwu{Placeholder}

\parab{Motion Estimation.}
The last step of our perception module is \textit{motion estimation}. The motion estimation procedure estimates the three different components of the current motion state (detailed above) of the detected objects: (1) the oriented bounding box of the vehicle, (2) the instant heading direction, and (3) the motion vector over a time window. This data is directly fed to \sysname's planning module and used to generate trajectory plans for each vehicle. The collected LiDAR data is very time-sensitive with regards to trajectory (path) planning; our proposed algorithm, therefore, aims to complete the motion estimation in real-time while maximizing the accuracy.

\ramesh{As with other sections, this is a very nice start. Please follow the comments I have given in the other sections to re-write the section. In particular, for this audience we need to help them understand what is novel relative to prior work, and what kinds of trade-offs we have made.}


\parag{Bounding box estimation.} Our motion estimation starts with bounding box estimation. As implemented in \cite{pclbbox}, a minimum oriented bounding box of a given vehicle is extracted by using eigenvectors and covariance matrix of the point cloud. Based on the extracted bounding box, our algorithm estimates three surface normals (i.e., front direction, side direction, and upper direction) of the bounding box; these are fed to the next step to select the correct normal vectors as a heading direction of the vehicle.

\parag{Heading direction estimation.} After the bounding box estimation, our algorithm selects one of three surface normals estimated in the bounding box estimation step to represent the heading direction of each vehicle. To filter out the heading direction of the vehicle at time $t$, our algorithm fetches a point cloud of the vehicle at time $t-1$ and compares it with the point cloud at $t$; this gives us a vehicle's moving direction from time $t-1$ to $t$. To this, we simply calculate the vector ($\overrightarrow{dv}_t$) between the vehicle's reference points (centroid) at time $t$  and at time $t-1$: $\overrightarrow{dv}_t = \overrightarrow{c_t} - \overrightarrow{c_{t-1}}$, where $\overrightarrow{c_t}$ and $\overrightarrow{c_{t-1}}$ are the 3D position vectors for the vehicle centroid at time $t$ and $t-1$, respectively. Next, we compare the direction of $\overrightarrow{dv}_t$ with the three surface normals of the vehicle and select the one with the most similarity with $\overrightarrow{dv}_t$. This method works under the assumption that the vehicle's moving direction from $t-1$ to $t$ is not much different from the vehicle's instant heading direction at $t$.

To get an accurate $\overrightarrow{dv}_t$, we first run ICP algorithm to align the point cloud of the vehicle at time $t-1$ with the point cloud of the vehicle at time $t$. Next, we use the original point cloud at $t-1$ and the aligned point cloud to robustly calculate $\overrightarrow{dv}_t$.
\pradipta{From the meeting, if I remember correctly, the point cloud here is only for the vehicle; not the entire frame. Right? If so, we need to make it clear.}
\christina{Yes. I simply changed to "point cloud of the vehicle". Do we need more explanation?}
\pradipta{Should be fine I guess. But there is a slight disconnect in the write up then bcoz all of a sudden you are talking about vehicle point cloud instead of the whole point cloud. Ramesh will have better idea about this.}

\parag{Motion vector estimation.} For the last step in our motion estimation, our algorithm tracks a motion vector. We can decompose the motion vector into two sub-components; direction and magnitude of the vector. Direction of the motion vector indicates an averaged heading direction over a given time window, $w$, and we interpret it to a heading trend within the time window \pradiptas{What do you mean here?}. Magnitude of the vector is nothing but the average speed over the time window $w$. Our algorithm estimates the direction of the motion vector by simply averaging the estimated heading direction over $w$. To get the magnitude of the motion vector, our algorithm fetches another point cloud of the vehicle which is $w$ frames ahead and runs ICP to align them. Similar to the heading vector estimation above, we calculate a displacement vector $\overrightarrow{dv}_t$ for the vehicle from time $t-w$ to time $t$ and set $|\overrightarrow{dv}_t|$ as the magnitude of the motion vector.
\christina{I mean the direction of the vector is somehow averaged heading direction. Can you help to make it more clear?}
\pradipta{But I thought the displacement vector direction is the motion vector direction. Is it not? How are you averaging the direction otherwise?}
We notice that our proposed motion estimation is vulnerable to noisy data from sensor faults and such noisy data is quite common in real-world data collection. To filter out such noises, we adopt Kalman filtering. \sysname maintains a separate Kalman filter model for each detected vehicle. Instead of outputting the instantaneous motion vector, our algorithm feeds the newly estimated motion vector to the Kalman filter and outputs a less noisy motion vector.


\fi


==> planner.tex <==
\section{\sysname Planning}
\label{s:planner}

% \fawad{I think I'll add a diagram here to show how different sub-modules work in the controller.}
% \sysname's controller module uses positions, bounding boxes and motion vectors along with a drivable space map from the perception module to control \sysname-compatible vehicles. The control module consists of the three sub-modules \ie the centralized planner at the edge for motion-planning, and the local low-level controller along with a PID controller at the vehicle which convert those paths to low-level vehicle controls (\eg steering wheel angle, throttle, and brake).

\parab{Inputs, Outputs, and Goals.}
From perception, \sysname's planning component receives bounding boxes for non-background objects, and their motion vectors. Some of these objects will be \sysname-capable vehicles\footnote{These are determined during cyber-physical association (\secref{s:part-extr}).}~---~these will follow trajectories designed by \sysname. For these, \sysname needs each vehicle's navigation goal, \eg where it is headed: we assume the planning component can get this by communicating with the vehicle. Other objects will be \sysname-oblivious: these include pedestrians, or vehicles driven by humans or on-board autonomous driving agents. The output of planning is a trajectory\footnote{To generate these trajectories, \sysname also needs a map of the drivable space (including road surface, lane markers and driving direction). These can either be obtained by scene analysis~\cite{background_filtering,lanedetection}, or from a one-time human annotation.}~---~a sequence of way-points, and times at which those way-points should be reached~---~for each \sysname-capable vehicle.

Planning executes at every frame and must satisfy two goals: (a) its decisions must fit within the end-to-end tail latency budget of 100~ms, (b) and it must generate collision-free trajectories at every instant, even in the presence of \sysname-oblivious objects.

% \parab{Goals and Requirements. } The controller must ensure collision-free driving for all \sysname-compatible vehicles with low latency in all deployment scenarios (\secref{sec:deployment}). The controller must support user-imposed traffic policies \eg prioritizing emergency vehicles, reducing traffic congestion \etc.

% \ramesh{the second sentence is good, but comes out of the blue. We might want to figure out whether we want to justify this requirement either here or earlier in the introduction or the arch section.}

\parab{Prior Work in Planning.} Motion planning is a large and mature field of research. In this paper, we do not seek to innovate in this space, but merely to demonstrate the existence of a fast planner that meets our objectives. Autonomous vehicles today use decentralized motion planning algorithms that search for paths in graphs ($A^{*}$~\cite{Astar}, Safe Interval Path Planning (SIPP)~\cite{SIPP}, and Dijkstra~\cite{Dijkstra}). \sysname requires a centralized motion planner, the best known of which is \eg Conflict Based Search~\cite{CBS}; but, this algorithm has high tail latency~\cite{cbslatency, SIPP}.

\parae{SIPP.}
In \sysname, we build upon a fast planner for a single robot for environments with dynamic obstacles, SIPP~\cite{SIPP}. A dynamic obstacle is one whose position changes over time. SIPP discretizes space into a 2D occupancy grid (\figref{fig:planning_examples}(a)) and plans a path for a given robot from a one location (source) to another (destination). Planning in dynamic environments adds an extra dimension \ie time, to the search space which can increase computational complexity. SIPP's efficiency relies on the following intuition. Consider an arbitrary grid element (\eg a square on the road surface). The time steps ($t_{1}, t_{2}, ...., t_{n}$) that this element is \textit{safe} for robot occupancy (meaning no other robot occupies it at that time) is unbounded and infinitely large. However, the number of time intervals ($[t_{1}, t_{n}]$) at which that location is safe is bounded and generally small. A (maximally) safe time interval ($[t_{1}, t_{n}]$) in one in which the location is safe for occupancy throughout the interval, but not safe one step before ($t_{0}$) and one step after ($t_{n+1}$) the interval.

The input to SIPP is a goal for a robot and the positions over time of the dynamic obstacles in the environment. Using the latter, SIPP first generates a sequence, for each grid element, of safe and unsafe intervals. Then, using the former, SIPP uses $A^{*}$ search to find a provably collision-free shortest path for the robot~\cite{SIPP}.

\parab{\sysname's Planner.} At each frame, \sysname must plan trajectories for every \sysname-capable vehicle. Without loss of generality, assume that vehicles are sorted in some order. \sysname's centralized planner runs SIPP for each vehicle in order; when running SIPP on the $i$-th vehicle, \sysname represents all $i-1$ previously planned vehicles as dynamic obstacles in SIPP. For example, when planning for the second vehicle, it represents the first vehicle as a dynamic obstacle (\figref{fig:planning_examples}(b)).

This approach may sacrifice optimality for speed: vehicles later in the planning order may see longer transit times. However, the approach may allow \sysname to achieve traffic policies that rely on prioritization (\eg prioritizing emergency vehicles). We have left it to future work to explore such traffic policies, and to design fast planning algorithms that can accommodate other traffic management policies.

% \begin{figure*}
%   \centering
%   \begin{minipage}{0.19\linewidth}
%     \centering
%     \includegraphics[width=\columnwidth,frame]{figs/intersection_example_a.pdf}
%     {\small (a)}
%   \end{minipage}
%   \begin{minipage}{0.19\linewidth}
%     \centering
%     \includegraphics[width=\columnwidth,frame]{figs/intersection_example_b.pdf}
%     {\small (b)}
%   \end{minipage}
%   \begin{minipage}{0.19\linewidth}
%     \centering
%     \includegraphics[width=\columnwidth,frame]{figs/intersection_example_c.pdf}
%     {\small (c)}
%   \end{minipage}
%   \begin{minipage}{0.19\linewidth}
%     \centering
%     \includegraphics[width=\columnwidth,frame]{figs/intersection_example_d.pdf}
%     {\small (d)}
%   \end{minipage}
%   \begin{minipage}{0.19\linewidth}
%     \centering
%     \includegraphics[width=\columnwidth,frame]{figs/intersection_example_e.pdf}
%     {\small (e)}
%   \end{minipage}
%   \caption{(a) A bird's eye view of an intersection. LiDARs are mounted on the traffic light poles at each of the four corners of the intersection. (b) An individual frame from each of the 4 LiDARs. (c) A fused frame. (d) Point clouds of traffic participants at the intersection. (e) Bounding boxes and motion vectors for traffic participants, calculated over successive frames.}
%   \label{fig:intersection_example}
% \end{figure*}

\begin{figure}[t]
  \centering
  \begin{minipage}{0.325\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/planning_example_a.pdf}
    {\small (a)}
  \end{minipage}
  \begin{minipage}{0.325\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/planning_example_c.pdf}
    {\small (b)}
  \end{minipage}
  \begin{minipage}{0.325\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/planning_example_b.pdf}
    {\small (c)}
  \end{minipage}
  \caption{\sysname planning examples. (a) The first (red) planned vehicle can use the entire drivable space. (b) The second (blue) planned vehicle cannot occupy grids planned for the first (the different shades represent different times at which grids are occupied). (c) The motion-adaptive buffer around a vehicle is proportional to its speed.}
  \label{fig:planning_examples}
\end{figure}

Because it was designed for robots, SIPP makes some idealized assumptions. The following paragraphs describe these, and explains how \sysname adapts SIPP to relax these assumptions. We also describe how \sysname must also be robust to losses of trajectories transmitted to \sysname-capable vehicles, as well as to errors in perception (error in bounding box sizes, motion vectors, heading estimation).

\paraspace\noindent$\blacktriangleright$
SIPP plans the entire trajectory for a robot, given all the dynamic obstacles in the environment. \sysname, because it must compute trajectories for all vehicles, including \sysname-oblivious vehicles whose trajectories can change dynamically, re-plans trajectories for every \sysname-capable vehicle at every frame. 

\paraspace\noindent$\blacktriangleright$
SIPP assumes (a) that each object has the same size, occupying one grid element, (b) that each object moves at a fixed speed, and (c) that it can start and stop instantaneously. To relax, (a) \sysname uses the bounding boxes generated by perception to determine grid occupancy. Because these bounding boxes may be incorrect, \sysname extends the bounding box by a small buffer on all sides. This extended buffer is \textit{motion-adaptive}: the faster the vehicle travels the larger is the buffer around it (\figref{fig:planning_examples}(c)).

To relax (b) and (c), \sysname generates waypoints over a longer horizon (10~s) than the inter-frame time (100~ms in our case). This addresses two issues. First, it transmits trajectories every hundred milliseconds, but if they are lost, the vehicle can use the previously-received trajectory\footnote{If there is a catastrophic failure, \sysname-capable vehicles must have a fallback-to-human strategy; autonomous driving will also need this.}. Second, instead of having to implement instant start and stop, the longer time horizon gives the vehicle's controller time to adapt to the vehicle's kinematic characteristics. The controller can determine, from the received trajectory, if it has to stop at some future point in time; it can then determine when to apply the brakes, and with what pressure, to effect the stop.
%\pradipta{how it resolves the fixed speed issue is not clear to me from this paragraph}

\paraspace\noindent$\blacktriangleright$
SIPP assumes that it is given the dynamic objects in the environment. For \sysname-capable vehicles that it has already planned trajectories for, \sysname knows their trajectories, and can represent them as dynamic obstacles when planning a trajectory for a vehicle. For each \sysname-oblivious object, \sysname uses its bounding box, and motion and heading vector; it assumes that these objects will move at the same speed, with the same heading over the 10~s planning horizon and generates a dynamic obstacle based on this assumption.

\secref{s:centralized-planner} describes the planner in detail, and \secref{s:local-controller} describes extensions to the on-board controller to enable \sysname to respect the vehicle's kinematic constraints.

% use on-board planning and control modules to plan motion and follow collision-free paths to reach their destinations. Since every vehicle plans for itself, work in industry and academia has focused on decentralized motion planning algorithms ($A^{*}$~\cite{Astar}, Safe Interval Path Planning (SIPP)~\cite{SIPP}, and Dijkstra~\cite{Dijkstra}). Centralized algorithms (\eg Conflict Based Search (CBS)~\cite{CBS}) for multi-robot/agent planning exist but, in practice, they have been used in more controlled environments like warehouses and are known to have large tail latencies~\cite{cbslatency, SIPP}. To this end, \sysname uses a decentralized low-latency algorithm, SIPP, in a centralized manner for motion planning.

% \ramesh{we might want to add a citation for the tail latencies.}
% \fawad{Addressed.}

\iffalse

% \textit{Challenges. }
\parab{SIPP. }
Planning in static environments is a well-studied problem that can be solved efficiently. Planning algorithms discretize space into a 2D occupancy grid and plan a path for a given robot from a one location (source) to another (destination). Planning in dynamic environments adds an extra dimension \ie time, to the search space and this increases computational complexity. SIPP is a graph-search algorithm for dynamic environments that is based on the following intuition. Although the \textit{time steps} ($t_{1}, t_{2}, ...., t_{n}$) that a given location in the occupancy grid is safe for robot occupation is unbounded and infinitely large; the number of \textit{time intervals} ($[t_{1}, t_{n}]$) at which that location is safe is bounded and generally small. A safe \textit{time interval} ($[t_{1}, t_{n}]$) in one in which the location is safe for occupation throughout the interval, but not safe one step before ($t_{0}$) and one step after ($t_{n+1}$) the interval. To scale, for every location in the 2D occupancy grid, SIPP discretizes time into contiguous safe and unsafe \textit{time intervals} or states. Squares with static obstacles \eg the sidewalk are unsafe eternally whereas others like the road have multiple safe and unsafe states. This allows SIPP to compactly represent each location with a few states. With this representation, SIPP solves the graph-search problem using $A^{*}$ search.

\ramesh{the above description is good, but you might want to add more academic language: to scale, SIPP discretizes space and time etc. Give the intuition behind what enables it to scale, and then describe how the algorithm works.}
\fawad{Addressed.}

\parab{Centralized Planning with SIPP. }
\sysname uses SIPP in a greedy, sequential manner for centralized control. Consider the full-deployment scenario (\secref{sec:deployment}). In this, \sysname first plans for a single vehicle with SIPP using only the static environment. Then, it uses the SIPP-generated path for first vehicle as a dynamic obstacle for the second vehicle. This way, the second vehicle can avoid static obstacles and the first vehicle. The third vehicle uses both the first and second vehicles as dynamic obstacles and so on. This way, \sysname can plan for all vehicles in a centralized manner using sequential SIPP.

\sysname uses a greedy approach for planning as opposed to an optimal approach like CBS for two reasons: a) latency, and b) flexibility. Optimal approaches tradeoff planning time (latency) to ensure robots reach their destinations in the minimum amount of time. In our case, a lower planning time (to meet the 100~ms latency budget), guaranteed by a greedy approach, is more important. Second, an optimal approach achieves a single goal \ie minimum overall trip time. With a greedy approach, \sysname creates opportunities support different types of user-defined traffic policies. For instance, besides minimizing trip times, it can prioritize emergency vehicles, ensure fair waiting times for all vehicles, ameliorate traffic congestion on a given road \etc.
% \sysname uses a greedy approach as opposed to a more optimal approach like CBS for the following reasons. Optimal approaches tradeoff have higher planning times to ensure all robots reach their destinations in the minimum amount of time. In our  case of autonomous driving, a lower planning time (to meet the 100~ms latency budget) is more important than time to plan is more important    is more important than First, although, the greedy approach does not guarantee an optimal solution, it  the greedy approach ensures that we reach a solution faster. Optimal  Instead of a greedy approach, we could have used an We could have used a more optimal approach for planning (\eg Conflict Based Search) We use a greedy approach in \sysname (as opposed to an optimal approach like CBS)  
% 1. For latency
    % CBS run times are higher so we can only use it once. It will have to be updated and run every step which makes it very expensive
    % Even if the environment changes, we can run SIPP over and over again because it has a lower cost
% 2. For user defined traffic policies
%   
% As opposed to a greedy approach, \sysname could have used an optimal algorithm like Conflict Based Search. 

% A centralized controller, as opposed to decentralized controllers today, creates opportunities for cross-car optimizations and impose user-defined traffic policies (as we show later).

\ramesh{similar comment here. First say that we run SIPP in a greedy manner, planning for each vehicle in turn, while treating previously planned vehicles as obstacles. When you say this, people will expect a discussion of why you chose greedy: fast versus non-optimal.}
\fawad{Addressed but still thinking about how to improve it}

\parab{Challenges. }
SIPP solves a graph-search problem to plan a path for a vehicle from source to destination without any regard to real-world vehicle physics and traffic regulations. In doing so, it makes assumptions that do not hold true in the real-world. For instance it assumes that: a) vehicles can stop/start moving instantly, b) vehicles move with uniform speed, c) vehicles can move in all directions, d) vehicles occupy a single square on the occupancy grid, and e) the controller knows the location of every dynamic obstacle on the occupancy grid. To use SIPP in a realistic scenario, \sysname must relax these assumptions. 

Secondly, though SIPP is faster than other centralized algorithms, it takes upto 1~second to complete a single planning cycle. Moreover, this time increases with the number of vehicles that it must plan for. \sysname must enable SIPP to scale to a large number of vehicles and reduce the time for a single planning cycle.

\parab{\sysname's Approach. }
% Three contributions
% Splitting functionality / parallelism
To add support for real-world dynamics, \sysname must balance two competing constraints. \sysname's controller needs additional functionality to understands real-world dynamics. However, this functionality increases computational complexity and increases latency. To achieve both goals, \sysname divides the control module into two sub-modules and distributes the additional functionality between them. This includes a centralized planner resides at the edge and a low-level controller on-board every vehicle. The centralized planner runs the SIPP planning for all vehicles. It then sends a set of waypoints to the on-board low-level control module which converts them to the steer angle, throttle and brake. 

% Real-world dynamics
An out-of-the-box SIPP algorithm only uses robot positions as inputs for planning. To add support for real-world scenarios, \sysname's centralized planner makes use of the motion vectors and bounding boxes of vehicles from the perception component. The centralized planner uses motion vectors to model motion and the bounding boxes to model the realistic size of every vehicle in SIPP. Similarly, the low-level control module, converts the output (designed for a robot that can start/stop instantly) from the planner to a realistic path that vehicle can follow. To do this, it uses the set of waypoints and vehicle dynamics (\eg braking force and acceleration).

% Latency requirement
Lastly, \sysname makes optimizations to SIPP that enable it to run a planning cycle within 10~ms for low-latency planning. This way \sysname can run the centralized planner at LiDAR frame rate. As we discuss later, this makes \sysname more robust to unexpected changes in the environment (\eg unexpected driver, pedestrian or cyclist behavior).

% these waypoints to  Then, it sends    Then, it adds functionality to \sysname adds functionality to the controller that enable it to understand real-world dynamics. It splits this into two sub-modules: a) a centralized planner, and b) a local low-level control module. 

% First, \sysname uses SIPP planning at LiDAR frame rate instead of single-shot planning. Second, \sysname adds functionality to the controller that enable it to understand real-world dynamics of vehicles and road regulations. It splits this functionality between the edge (centralized controller) and the vehicle (local planner).

\ramesh{The LIDAR and single shot planning comes out of the blue; there is nothing in the prior text that prepares the reader for this. At this point, the reader is expecting some description of how you relax the assumptions. Also, it is unclear what problem functionality splitting solves.}
\fawad{I changed the entire approach because I missed out on many points. Please check it now}
% in SIPP to help it understand the real-world dynamics of a vehicle \eg its size and momentum. Last, \sysnam 
% whereas dynamic object   
% are used, \sysname controls multiple     a planning module along with a control module to control the motion of the vehicle. The planning module performs two functions: a) it plans a collision-free path for a vehicle from source to destination (path-planning) and b) it plans the motion of the vehicle to follow that path (motion-planning). The control module converts that motion to low-level control signals that the vehicle can understand. 

\begin{algorithm}[t]
  \caption{Centralized Planner}
  \label{algo:controller}
\SetKwFunction{CalculateDrivableSpace}{CalculateDrivableSpace}
\SetKwFunction{QueryPerception}{QueryPerception}
\SetKwFunction{MotionEstimation}{MotionEstimation}
\SetKwFunction{MotionAdaptiveBuffer}{MotionAdaptiveBuffer}
\SetKwFunction{AddDynamicObstacles}{AddDynamicObstacles}
\SetKwFunction{SippPlanning}{SippPlanning}
\SetKwFunction{RecoveryMode}{RecoveryMode}
\SetKwFunction{AddStaticObstacles}{AddStaticObstacles}
\SetKwFunction{GenerateIntervals}{GenerateIntervals}
\SetKwFunction{PriorityFunction}{PriorityFunction}
\SetKwFunction{Append}{Append}
\SetKwFunction{SendOverNetwork}{SendOverNetwork}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{\sysname-compatible objects $V_{C}$ \\ Non-compatible objects $V_{E}$ \\ Stitched point cloud $S$}
% ${Vehicle poses $P$, bounding boxes $B$, motion vectors $M$ and stitched point cloud $S$} % P for the set of point clouds and G for the set of gps tags
\Output{Vehicle trajectories $W$ for $V_{C}$}
\BlankLine
$P_{C}, M_{C}, B_{C} \leftarrow $ \QueryPerception ( $V_{C}$ ) \\ % Query perception for ego-vehicles
$P_{E}, M_{E}, B_{E} \leftarrow $ \QueryPerception ( $V_{E}$ ) \\ % Query perception for non-ego vehicles
$S_{D} \leftarrow $ \CalculateDrivableSpace {$S$} \\
$C. $ \AddStaticObstacles { $S_{D}$ } \\
% \ForEach { $v_{i}$ in $V_{E}$, $p_{i}$ in $P_{E}$, $m_{i}$ in $M_{E}$, $b_{i}$ in $B_{E}$ }
\ForEach { $v_{i}$ in $V_{E}$ } %, $p_{i}$ in $P_{E}$, $m_{i}$ in $M_{E}$, $b_{i}$ in $B_{E}$ }
{
    $t_{i} \leftarrow$ \MotionEstimation { $p_{i}$, $m_{i}$ } \\
    $d_{i} \leftarrow$ \MotionAdaptiveBuffer { $t_{i}$, $b_{i}$, $m_{i}$ } \\
    $C. $\AddDynamicObstacles { $d_{i}$ } \\
}
% $C. $\GenerateIntervals { } \\
$V^{'}_{C} \leftarrow $ \PriorityFunction { $V_{C}$ }\\
\ForEach { $v_{i}$ in $V^{'}_{C}$ } %, $p_{i}$ in $P_{E}$, $m_{i}$ in $M_{E}$, $b_{i}$ in $B_{E}$ }
{
    $w_{i} \leftarrow$ $C .$\SippPlanning { $p_{i}$, $g_{i}$ } \\
    % $W .$\Append{ $w_{i}$ } \\
    \SendOverNetwork { $v_{i}$ , $w_{i}$ } \\
    $d_{i} \leftarrow$ $C .$\MotionAdaptiveBuffer { $w_{i}$ } \\
    $C. $\AddDynamicObstacles { $d_{i}$ } \\
    % $d_{i} \leftarrow$ \MotionAdaptiveBuffer { $t_{i}$, $b_{i}$, $m_{i}$ } \\
    % $C. $\LoadDynamicObstacle { $d_{i}$ } \\
}
\end{algorithm}

\begin{algorithm}[t]
  \caption{Local Controller}
  \label{algo:planner}
\SetKwFunction{ReceiveTrajectory}{ReceiveTrajectory}
\SetKwFunction{ValidControlCycle}{ValidControlCycle}
\SetKwFunction{ValidTrajectory}{ValidTrajectory}
\SetKwFunction{RecoveryMode}{RecoveryMode}
\SetKwFunction{HasWaitCycle}{HasWaitCycle}
\SetKwFunction{GetWaitPoint}{GetWaitPoint}
\SetKwFunction{GetBrakingDistance}{GetBrakingDistance}
\SetKwFunction{ApplyBrake}{ApplyBrake}
\SetKwFunction{MoveToWaypoint}{MoveToWaypoint}
\SetKwFunction{SelectWaypoint}{SelectWaypoint}
\SetKwFunction{ApplyControl}{ApplyControl}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{Centralized planned trajectory $t$}
\Output{Low-level control signal $S$}
\BlankLine
$w \leftarrow$ \ReceiveTrajectory { } \\
\If  { $!$ \ValidControlCycle {$w$}  }
     {
        $w \leftarrow$ \RecoveryMode { } \\
     }
    
\eIf { \HasWaitCycle {$w$} }
     {
        $d_{s}, p_{s} \leftarrow$ \GetWaitPoint { $w$ } \\
        $d_{b} \leftarrow$ \GetBrakingDistance { $v$ } \\
        \eIf { $d_{b}$ $\leq$ $d_{s}$  }
        {
            $S \leftarrow$ \ApplyBrake { } \\
        }
        {
            $S \leftarrow$ \MoveToWaypoint { $p_{s}$ } \\
        }
     }
     {
        $p \leftarrow$ \SelectWaypoint { $w$ } \\
        $S \leftarrow$ \MoveToWaypoint { $p$ } \\
     }
\ApplyControl {$S$} \\
\end{algorithm}

\subsection{Centralized Planner}
The centralized planner, which resides at the edge, takes perception data and uses it to plan paths for all \sysname-compatible vehicles. It then sends these paths to all vehicles over the network. The planner generates paths for every vehicle at 10~Hz. The local low-level controllers on-board every vehicle convert these path to control signals (steer, throttle, and brake) that the vehicle can understand.

% \sysname uses the real-time scene understanding from the perception module to plan safe and efficient paths for \sysname-compatible vehicles. We call this component the \textit{centralized controller}. This component runs at the edge. 
%The edge runs trajectory planning for all \sysname-compatible vehicles on the road. 
% Self-driving vehicles today have a similar component today, however, this component is decentralized component so it plans a trajectory for a single vehicle. 

The perception module sends perception data about dynamic and static objects to the centralized controller. Dynamic objects include \sysname-compatible objects (vehicles with \sysname's low-level controller) and non-compatible objects (vehicles without \sysname's low-level controller, cyclists and pedestrians \etc). The centralized planner receives the position, bounding box, and motion vector (lines 1 and 2 of \algoref{algo:controller}) of every dynamic object from the perception module. Static objects include drivable area, the sidewalk, buildings, and traffic lights \etc For this, the planner receives a stitched 3D point cloud $S$ of the scene. It uses this to divide the scene into static obstacles and drivable space (line 3 of \algoref{algo:controller}).

\ramesh{does the term non-compatible also encompass cyclists and pedestrians?}
\fawad{Yes, addressed.}

The planner uses SIPP to plan every \sysname-compatible vehicle's motion. The planner converts the stitched point cloud $S$ into a 2D occupancy grid $S_{D}$ (with drivable and non-drivable blocks) and feeds it to SIPP (lines 3 and 4 of \algoref{algo:controller}). In a single agent scenario \ie only a single vehicle with no dynamic object, this occupancy grid would be enough for SIPP to plan a collision-free path. But in a realistic scenario, there are a number of dynamic obstacles which include both \sysname-compatible and non-compatible objects. \sysname needs to make SIPP aware of the locations of the objects at every instant in time in order to plan collision free paths. \sysname knows paths for all compatible objects because it plans paths for them. However, it has no way of knowing trajectories for non-compatible objects.

% an   The inputs to SIPP are: a) source and destination locations of the agent/car, and b) the set of obstacles in the environment. The set of obstacles consist of persistent static obstacles \eg the side-walk or a building and dynamic obstacles \eg traffic participants like other vehicles and pedestrains. Using these, SIPP plans the shortest non-collision path for the vehicle from source to destination.

To surmount this challenge, \sysname estimates the motion of all non-compatible vehicles\footnote{Like vehicles, we can estimate the motion of pedestrains as well. In this paper, we focus only on vehicles and the extension to pedestrains for future work.} and then feeds these estimates to SIPP (lines 5-9 of \algoref{algo:controller}). To do motion estimation for a non-compatible vehicle $v_{i}$, \sysname uses its motion vector $m_{i}$ and position estimate $p_{i}$ to forecast its trajectory $t_{i}$ over the next $X$ steps. To incorporate the vehicle's actual dimensions, \sysname uses the bounding boxes of every vehicle. However, this is not enough to relax the instant start/stop assumption of the SIPP algorithm or compensate for errors in perception/motion estimation.

To help alleviate the instant start/stop assumption and make the planner robust to perception errors, we form a motion adaptive buffer $d_{i}$ around the vehicle's trajectory $t_{i}$ (line 7 of \algoref{algo:controller}). The motion adaptive buffer wraps a dynamic bounding box around every position of the estimated trajectory $t_{i}$ for the vehicle $v_{i}$. The dynamic bounding box ensures safe driving distance between that vehicle and \sysname-compatible vehicles. This dynamic bounding box is a function of the vehicle bounding box $b_{i}$ and its motion vector $m_{i}$. At rest, the dynamic bounding box is the smallest and grows as the vehicle moves faster. Then, the planner feeds this to SIPP as a dynamic obstacle (line 8 of \algoref{algo:controller}). The planner uses the same technique for all non-compatible vehicles $V_{E}$ as well. 
% Finally, the controller combines the motion adaptive buffered trajectories of all vehicles and 

\ramesh{this notion of a motion adaptive box is interesting and could use a separate graphic as well as careful justification (perhaps it can be part of an ablation study)?}
\fawad{Please check now, I tried to justify it more and will add a figure too}

Next, the planner plans paths for all \sysname-compatible vehicles sequentially. The sequential order in which paths are planned allows for user-defined traffic policies. For instance, to prioritize an emergency vehicle at an intersection, SIPP will plan for it first and then use it as a dynamic obstacle for all other vehicles. So, the planner sorts \sysname-compatible vehicles $V^{'}_{C}$ based on a user-defined policy (line 10 of \algoref{algo:controller}). After this, the planner feeds the current position $p_{i}$ and goal $g_{i}$ of every compatible vehicle $v_{i}$ to SIPP. SIPP generates a set of collision-free way-points $w_{i}$ to take the vehicle from it position $p_{i}$ to its destination $g_{i}$ (line 13 of \algoref{algo:controller}). The planner sends these set of way points to the vehicle's on-board local low-level control module over the network (line 13 of \algoref{algo:controller}) using their cyber-physical association. Like a non-compatible vehicle, the planner forms a motion adaptive buffer around the current vehicle's trajectory and feeds it to SIPP as a dynamic obstacle for the next vehicle. At the end, the planner plans and sends paths to all compatible vehicles.

\ramesh{this notion of a policy being translated to the order in which your plan for vehicles is good. We might want to think a little bit about giving examples of practical policies, and how they can be translated into planning ordering. We don't have to go too deep into this, but we should be able to show the existence of 1 or 2 practical policies that can be implemented this way.}

% For every point in the estimated trajectory $t_{i}$, the motion adaptive filter wraps a bounding box around that   
% If SIPP assumptions about the world were true, controller could feed the trajectory $t_{i}$ of the vehicle $v_{i}$ to SIPP as dynamic obstacle. However, in the real-world, there can be errors in perception, or motion estimation and 

% For this, it extrapolates the vehi Given the present position estimate $p_{i}$, the motion estimation module extrapolates it using the magnitude and direction of the motion vector $m_{i}$ (line 6 of \algoref{algo:controller}). It uses the magnitude and direction of the the motion vector $m_{i}$ to determine position ov    estimates the motion of non-compatible vehicles and 
% Given an occupancy grid with static obstacles,  is a graph-search algorithm that finds the shortest path from source to destination in a given graph.  

% the centralized: a) stitched 3D  The centralized controller receives perception information about all the position, bounding box, and motion vector for every vehicle (both \sysname-compatible and non-compatible) along with a stitched point cloud from the perception module (\algoref{algo:controller}).  uses perception data (positions, bounding boxes, motion vectors and a drivable space map) from the perception module to generate trajectories for all \sysname-compatible vehicles. 
%% - Path planning
% \sysname uses the real-time scene understanding from the perception module to plan a safe and efficient path for vehicles to follow on the road. We call this component \textit{trajectory planning}. This component runs at the edge and it is a part of the planning module. The edge runs trajectory planning for all vehicles on the road. This creates opportunities for cross-car optimizations. Self-driving vehicles today have a similar component today, however, this component is decentralized component so it plans a trajectory for a single vehicle.

% \ramesh{For each component, say where it runs. Also, for path planning, say that the infrastructure has to do this for each car. This is an interesting point, because it permits cross-car optimizations unlike decentralized autonomous driving decisions made by each car.}
% \fawad{Addressed.}
%% - Delivery of low-level control signals
% \fawad{we might need a closed-loop component somewhere here}
\subsection{Local Planner}
Every \sysname-compatible vehicle has an on-board local low-level controller and PID controller that receives the set of planned way-points from the centralized planner over the network (\algoref{algo:planner}). The local controller translates these to low-level control signals (throttle, steer, and brake) that can be directly applied to each vehicle. The local controller runs every 2-3~ms in the vehicle. 

The local controller receives the planned trajectory $w$ from the centralized planner every 100~ms (line 1 of \algoref{algo:planner}). The planner may fail to plan a path for a vehicle or there might be a network failure. For robustness, the low-level controller checks if it has received the trajectory within a latency budget and if received path is valid (line 2 of \algoref{algo:planner}). If either of these are not true, it goes into recovery mode (line 3 of \algoref{algo:planner}). In recovery mode, the controller uses the last valid planned trajectory for the vehicle. The trajectory that the controller receives inform it of the vehicle's planned path for the next $X$ steps. It would have sufficed to send the vehicle its position for just the next 100~ms but this redundancy helps relax SIPP's instant start/stop assumption and introduces robustness.

\ramesh{The previous paragraph is important from a networking perspective. This idea is similar to soft state that permits robustness; see the Clark paper in the 551 readings.}

Given the planned trajectory $w$, the controller determines whether the vehicle has to wait at any point along it path (line 5 of \algoref{algo:planner}). We call this the wait cycle. If there is a wait cycle, it finds the position $p_{s}$ associated with the wait cycle and the distance of the vehicle from it $d_{s}$ (line 6 of \algoref{algo:planner}). Next, the controller calculates the braking distance $d_{b}$ (distance to bring the vehicle to a stop) of the vehicle using its current velocity $v$ (line 7 of \algoref{algo:planner}). If the braking distance is less than or equal to the distance from the stopping point (line 8 of \algoref{algo:planner}), the controller generates a signal $S$ to apply brakes (line 9 of \algoref{algo:planner}). Without this, vehicles would apply brakes at the spatial position of the wait cycle and hence overshoot it. With this maneuver, \sysname ensures that vehicles can adhere to SIPP's collision-free planned paths. On the other hand, if the vehicle is far away from the stopping point, then the controller generates a signal $S$ to continue moving the vehicle towards the stopping point (line 11 of \algoref{algo:planner}). We calculate braking distance using a standard equation~\cite{brakingdistance}.% and multiply it with a safety factor for robustness.

\ramesh{I couldn't find where wait cycle was previously defined.}
\fawad{Addressed.}

If there is no wait cycle in the entire trajectory $w$, the controller selects the next suitable way-point $p$ (line 14 of \algoref{algo:planner}) and generates a signal to move the vehicle towards that way-point (line 15 of \algoref{algo:planner}). Finally, the local controller applies the control signal $S$ to the vehicle (line 17 of \algoref{algo:planner}).

% As mentioned above, SIPP assumes that any vehicle can stop/start moving instantly. 
% After planning paths, \sysname sends them to all vehicles. %To do this, first, \sysname translates the path planned for each vehicle into low-level control (throttle and steering) signals. 
% To do this, first, \sysname associates the cyber presence of every vehicle in the perception module with its physical presence (network ID). This component lies at the edge inside the network module. Next, \sysname uses the network module to send the planned paths to all vehicles. %Current autonomous vehicle pipelines do  This component does not perform cyber-physical associations. %The first component (translation from path to signals) lies in the control module at the edge. 
% \sysname clients on the vehicles receive these trajectories. Besides this, the network module also transports data from sensors to the edge for perception. Self-driving vehicles pipelines today do not contain the network module. Then, these clients translate the planned trajectory into low-level control (throttle and steering) signals. The vehicle then uses these signals in closed feedback loop to drive the vehicle. This component lies in the control module at the vehicle. Current autonomous driving pipelines also contain a similar component.

% \fawad{Added a high-level planning layer that will reside at the cloud}
% Lastly, since the long time-scale path planning is relatively less latency-sensitive, it can be placed at the edge, the cloud or the car. This component draws safe and efficient paths for all vehicles from their origin to destinations.

\fi


==> planner_new.tex <==
\section{Planning}
\label{s:planner}
  
% \fawad{I think I'll add a diagram here to show how different sub-modules work in the controller.}
% \sysname's controller module uses positions, bounding boxes and motion vectors along with a drivable space map from the perception module to control \sysname-compatible vehicles. The control module consists of the three sub-modules \ie the centralized planner at the edge for motion-planning, and the local low-level controller along with a PID controller at the vehicle which convert those paths to low-level vehicle controls (\eg steering wheel angle, throttle, and brake).

\parab{Inputs, Outputs, and Goals.}
From perception, \sysname's planner receives bounding boxes for non-background objects, and their motion vectors. Some of these objects will be \sysname-capable vehicles; these follow trajectories designed by \sysname. For these, \sysname needs each vehicle's navigation goal, \eg where it is headed: we assume the planning component can get this by communicating with the vehicle. Other objects will be \sysname-oblivious: these include pedestrians, or vehicles driven by humans or on-board autonomous driving agents. The output of planning is a trajectory~---~a sequence of way-points, and times at which those way-points should be reached~---~for each \sysname-capable vehicle.

% \footnote{These are determined during cyber-physical association (\secref{s:part-extr}).}
% \footnote{To generate these trajectories, \sysname also needs a map of the drivable space (including road surface, lane markers and driving direction). These can either be obtained by scene analysis~\cite{background_filtering,lanedetection}, or from a one-time human annotation.}

Planning executes at every frame and must satisfy two goals: (a) it must fit within the tail latency budget of 100~ms, (b) and it must generate collision-free trajectories at every instant even in the presence of \sysname-oblivious objects.

% \parab{Goals and Requirements. } The controller must ensure collision-free driving for all \sysname-compatible vehicles with low latency in all deployment scenarios (\secref{sec:deployment}). The controller must support user-imposed traffic policies \eg prioritizing emergency vehicles, reducing traffic congestion \etc.

% \ramesh{the second sentence is good, but comes out of the blue. We might want to figure out whether we want to justify this requirement either here or earlier in the introduction or the arch section.}
\begin{figure}[t]
  \centering
  \begin{minipage}{0.25\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/planning_example_a.pdf}
    {\small (a)}
  \end{minipage}
  \begin{minipage}{0.25\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/planning_example_b.pdf}
    {\small (b)}
  \end{minipage}
  \begin{minipage}{0.25\linewidth}
    \centering
    \includegraphics[width=\columnwidth,frame]{figs/planning_example_c.pdf}
    {\small (c)}
  \end{minipage}
  \caption{(a) The first (red) planned vehicle can use the entire drivable space. (b) The second (blue) vehicle treats the first as an obstacle (different shades represent different times at which grids are occupied). (c) The motion-adaptive buffer around a vehicle is proportional to its speed.}
  \label{fig:planning_examples}
\end{figure}



% \parab{Prior Work in Planning.} Autonomous driving uses \textit{decentralized} motion planning algorithms that search for a path for the \textit{ego-vehicle} in graphs, based on variants of $A^{*}$~\cite{Astar} search. For example, Autoware uses a lattice-based discretization of the state space~\cite{mcnaughton11:_motion} for the search, while Baidu Apollo~\cite{BaiduSpecs} uses a modified $A^{*}$ search with heuristics to guide the search. In contrast, \sysname requires a \textit{centralized} motion planner (one that plans for all vehicles, not just the ego-vehicle), the best known of which is Conflict Based Search~\cite{CBS}, but this algorithm has high tail latency~\cite{cbslatency, SIPP}.

% \parae{SIPP.}
% \sysname adapts a fast, decentralized, planner for a single robot for environments with dynamic obstacles, SIPP~\cite{SIPP}. A dynamic obstacle is one whose position changes over time. SIPP discretizes space into a 2D occupancy grid (\figref{fig:planning_examples}(a)) and plans a path for a given robot from a one location (source) to another (destination). Planning in dynamic environments adds an extra dimension \ie time, to the search space which can increase computational complexity. SIPP's efficiency relies on the following intuition. Consider an arbitrary grid element (\eg a square on the road surface). The time steps ($t_{1}, t_{2}, ...., t_{n}$) that this element is \textit{safe} for robot occupancy (meaning no other robot occupies it at that time) is unbounded and infinitely large. However, the number of time \textit{intervals} ($[t_{1}, t_{n}]$) at which that location is safe is bounded and generally small. A (maximally) safe time interval ($[t_{1}, t_{n}]$) in one in which the location is safe for occupancy throughout the interval, but not safe one step before ($t_{0}$) and one step after ($t_{n+1}$) the interval.

% The input to SIPP is a goal for a robot and the positions over time of the dynamic obstacles in the environment. Using the latter, SIPP first generates a sequence, for each grid element, of safe and unsafe intervals. Then, using the former, SIPP uses $A^{*}$ search to find a provably collision-free shortest path for the robot~\cite{SIPP}.

\parab{\sysname's Planner.} The best-known centralized robot motion planner, Conflict Based Search~\cite{CBS} that jointly optimizes paths for multiple robots, has high tail latency~\cite{cbslatency, SIPP}. Instead, we use a fast \textit{single-robot} motion planner, SIPP~\cite{SIPP}. The input to SIPP is a goal for a robot and the positions over time of the dynamic obstacles in the environment. The output is a provably collision-free shortest path for the robot~\cite{SIPP}.

At each frame, \sysname must plan trajectories for every \sysname-capable vehicle. Without loss of generality, assume that vehicles are sorted in some order. \sysname's centralized planner iteratively plans trajectories for vehicles in that order:
\begin{quote}
\textit{When running SIPP on the $i$-th vehicle, \sysname represents all $i-1$ previously planned vehicles as dynamic obstacles in SIPP.}
\end{quote}
\figref{fig:planning_examples}(b) illustrates this, in which the trajectory of a previously planned (red) vehicle is represented as an obstacle when planning a trajectory for the blue vehicle.

This approach has two important properties:
%\begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=0ex,parsep=1ex,leftmargin=*]
\begin{enumerate}[nosep,wide]
\item All trajectories are collision-free. Two cars $i$ and $j$ cannot collide, since, if $j>i$, $j$'s trajectory would have used $i$'s as an obstacle, and SIPP generates a collision-free trajectory for each vehicle.
\item \sysname's planner cannot result in a traffic deadlock. A deadlock occurs when there exists a cycle of cars in which each car's forward progress on its currently planned trajectory is hampered by another. \figref{fig:deadlock} shows examples of deadlocked traffic with two, three, and four cars (these scenarios under which these deadlocks occurred are described in \secref{s:high-thro-traff}). However, \sysname cannot deadlock. If there exists a cycle, there must be at least one pair of cars $i, j$ where $i < j$ and $i$ blocks $j$. But this is not possible, because, when planning for $j$, \sysname represents $i$'s trajectory as an obstacle.
\end{enumerate}

% \begin{figure}[t]
%   \centering
%   \begin{minipage}{0.325\linewidth}
%     \centering
%     \includegraphics[width=\columnwidth,frame]{figs/deadlock_2_vehicles.png}
%     % {\small (a)}
%   \end{minipage}
%   \begin{minipage}{0.325\linewidth}
%     \centering
%     \includegraphics[width=\columnwidth,frame]{figs/deadlock_3_vehicles.png}
%     % {\small (b)}
%   \end{minipage}
%   \begin{minipage}{0.325\linewidth}
%     \centering
%     \includegraphics[width=\columnwidth,frame]{figs/deadlock_4_vehicles.png}
%     % {\small (c)}
%   \end{minipage}
%   \caption{With autonomous driving's de-centralized planning, in the absence of a traffic light controller, vehicles come to a deadlock at the intersection where they are unable to cross it..}
%   \label{fig:deadlock_example}
% \end{figure}



\begin{figure}[t]
  \centering
  \includegraphics[width=0.95\columnwidth]{figs/fig_deadlocks_combined_ver2.pdf}
  \caption{With autonomous driving's decentralized planning, in the absence of a traffic light controller, vehicles come to a deadlock at the intersection where they are unable to cross it.}
  \label{fig:deadlock}
\end{figure}


However, this approach may sacrifice optimality in transit times: vehicles later in the planning order may see longer transit times. On the flip side, it may allow \sysname to achieve novel traffic policies (\eg those that prioritize emergency vehicles). Future work can explore such traffic policies.

Because it was designed for robots, SIPP makes some idealized assumptions. \sysname adapts SIPP to relax these.

\parae{Robustness to \sysname-oblivious participants.}
SIPP plans the entire trajectory for a robot once, given all the dynamic obstacles in the environment. \sysname, to deal with \sysname-oblivious vehicles whose trajectories can change dynamically, re-plans trajectories for every \sysname-capable vehicle at every frame. This relaxes assumption in SIPP that all objects move at a fixed speed. For each \sysname-oblivious object, \sysname uses its bounding box, motion and heading vector. 

% \begin{figure*}
%   \centering
%   \begin{minipage}{0.19\linewidth}
%     \centering
%     \includegraphics[width=\columnwidth,frame]{figs/intersection_example_a.pdf}
%     {\small (a)}
%   \end{minipage}
%   \begin{minipage}{0.19\linewidth}
%     \centering
%     \includegraphics[width=\columnwidth,frame]{figs/intersection_example_b.pdf}
%     {\small (b)}
%   \end{minipage}
%   \begin{minipage}{0.19\linewidth}
%     \centering
%     \includegraphics[width=\columnwidth,frame]{figs/intersection_example_c.pdf}
%     {\small (c)}
%   \end{minipage}
%   \begin{minipage}{0.19\linewidth}
%     \centering
%     \includegraphics[width=\columnwidth,frame]{figs/intersection_example_d.pdf}
%     {\small (d)}
%   \end{minipage}
%   \begin{minipage}{0.19\linewidth}
%     \centering
%     \includegraphics[width=\columnwidth,frame]{figs/intersection_example_e.pdf}
%     {\small (e)}
%   \end{minipage}
%   \caption{(a) A bird's eye view of an intersection. LiDARs are mounted on the traffic light poles at each of the four corners of the intersection. (b) An individual frame from each of the 4 LiDARs. (c) A fused frame. (d) Point clouds of traffic participants at the intersection. (e) Bounding boxes and motion vectors for traffic participants, calculated over successive frames.}
%   \label{fig:intersection_example}
% \end{figure*}


\parae{Robustness to perception errors.}
SIPP assumes that each object has the same size, occupying one grid element. To relax this to permit different vehicle sizes (cars, trucks), \sysname uses the bounding boxes generated by perception to determine grid occupancy. The bounding boxes may be incorrect, so \sysname extends the bounding box by a small buffer on all sides. This extended buffer is \textit{motion-adaptive}: the faster the vehicle travels the larger is the buffer around it (\figref{fig:planning_examples}(c)).

\parae{Robustness to packet losses.}
The trajectory generated by \sysname is transmitted over a wireless network to the vehicle. To be robust to packet losses, \sysname generates waypoints over a longer horizon (10~s~\cite{shalevshwartz2018formal}) than the inter-frame time (100~ms in our case). This way,
it transmits trajectories every 100~ms, but if a transmission is lost, the vehicle can use the previously-received trajectory.\footnote{In a catastrophic failure, \sysname-capable vehicles must have a fallback-to-human strategy, as will autonomous driving.}

\parae{Robustness to vehicle kinematics limitations.}
SIPP assumes that a vehicle can start and stop instantaneously. In practice, a vehicle's kinematic characteristics dictate how quickly vehicles can start and stop. The longer planning horizon helps with the vehicle's controller time to adapt to vehicle kinematics. The controller (on-board the vehicle) can determine, from the received trajectory, if it has to stop at some future point in time; it can then decide when to apply the brakes, and with what intensity, to effect the stop.

% \parab{\sysname Extensions to On-board Control.} Every \sysname-compatible vehicle has an on-board local low-level controller and PID controller that receives the set of planned way-points from the centralized planner over the network. The local controller translates these to low-level control signals (throttle, steer, and brake) that can be directly applied to each vehicle. The local controller runs every 2-3~ms in the vehicle. 

% The local controller receives the planned trajectory (for that vehicle) from the centralized planner every 100~ms. If it does not receive a trajectory from the centralized planner within a latency budget (\eg due to network failure), it initiates a recovery mode, which uses the last valid trajectory received by the vehicle in a previous cycle. The local controller can afford to do this because the planner plans, and sends a trajectory for a longer time horizon (\secref{s:planner}). It would have sufficed to send the vehicle its trajecotry for just the next 100~ms but instead, \sysname sends a trajectory for the next $x$ seconds. This redundancy in the design not only addresses network failures but also helps relax SIPP's instant start/stop assumption and introduces robustness.

% % \ramesh{The previous paragraph is important from a networking perspective. This idea is similar to soft state that permits robustness; see the Clark paper in the 551 readings.}

% Given the planned trajectory for the next $x$ seconds, the local controller determines whether the vehicle has to wait at any point along its planned trajectory. We call this a wait cycle. If there is a wait cycle, it finds the position associated with the wait cycle and the distance of the vehicle from it. The controller then calculates the braking distance (distance to bring the vehicle to a complete stop) of the vehicle using its motion vector. If the braking distance is less than or equal to the distance from the stopping point, the controller generates a signal to apply brake. Without this, vehicles would apply brakes at the spatial position of the wait cycle and hence overshoot it. With this maneuver, \sysname ensures that vehicles can adhere to SIPP's collision-free planned paths. On the other hand, if the vehicle is far away from the stopping point, then the controller generates a signal to continue moving the vehicle towards the stopping point. We calculate braking distance using a standard equation~\cite{brakingdistance}.% and multiply it with a safety factor for robustness.

% % \ramesh{I couldn't find where wait cycle was previously defined.}
% % \fawad{Addressed.}

% If there is no wait cycle in the entire trajectory, the controller selects the next suitable way-point and generates a signal to move the vehicle towards that way-point. Finally, the local controller applies the control signal to the vehicle.

% \secref{s:centralized-planner} describes the planner in detail, and \secref{s:local-controller} describes extensions to the on-board controller to enable \sysname to respect the vehicle's kinematic constraints.

% use on-board planning and control modules to plan motion and follow collision-free paths to reach their destinations. Since every vehicle plans for itself, work in industry and academia has focused on decentralized motion planning algorithms ($A^{*}$~\cite{Astar}, Safe Interval Path Planning (SIPP)~\cite{SIPP}, and Dijkstra~\cite{Dijkstra}). Centralized algorithms (\eg Conflict Based Search (CBS)~\cite{CBS}) for multi-robot/agent planning exist but, in practice, they have been used in more controlled environments like warehouses and are known to have large tail latencies~\cite{cbslatency, SIPP}. To this end, \sysname uses a decentralized low-latency algorithm, SIPP, in a centralized manner for motion planning.

% \ramesh{we might want to add a citation for the tail latencies.}
% \fawad{Addressed.}

\iffalse

% \textit{Challenges. }
\parab{SIPP. }
Planning in static environments is a well-studied problem that can be solved efficiently. Planning algorithms discretize space into a 2D occupancy grid and plan a path for a given robot from a one location (source) to another (destination). Planning in dynamic environments adds an extra dimension \ie time, to the search space and this increases computational complexity. SIPP is a graph-search algorithm for dynamic environments that is based on the following intuition. Although the \textit{time steps} ($t_{1}, t_{2}, ...., t_{n}$) that a given location in the occupancy grid is safe for robot occupation is unbounded and infinitely large; the number of \textit{time intervals} ($[t_{1}, t_{n}]$) at which that location is safe is bounded and generally small. A safe \textit{time interval} ($[t_{1}, t_{n}]$) in one in which the location is safe for occupation throughout the interval, but not safe one step before ($t_{0}$) and one step after ($t_{n+1}$) the interval. To scale, for every location in the 2D occupancy grid, SIPP discretizes time into contiguous safe and unsafe \textit{time intervals} or states. Squares with static obstacles \eg the sidewalk are unsafe eternally whereas others like the road have multiple safe and unsafe states. This allows SIPP to compactly represent each location with a few states. With this representation, SIPP solves the graph-search problem using $A^{*}$ search.

\ramesh{the above description is good, but you might want to add more academic language: to scale, SIPP discretizes space and time etc. Give the intuition behind what enables it to scale, and then describe how the algorithm works.}
\fawad{Addressed.}

\parab{Centralized Planning with SIPP. }
\sysname uses SIPP in a greedy, sequential manner for centralized control. Consider the full-deployment scenario (\secref{sec:deployment}). In this, \sysname first plans for a single vehicle with SIPP using only the static environment. Then, it uses the SIPP-generated path for first vehicle as a dynamic obstacle for the second vehicle. This way, the second vehicle can avoid static obstacles and the first vehicle. The third vehicle uses both the first and second vehicles as dynamic obstacles and so on. This way, \sysname can plan for all vehicles in a centralized manner using sequential SIPP.

\sysname uses a greedy approach for planning as opposed to an optimal approach like CBS for two reasons: a) latency, and b) flexibility. Optimal approaches tradeoff planning time (latency) to ensure robots reach their destinations in the minimum amount of time. In our case, a lower planning time (to meet the 100~ms latency budget), guaranteed by a greedy approach, is more important. Second, an optimal approach achieves a single goal \ie minimum overall trip time. With a greedy approach, \sysname creates opportunities support different types of user-defined traffic policies. For instance, besides minimizing trip times, it can prioritize emergency vehicles, ensure fair waiting times for all vehicles, ameliorate traffic congestion on a given road \etc.
% \sysname uses a greedy approach as opposed to a more optimal approach like CBS for the following reasons. Optimal approaches tradeoff have higher planning times to ensure all robots reach their destinations in the minimum amount of time. In our  case of autonomous driving, a lower planning time (to meet the 100~ms latency budget) is more important than time to plan is more important    is more important than First, although, the greedy approach does not guarantee an optimal solution, it  the greedy approach ensures that we reach a solution faster. Optimal  Instead of a greedy approach, we could have used an We could have used a more optimal approach for planning (\eg Conflict Based Search) We use a greedy approach in \sysname (as opposed to an optimal approach like CBS)  
% 1. For latency
    % CBS run times are higher so we can only use it once. It will have to be updated and run every step which makes it very expensive
    % Even if the environment changes, we can run SIPP over and over again because it has a lower cost
% 2. For user defined traffic policies
%   
% As opposed to a greedy approach, \sysname could have used an optimal algorithm like Conflict Based Search. 

% A centralized controller, as opposed to decentralized controllers today, creates opportunities for cross-car optimizations and impose user-defined traffic policies (as we show later).

\ramesh{similar comment here. First say that we run SIPP in a greedy manner, planning for each vehicle in turn, while treating previously planned vehicles as obstacles. When you say this, people will expect a discussion of why you chose greedy: fast versus non-optimal.}
\fawad{Addressed but still thinking about how to improve it}

\parab{Challenges. }
SIPP solves a graph-search problem to plan a path for a vehicle from source to destination without any regard to real-world vehicle physics and traffic regulations. In doing so, it makes assumptions that do not hold true in the real-world. For instance it assumes that: a) vehicles can stop/start moving instantly, b) vehicles move with uniform speed, c) vehicles can move in all directions, d) vehicles occupy a single square on the occupancy grid, and e) the controller knows the location of every dynamic obstacle on the occupancy grid. To use SIPP in a realistic scenario, \sysname must relax these assumptions. 

Secondly, though SIPP is faster than other centralized algorithms, it takes upto 1~second to complete a single planning cycle. Moreover, this time increases with the number of vehicles that it must plan for. \sysname must enable SIPP to scale to a large number of vehicles and reduce the time for a single planning cycle.

\parab{\sysname's Approach. }
% Three contributions
% Splitting functionality / parallelism
To add support for real-world dynamics, \sysname must balance two competing constraints. \sysname's controller needs additional functionality to understands real-world dynamics. However, this functionality increases computational complexity and increases latency. To achieve both goals, \sysname divides the control module into two sub-modules and distributes the additional functionality between them. This includes a centralized planner resides at the edge and a low-level controller on-board every vehicle. The centralized planner runs the SIPP planning for all vehicles. It then sends a set of waypoints to the on-board low-level control module which converts them to the steer angle, throttle and brake. 

% Real-world dynamics
An out-of-the-box SIPP algorithm only uses robot positions as inputs for planning. To add support for real-world scenarios, \sysname's centralized planner makes use of the motion vectors and bounding boxes of vehicles from the perception component. The centralized planner uses motion vectors to model motion and the bounding boxes to model the realistic size of every vehicle in SIPP. Similarly, the low-level control module, converts the output (designed for a robot that can start/stop instantly) from the planner to a realistic path that vehicle can follow. To do this, it uses the set of waypoints and vehicle dynamics (\eg braking force and acceleration).

% Latency requirement
Lastly, \sysname makes optimizations to SIPP that enable it to run a planning cycle within 10~ms for low-latency planning. This way \sysname can run the centralized planner at LiDAR frame rate. As we discuss later, this makes \sysname more robust to unexpected changes in the environment (\eg unexpected driver, pedestrian or cyclist behavior).

% these waypoints to  Then, it sends    Then, it adds functionality to \sysname adds functionality to the controller that enable it to understand real-world dynamics. It splits this into two sub-modules: a) a centralized planner, and b) a local low-level control module. 

% First, \sysname uses SIPP planning at LiDAR frame rate instead of single-shot planning. Second, \sysname adds functionality to the controller that enable it to understand real-world dynamics of vehicles and road regulations. It splits this functionality between the edge (centralized controller) and the vehicle (local planner).

\ramesh{The LIDAR and single shot planning comes out of the blue; there is nothing in the prior text that prepares the reader for this. At this point, the reader is expecting some description of how you relax the assumptions. Also, it is unclear what problem functionality splitting solves.}
\fawad{I changed the entire approach because I missed out on many points. Please check it now}
% in SIPP to help it understand the real-world dynamics of a vehicle \eg its size and momentum. Last, \sysnam 
% whereas dynamic object   
% are used, \sysname controls multiple     a planning module along with a control module to control the motion of the vehicle. The planning module performs two functions: a) it plans a collision-free path for a vehicle from source to destination (path-planning) and b) it plans the motion of the vehicle to follow that path (motion-planning). The control module converts that motion to low-level control signals that the vehicle can understand. 

\begin{algorithm}[t]
  \caption{Centralized Planner}
  \label{algo:controller}
\SetKwFunction{CalculateDrivableSpace}{CalculateDrivableSpace}
\SetKwFunction{QueryPerception}{QueryPerception}
\SetKwFunction{MotionEstimation}{MotionEstimation}
\SetKwFunction{MotionAdaptiveBuffer}{MotionAdaptiveBuffer}
\SetKwFunction{AddDynamicObstacles}{AddDynamicObstacles}
\SetKwFunction{SippPlanning}{SippPlanning}
\SetKwFunction{RecoveryMode}{RecoveryMode}
\SetKwFunction{AddStaticObstacles}{AddStaticObstacles}
\SetKwFunction{GenerateIntervals}{GenerateIntervals}
\SetKwFunction{PriorityFunction}{PriorityFunction}
\SetKwFunction{Append}{Append}
\SetKwFunction{SendOverNetwork}{SendOverNetwork}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{\sysname-compatible objects $V_{C}$ \\ Non-compatible objects $V_{E}$ \\ Stitched point cloud $S$}
% ${Vehicle poses $P$, bounding boxes $B$, motion vectors $M$ and stitched point cloud $S$} % P for the set of point clouds and G for the set of gps tags
\Output{Vehicle trajectories $W$ for $V_{C}$}
\BlankLine
$P_{C}, M_{C}, B_{C} \leftarrow $ \QueryPerception ( $V_{C}$ ) \\ % Query perception for ego-vehicles
$P_{E}, M_{E}, B_{E} \leftarrow $ \QueryPerception ( $V_{E}$ ) \\ % Query perception for non-ego vehicles
$S_{D} \leftarrow $ \CalculateDrivableSpace {$S$} \\
$C. $ \AddStaticObstacles { $S_{D}$ } \\
% \ForEach { $v_{i}$ in $V_{E}$, $p_{i}$ in $P_{E}$, $m_{i}$ in $M_{E}$, $b_{i}$ in $B_{E}$ }
\ForEach { $v_{i}$ in $V_{E}$ } %, $p_{i}$ in $P_{E}$, $m_{i}$ in $M_{E}$, $b_{i}$ in $B_{E}$ }
{
    $t_{i} \leftarrow$ \MotionEstimation { $p_{i}$, $m_{i}$ } \\
    $d_{i} \leftarrow$ \MotionAdaptiveBuffer { $t_{i}$, $b_{i}$, $m_{i}$ } \\
    $C. $\AddDynamicObstacles { $d_{i}$ } \\
}
% $C. $\GenerateIntervals { } \\
$V^{'}_{C} \leftarrow $ \PriorityFunction { $V_{C}$ }\\
\ForEach { $v_{i}$ in $V^{'}_{C}$ } %, $p_{i}$ in $P_{E}$, $m_{i}$ in $M_{E}$, $b_{i}$ in $B_{E}$ }
{
    $w_{i} \leftarrow$ $C .$\SippPlanning { $p_{i}$, $g_{i}$ } \\
    % $W .$\Append{ $w_{i}$ } \\
    \SendOverNetwork { $v_{i}$ , $w_{i}$ } \\
    $d_{i} \leftarrow$ $C .$\MotionAdaptiveBuffer { $w_{i}$ } \\
    $C. $\AddDynamicObstacles { $d_{i}$ } \\
    % $d_{i} \leftarrow$ \MotionAdaptiveBuffer { $t_{i}$, $b_{i}$, $m_{i}$ } \\
    % $C. $\LoadDynamicObstacle { $d_{i}$ } \\
}
\end{algorithm}

\begin{algorithm}[t]
  \caption{Local Controller}
  \label{algo:planner}
\SetKwFunction{ReceiveTrajectory}{ReceiveTrajectory}
\SetKwFunction{ValidControlCycle}{ValidControlCycle}
\SetKwFunction{ValidTrajectory}{ValidTrajectory}
\SetKwFunction{RecoveryMode}{RecoveryMode}
\SetKwFunction{HasWaitCycle}{HasWaitCycle}
\SetKwFunction{GetWaitPoint}{GetWaitPoint}
\SetKwFunction{GetBrakingDistance}{GetBrakingDistance}
\SetKwFunction{ApplyBrake}{ApplyBrake}
\SetKwFunction{MoveToWaypoint}{MoveToWaypoint}
\SetKwFunction{SelectWaypoint}{SelectWaypoint}
\SetKwFunction{ApplyControl}{ApplyControl}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{Centralized planned trajectory $t$}
\Output{Low-level control signal $S$}
\BlankLine
$w \leftarrow$ \ReceiveTrajectory { } \\
\If  { $!$ \ValidControlCycle {$w$}  }
     {
        $w \leftarrow$ \RecoveryMode { } \\
     }
    
\eIf { \HasWaitCycle {$w$} }
     {
        $d_{s}, p_{s} \leftarrow$ \GetWaitPoint { $w$ } \\
        $d_{b} \leftarrow$ \GetBrakingDistance { $v$ } \\
        \eIf { $d_{b}$ $\leq$ $d_{s}$  }
        {
            $S \leftarrow$ \ApplyBrake { } \\
        }
        {
            $S \leftarrow$ \MoveToWaypoint { $p_{s}$ } \\
        }
     }
     {
        $p \leftarrow$ \SelectWaypoint { $w$ } \\
        $S \leftarrow$ \MoveToWaypoint { $p$ } \\
     }
\ApplyControl {$S$} \\
\end{algorithm}

\subsection{Centralized Planner}
The centralized planner, which resides at the edge, takes perception data and uses it to plan paths for all \sysname-compatible vehicles. It then sends these paths to all vehicles over the network. The planner generates paths for every vehicle at 10~Hz. The local low-level controllers on-board every vehicle convert these path to control signals (steer, throttle, and brake) that the vehicle can understand.

% \sysname uses the real-time scene understanding from the perception module to plan safe and efficient paths for \sysname-compatible vehicles. We call this component the \textit{centralized controller}. This component runs at the edge. 
%The edge runs trajectory planning for all \sysname-compatible vehicles on the road. 
% Self-driving vehicles today have a similar component today, however, this component is decentralized component so it plans a trajectory for a single vehicle. 

The perception module sends perception data about dynamic and static objects to the centralized controller. Dynamic objects include \sysname-compatible objects (vehicles with \sysname's low-level controller) and non-compatible objects (vehicles without \sysname's low-level controller, cyclists and pedestrians \etc). The centralized planner receives the position, bounding box, and motion vector (lines 1 and 2 of \algoref{algo:controller}) of every dynamic object from the perception module. Static objects include drivable area, the sidewalk, buildings, and traffic lights \etc For this, the planner receives a stitched 3D point cloud $S$ of the scene. It uses this to divide the scene into static obstacles and drivable space (line 3 of \algoref{algo:controller}).

\ramesh{does the term non-compatible also encompass cyclists and pedestrians?}
\fawad{Yes, addressed.}

The planner uses SIPP to plan every \sysname-compatible vehicle's motion. The planner converts the stitched point cloud $S$ into a 2D occupancy grid $S_{D}$ (with drivable and non-drivable blocks) and feeds it to SIPP (lines 3 and 4 of \algoref{algo:controller}). In a single agent scenario \ie only a single vehicle with no dynamic object, this occupancy grid would be enough for SIPP to plan a collision-free path. But in a realistic scenario, there are a number of dynamic obstacles which include both \sysname-compatible and non-compatible objects. \sysname needs to make SIPP aware of the locations of the objects at every instant in time in order to plan collision free paths. \sysname knows paths for all compatible objects because it plans paths for them. However, it has no way of knowing trajectories for non-compatible objects.

% an   The inputs to SIPP are: a) source and destination locations of the agent/car, and b) the set of obstacles in the environment. The set of obstacles consist of persistent static obstacles \eg the side-walk or a building and dynamic obstacles \eg traffic participants like other vehicles and pedestrains. Using these, SIPP plans the shortest non-collision path for the vehicle from source to destination.

To surmount this challenge, \sysname estimates the motion of all non-compatible vehicles\footnote{Like vehicles, we can estimate the motion of pedestrains as well. In this paper, we focus only on vehicles and the extension to pedestrains for future work.} and then feeds these estimates to SIPP (lines 5-9 of \algoref{algo:controller}). To do motion estimation for a non-compatible vehicle $v_{i}$, \sysname uses its motion vector $m_{i}$ and position estimate $p_{i}$ to forecast its trajectory $t_{i}$ over the next $X$ steps. To incorporate the vehicle's actual dimensions, \sysname uses the bounding boxes of every vehicle. However, this is not enough to relax the instant start/stop assumption of the SIPP algorithm or compensate for errors in perception/motion estimation.

To help alleviate the instant start/stop assumption and make the planner robust to perception errors, we form a motion adaptive buffer $d_{i}$ around the vehicle's trajectory $t_{i}$ (line 7 of \algoref{algo:controller}). The motion adaptive buffer wraps a dynamic bounding box around every position of the estimated trajectory $t_{i}$ for the vehicle $v_{i}$. The dynamic bounding box ensures safe driving distance between that vehicle and \sysname-compatible vehicles. This dynamic bounding box is a function of the vehicle bounding box $b_{i}$ and its motion vector $m_{i}$. At rest, the dynamic bounding box is the smallest and grows as the vehicle moves faster. Then, the planner feeds this to SIPP as a dynamic obstacle (line 8 of \algoref{algo:controller}). The planner uses the same technique for all non-compatible vehicles $V_{E}$ as well. 
% Finally, the controller combines the motion adaptive buffered trajectories of all vehicles and 

\ramesh{this notion of a motion adaptive box is interesting and could use a separate graphic as well as careful justification (perhaps it can be part of an ablation study)?}
\fawad{Please check now, I tried to justify it more and will add a figure too}

Next, the planner plans paths for all \sysname-compatible vehicles sequentially. The sequential order in which paths are planned allows for user-defined traffic policies. For instance, to prioritize an emergency vehicle at an intersection, SIPP will plan for it first and then use it as a dynamic obstacle for all other vehicles. So, the planner sorts \sysname-compatible vehicles $V^{'}_{C}$ based on a user-defined policy (line 10 of \algoref{algo:controller}). After this, the planner feeds the current position $p_{i}$ and goal $g_{i}$ of every compatible vehicle $v_{i}$ to SIPP. SIPP generates a set of collision-free way-points $w_{i}$ to take the vehicle from it position $p_{i}$ to its destination $g_{i}$ (line 13 of \algoref{algo:controller}). The planner sends these set of way points to the vehicle's on-board local low-level control module over the network (line 13 of \algoref{algo:controller}) using their cyber-physical association. Like a non-compatible vehicle, the planner forms a motion adaptive buffer around the current vehicle's trajectory and feeds it to SIPP as a dynamic obstacle for the next vehicle. At the end, the planner plans and sends paths to all compatible vehicles.

\ramesh{this notion of a policy being translated to the order in which your plan for vehicles is good. We might want to think a little bit about giving examples of practical policies, and how they can be translated into planning ordering. We don't have to go too deep into this, but we should be able to show the existence of 1 or 2 practical policies that can be implemented this way.}

% For every point in the estimated trajectory $t_{i}$, the motion adaptive filter wraps a bounding box around that   
% If SIPP assumptions about the world were true, controller could feed the trajectory $t_{i}$ of the vehicle $v_{i}$ to SIPP as dynamic obstacle. However, in the real-world, there can be errors in perception, or motion estimation and 

% For this, it extrapolates the vehi Given the present position estimate $p_{i}$, the motion estimation module extrapolates it using the magnitude and direction of the motion vector $m_{i}$ (line 6 of \algoref{algo:controller}). It uses the magnitude and direction of the the motion vector $m_{i}$ to determine position ov    estimates the motion of non-compatible vehicles and 
% Given an occupancy grid with static obstacles,  is a graph-search algorithm that finds the shortest path from source to destination in a given graph.  

% the centralized: a) stitched 3D  The centralized controller receives perception information about all the position, bounding box, and motion vector for every vehicle (both \sysname-compatible and non-compatible) along with a stitched point cloud from the perception module (\algoref{algo:controller}).  uses perception data (positions, bounding boxes, motion vectors and a drivable space map) from the perception module to generate trajectories for all \sysname-compatible vehicles. 
%% - Path planning
% \sysname uses the real-time scene understanding from the perception module to plan a safe and efficient path for vehicles to follow on the road. We call this component \textit{trajectory planning}. This component runs at the edge and it is a part of the planning module. The edge runs trajectory planning for all vehicles on the road. This creates opportunities for cross-car optimizations. Self-driving vehicles today have a similar component today, however, this component is decentralized component so it plans a trajectory for a single vehicle.

% \ramesh{For each component, say where it runs. Also, for path planning, say that the infrastructure has to do this for each car. This is an interesting point, because it permits cross-car optimizations unlike decentralized autonomous driving decisions made by each car.}
% \fawad{Addressed.}
%% - Delivery of low-level control signals
% \fawad{we might need a closed-loop component somewhere here}
\subsection{Local Planner}
Every \sysname-compatible vehicle has an on-board local low-level controller and PID controller that receives the set of planned way-points from the centralized planner over the network (\algoref{algo:planner}). The local controller translates these to low-level control signals (throttle, steer, and brake) that can be directly applied to each vehicle. The local controller runs every 2-3~ms in the vehicle. 

The local controller receives the planned trajectory $w$ from the centralized planner every 100~ms (line 1 of \algoref{algo:planner}). The planner may fail to plan a path for a vehicle or there might be a network failure. For robustness, the low-level controller checks if it has received the trajectory within a latency budget and if received path is valid (line 2 of \algoref{algo:planner}). If either of these are not true, it goes into recovery mode (line 3 of \algoref{algo:planner}). In recovery mode, the controller uses the last valid planned trajectory for the vehicle. The trajectory that the controller receives inform it of the vehicle's planned path for the next $X$ steps. It would have sufficed to send the vehicle its position for just the next 100~ms but this redundancy helps relax SIPP's instant start/stop assumption and introduces robustness.

\ramesh{The previous paragraph is important from a networking perspective. This idea is similar to soft state that permits robustness; see the Clark paper in the 551 readings.}

Given the planned trajectory $w$, the controller determines whether the vehicle has to wait at any point along it path (line 5 of \algoref{algo:planner}). We call this the wait cycle. If there is a wait cycle, it finds the position $p_{s}$ associated with the wait cycle and the distance of the vehicle from it $d_{s}$ (line 6 of \algoref{algo:planner}). Next, the controller calculates the braking distance $d_{b}$ (distance to bring the vehicle to a stop) of the vehicle using its current velocity $v$ (line 7 of \algoref{algo:planner}). If the braking distance is less than or equal to the distance from the stopping point (line 8 of \algoref{algo:planner}), the controller generates a signal $S$ to apply brakes (line 9 of \algoref{algo:planner}). Without this, vehicles would apply brakes at the spatial position of the wait cycle and hence overshoot it. With this maneuver, \sysname ensures that vehicles can adhere to SIPP's collision-free planned paths. On the other hand, if the vehicle is far away from the stopping point, then the controller generates a signal $S$ to continue moving the vehicle towards the stopping point (line 11 of \algoref{algo:planner}). We calculate braking distance using a standard equation~\cite{brakingdistance}.% and multiply it with a safety factor for robustness.

\ramesh{I couldn't find where wait cycle was previously defined.}
\fawad{Addressed.}

If there is no wait cycle in the entire trajectory $w$, the controller selects the next suitable way-point $p$ (line 14 of \algoref{algo:planner}) and generates a signal to move the vehicle towards that way-point (line 15 of \algoref{algo:planner}). Finally, the local controller applies the control signal $S$ to the vehicle (line 17 of \algoref{algo:planner}).

% As mentioned above, SIPP assumes that any vehicle can stop/start moving instantly. 
% After planning paths, \sysname sends them to all vehicles. %To do this, first, \sysname translates the path planned for each vehicle into low-level control (throttle and steering) signals. 
% To do this, first, \sysname associates the cyber presence of every vehicle in the perception module with its physical presence (network ID). This component lies at the edge inside the network module. Next, \sysname uses the network module to send the planned paths to all vehicles. %Current autonomous vehicle pipelines do  This component does not perform cyber-physical associations. %The first component (translation from path to signals) lies in the control module at the edge. 
% \sysname clients on the vehicles receive these trajectories. Besides this, the network module also transports data from sensors to the edge for perception. Self-driving vehicles pipelines today do not contain the network module. Then, these clients translate the planned trajectory into low-level control (throttle and steering) signals. The vehicle then uses these signals in closed feedback loop to drive the vehicle. This component lies in the control module at the vehicle. Current autonomous driving pipelines also contain a similar component.

% \fawad{Added a high-level planning layer that will reside at the cloud}
% Lastly, since the long time-scale path planning is relatively less latency-sensitive, it can be placed at the edge, the cloud or the car. This component draws safe and efficient paths for all vehicles from their origin to destinations.

\fi


==> proposed_arch.tex <==
\section{The \sysname Architecture}
\label{sec:architecture}

%\ramesh{Note to self: Not just LiDARs but stereo cameras as well.}
%\ramesh{Note to self: Discuss fallback somewhere.}

Before describing the system architecture, we briefly describe how autonomous vehicles work today.

%% This can go into the intro?

\subsection{Autonomous Vehicles Today}
\label{sec:background}

Autonomous vehicles consist of three logical components~\cite{paden2016survey,pendleton2017perception}: perception, planning, and control (\figref{fig:netd_arch}(a)).

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.9\columnwidth]{figs/fig_autonomous_driving_stack.pdf}
%   \caption{Self-driving stack}
%   \label{fig:av_stack}
% \end{figure}

\parab{Perception.} To perceive and extract knowledge about the world, an autonomous vehicle uses one or more 3D sensors capable of depth perception (\eg radars, stereo cameras, and LiDARs). A LiDAR, for example, sends millions of light pulses 10 or more times a second in all directions, whose reflections enable the LiDAR to estimate the position of points on objects or surfaces in the environment. The output of a LiDAR is a 3D \textit{point cloud} that contains points with associated 3D positions. Stereo cameras also output point clouds, but estimate depth using the positions of pixels in the left and right images of their two cameras. In this paper, we focus on LiDAR-based perception, leaving it to future work to explore other sensing modalities.

An autonomous vehicle's \textit{perception module} extracts an abstract scene description, consisting of static and dynamic objects, from these point clouds. Static objects include road surfaces, lane markers~\cite{lanedetection}, and safe drivable space~\cite{drivablespace}. The module also identifies dynamic objects (other vehicles, pedestrians, bicyclists) and tracks them. Finally, it estimates the vehicle's own position, using SLAM (Simultaneous Localization and Mapping)~\cite{slam_part1,slam_part2} algorithms. 

% understand the scene around it, detect drivable space, and localize itself (\figref{fig:av_stack}). First, the module segments the scene it sees through its sensors into static and dynamic objects. For this, it can use semantic segmentation tools~\cite{DeepLab}, background subtraction~\cite{Octree}, and ground-plane extraction~\cite{groundplane} \etc. Then, it extracts the road surface, detects lane markers~\cite{lanedetection} and safe drivable space~\cite{drivablespace}. To localize the vehicle, the perception module matches \textit{features} in its point cloud with those in SLAM (Simultaneous Localization and Mapping)~\cite{slam_part1,slam_part2} generated \textit{3D maps}~\cite{CarMap}. The map contains the positions of the matched features, using which the vehicle can triangulate its own position.

% and are constructed from LiDARs or 
% cameras (multi-view stereo~\cite{colmap}).

% These maps are dense reconstructions of the physical world 
% around the vehicle and enable it to see beyond it's sensors' range.
% SLAM uses cameras~\cite{ORB-SLAM2} or LiDARs~\cite{LOAM} along 
% with other sensors (GPS) to precisely localize a vehicle by 
% tracking static features in its surroundings.   
% \ramesh{Do they use SLAM, or SLAM-generated maps? Also, consider whether this detail is important from the perspective of the story. Do we use SLAM anywhere else? If we only plan to make a passing reference, may introduce it there.}
% \fawad{I think it might be important because we will have a localization experiment later on and then we need to compare our approach with what autonomous vehicles have now.}

% 2.2 Control
\parab{Planning.} The planning module uses abstract scene description from the perception component to plan and execute a safe path for the vehicle, while satisfying performance and comfort objectives~\cite{paden2016survey} (\eg smooth driving, minimal travel time \etc). Planning consists of three sub-tasks, distinguished by the time-scales at which they operate.

% Route planning module
\textit{Route planning}, usually executed once per trip, determines a safe \textit{path} (represented as a sequence of way-points through the road network) for the vehicle from the origin to the destination. \textit{Behavior planning}, which operates at time-scales of a few seconds, uses the path way-points and information about other objects and traffic participants (pedestrians, vehicles) to determine a set of driving maneuvers (\eg intersection navigation, lane-following, right turn at stop sign, parking \etc) for the vehicle to use at each part of the planned path. \textit{Motion planning} converts behaviors into short-term \textit{trajectories} (at the timescale of 100s of milliseconds) that the vehicle must follow. A trajectory is a sequence of way-points, together with the precise times at which the vehicle must arrive at those way-points.

\parab{Control.} This component takes a trajectory and converts it, at millisecond timescales, to low-level actuator (\eg throttle, steering, brake) signals.

\parab{Performance Considerations.} Beyond the functional decomposition described above, today's self driving software and hardware must satisfy several requirements~\cite{lin18:_archit_implic_auton_drivin}. Two of these are important: frame rate processing, and an end-to-end tail latency of less than 100~ms~\cite{lin18:_archit_implic_auton_drivin}. With a LiDAR sensor that generates frames at 10 frames per second, these requirements mean that the autonomous driving stack must have a throughput of at least 10 frames a second, and must produce an updated trajectory derived from a frame no later than 100~ms after the frame was generated (this number is derived based on human perception limits~\cite{lin18:_archit_implic_auton_drivin}). Autonomous vehicles must also satisfy other power and cooling requirements~\cite{lin18:_archit_implic_auton_drivin} which are beyond the scope of this paper\footnote{We note, however, that \sysname can significantly reduce power and cooling requirements by offloading perception and planning to infrastructure.}.

\subsection{An Architectural Shift: \sysname}
\label{s:de-coupl-perc}

% that uses actuator signals to ensure the vehicle follows the planned 
% trajectory and minimizes errors in doing so. The vehicle runs the 
% control module as fast as possible (every millisecond).

%  \ramesh{In the previous para, do we want to mention the timescales at which these decisions happen? This will be crucial in deciding what we can offload, and what we cannot. Also, in the writing above, you can make it clear what are the inputs/outputs of each stage.}
%  \fawad{Addressed.}
%  \ramesh{Your writing has fewer passive voice sentences than it used to, which is good. There are a couple in the para above: behaviors are represented, are caused etc.}
% \fawad{Addressed.}

%  \ramesh{Do we need the rest of this text? Doesn't seem relevant for our paper. Might be important to discuss briefly in related work, though.}

% Move to related work section
% \parab{Connected \& Automated Vehicles.}
% Introducing connectivity and coordination between autonomous vehicles 
% and the infrastructure can reduce sources of uncertainty, enabling 
% safer, and energy-efficient driving. An example of a proposed 
% control and planning architecture for such a 
% system~\cite{guanetti2018control} decouples real-time safety-critical 
% control tasks at the vehicle from 
% remote routing and planning at the cloud. The real-time control 
% module consists of powertrain control, motion control, and 
% motion planning. The remote planning mostly provides routing 
% information but also dynamic road maps, historical traffic 
% data and external compute for non-safety critical tasks. 
% We describe various components of the architecture briefly 
% below because it is similar, in some ways, to our proposed system.

% In such this architecture, remote planning and routing modules 
% perform longer timescale planning using historical data and maps 
% for efficient trip planning. It consists of eco-routing, 
% eco-driving and battery charge planning sub-modules. The 
% eco-driving and routing modules orchestrate vehicles into 
% fleets of vehicle that travel together called platoons. As platoons, 
% coordinated driving reduces frequent speed changes to increase 
% fuel efficiency. Moreover, the battery charge planning 
% module benefit from more extensive and accurate forecasts available 
% to intelligently plan recharge cycles. 

% The real-time motion planning module coordinates with the 
% remote modules to plan a paths for vehicles within the platoons 
% using cooperative adaptive cruise control. It performs  
% functions like collision avoidance and lane-changing but enhances them 
% cooperative perception and control. 
% Motion control governs the longitudinal (acceleration) and 
% lateral (steering) motion of the car along the planned path. 
% This module uses cooperative adaptive cruise control with enabled 
% by cooperative perception for closed-loop in-vehicle robustness. 
% Lastly, powertrain controls supply energy required to move the car 
% (\eg engine on/off, gear control). In a connected architecture, 
% powertrain control is more efficient because traffic forecasts 
% are made available by cooperative perception and maps and 
% this allows more-informed energy-planning.

%% End Ramesh's outline

% Background:
% - LiDAR/depth-perception: these are becoming cheap

% - Background on vehicular control (reading)
% \subsection{Vehicle Control}
% \label{sec:bg_vehicle_control}
% Based on the degree of autonomy, the Levels of Autonomous Driving:
% Level 0: human-driven
% Level 1: driver-assists like adaptive cruise control, anti-lock braking systems and electronic stability control.
% Level 2: advanced assistance such as hazard-minimizing longitudinal/lateral control [19] or emergency braking [20], [21], based upon set-based formal control theoretic methods to compute ‘worst-case’ sets of provably collision free (safe) states [22]–[24].
% Level 3: the system monitors the environment and can drive with full autonomy under certain conditions, but the human operator is still required to take control if the driving task leaves the autonomous system’s operational envelope. 
% Level 4: vehicle is capable of fully autonomous driving in certain conditions and will safely control the vehicle if the operator fails to take control upon request to intervene.
% Level 5: systems are fully autonomous in all driving modes.

% Connected vehicles:
% Improve throughput at intersections and reduce shock waves

\parab{Recent Technology Trends.}
%% - emergence of edge computing, 5G (add some citations, industry references)
Three technological trends motivate the architectural shift we consider in this paper.
% 5G
% 10 - 100x faster than 4G
% 1ms latency whereas for 4G it was 200ms
% Reaction time to visual stimulus for humans is 250 ms
5G, the fifth generation of cellular network technology~\cite{5g,Qualcomm5g,Ericsson}, promises gigabit speeds and latency as low as 1~ms. Vehicle manufacturers are standardizing 5G technologies like CV2X~\cite{QualcommCV2X} and LTE Direct~\cite{LTEDirect} for cooperative perception, path-planning, and control.
% Edge-computing
At the same time, edge-computing is moving computational resources (both CPU and GPU~\cite{nvidiaedge}) closer to data sources to support latency-critical applications~\cite{ibmedge}. By some estimates, edge-servers will handle 75\% of the processing workloads handled by the cloud today~\cite{edgegartner}. 
% Solid state lidars - S3 Quanergy
% Remove all moving parts
% A) Optical phased array B) rotating MEMS mirrors
% Has the ability to zoom in and out because we control the beam direction
% More reliable (100,000 hrs vs 293) and cheaper (100$)
Finally, LiDAR prices are falling dramatically due to competition and improved technology and manufacturing. A typical 64-beam LiDAR~\cite{Ouster,Velodyne} today costs a few thousand dollars. In the next few years LiDARs will likely cost a few hundred dollars~\cite{sslidars,huawei_lidar}. 

% \ramesh{Couple usually means 2, so if you don't mean that, use few}.
% \fawad{Yes, I was trying to say 200 dollars}

% - implications: lidAR will replace surveillance cameras, edge computing will mean that they can be processed close to the data, 5G means that information can be delivered at low-latency
% These trends point to a future in which: a) solid-state LiDARs will replace surveillance cameras for better security and privacy~\cite{OusterTracking} on the road, b) edge-compute resources can process this data 

% \ramesh{In the previous para, we might also want to cover emerging vehicle wireless technologies beyond DSRC, to show that vehicles are also taking advantage of emerging 5G.}
% \fawad{Addressed.}

% Position (every hotnets paper has to have a position :-))
\parab{\sysname: Moving Perception and Planning to Roadside Infrastructure.}
% - These trends imply that it might be possible, in the future, to decouple perception and control for autonomous driving: perception and longer-time scale control can reside in the infrastructure, while only fast timescale control resides in the network infrastructure (we call this NetDriving).
These trends suggest a future world in which LiDARs are cheap enough to mount ubiquitously on light poles (in addition to, or in place of, surveillance cameras). Edge-compute infrastructure can process LiDAR data in near real-time, and 5G can convey the results of that processing in milliseconds.

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.9\columnwidth]{figs/NetDriving_arch.png}
%   \caption{\sysname Architecture}
%   \label{fig:netd_arch}
% \end{figure}

This motivates an architectural shift for autonomous vehicle design that we call \sysname (\figref{fig:netd_arch}(b)). \sysname offloads \textit{perception and planning} to roadside infrastructure. Control remains on-board the vehicle because it involves tight sub-millisecond feedback loops.

% Given these trends, we envision, in the future, it might be possible to re-architect and decouple different components of autonomous driving. Longer-time scale planning will reside at the cloud, latency-sensitive planning and perception at the edge, whereas real-time control will stay inside the vehicle.

% Based on operation timescales mentioned in \secref{sec:background}, only the control module needs to remain in the vehicle. The whole planning module (path-planning, behavior decision, and motion planning) can stay outside the vehicle. Moreover, with fixed LiDARs, the perception module can also move to the edge where it supplies real-time sensor data to the planning module. More specifically, in the planning module, the path-planning sub-module is agnostic of sensor data, so it can be moved anywhere. It plans a path for every vehicle and sends it to the behavior decision sub-module. The behavior decision, and motion planning sub-modules have a common requirement. Both need real-time perception data. So, they are placed at the edge, near the sensing infrastructure. The behavior decision sub-module feeds its output to the motion planning sub-module. The motion planning sub-module generates a trajectory for the vehicle. It then sends this trajectory instantly to the vehicle. The vehicle converts this to low-level actuation signals to control the vehicle. 

% These architectural decouple perception and planning from low-level control, we call this \sysname.
% - this has cost and reliability benefits that we discuss below
% This has cost and reliability benefits that we discuss in detail below.

% \ramesh{The above para is a little vague and maybe confusing. First, we need to be more specific and couch this para in terms of the building blocks we identified in the previous section. Start by saying what needs to remain in the car. Then identify which pieces can move outside: behavior? motion planning? For path planning, if it doesn't use LiDAR, we can say we're agnostic; it can be implemented anywhere but its output needs to go to the motion planner etc.}
% \fawad{Addressed}

% \sysname needs: a) milli-second network latency, b) powerful compute resources at the edge, and c) ubiquitous 3D road-side sensors.
% With cost-effective 3D sensors deployed on the road, 250x lower latency than visual stimulus reaction time and powerful compute at the edge to process that data, \sysname is around the corner.

% Source for figure: https://docs.google.com/drawings/d/1eW5kuEXE6dO-kTs-xECv2STZYocAbkAxDfSgDs0zPsk/edit
\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\columnwidth]{figs/fig_sys_arch.pdf}
  \caption{\sysname architecture in an overtaking scenario from CarLA~\cite{Carla}. Roadside LiDARs transmit data over a wired network to an edge cluster. \sysname's perception extracts vehicles and their motion information, and its planning component determines that the blue vehicle can safely pass the stalled vehicle. \sysname wirelessly delivers a trajectory designed for the blue vehicle, whose control component executes the trajectory.}
  \label{fig:sys_overtaking}
%   \fawad{Note to self: replace this with a figure that shows infra sensors as well}
\end{figure}

% Overview of NetDriving
% - use a picture/scenario to maybe take one of the CarLA challenge problems (the single lane overtaking one)

% \ramesh{Put figure before parab; otherwise heading doesn't show up correctly.}
% \parab{Overview of \sysname.}
% Show that today's approaches would find difficult
% \fawad{I think we can comment out the following paragraph which shows how today's approaches will tackle this problem. It might be sufficient to just say how autonomous vehicles will tackle it} \ramesh{Sounds good, but autonomous vehicles might do roughly the same without AVR. Also, perhaps pick an intersection challenge from CarLA if there is one? Make sure to point out that this is from the CarLA challenge, not something we're making up.}
To understand how \sysname works, consider a scenario in which the blue vehicle in \figref{fig:sys_overtaking} wishes to pass a stationary red vehicle but there is an oncoming vehicle in the opposite lane. This is a well-known challenge for autonomous vehicles \cite{Carla} and for human drivers as well. In \sysname, roadside LiDARs convey point-clouds to \sysname's perception component running on an edge-compute server\footnote{In this paper, we assume that because LiDARs are statically deployed on infrastructure, they have wired connectivity. Wirelessly streaming compressed LiDAR data can ease deployment, but we have left this to future work.}. That component analyzes the scene, and outputs an abstract scene description containing vehicles and pedestrians, their velocities and heading.

\sysname's planner determines that the oncoming vehicle is far enough away that the blue vehicle can pass the stationary vehicle safely. It generates a trajectory for the blue vehicle, and transmits the trajectory over wireless to the vehicle (this is where \sysname needs 5G's low latency), whose control component effects the trajectory. To address this challenge, prior work has proposed other approaches such as directly sharing sensor readings between vehicles~\cite{AVR}; we discuss these in \secref{sec:related_work}.

\parab{Benefits.} The preceding discussion highlights two advantages of \sysname. First, well-placed infrastructure sensors can perceive more of the environment around a vehicle than sensors on the vehicle itself (in our example, a LiDAR mounted on the blue vehicle cannot see the oncoming vehicle because of the line-of-sight limitations). Second, if every vehicle were \sysname capable, then \sysname's planner could jointly plan trajectories all vehicles in the scene; in our example, \sysname could instruct the oncoming vehicle (\figref{fig:sys_overtaking}) to slow down enough to allow the blue vehicle to pass (\secref{s:planner}). These advantages can improve safety and increase roadway utilization (\secref{sec:evaluation}). 

\parab{Practical Considerations.} When deployed everywhere, \sysname can also simplify autonomous vehicle designs: they will no longer need expensive sensors thereby reducing cost~\cite{qzvehiclecost,reutersvehiclecost}, nor power-hungry on-board compute~\cite{lin18:_archit_implic_auton_drivin}, nor expensive high-definition maps~\cite{3dmapcost}.

Of course, full deployment of \sysname everywhere is unlikely anytime soon. It will likely be initially partially deployed in high-traffic areas (intersections, downtown areas, ports). Even there, it will likely be rolled out in two stages. The first stage is perception offload, in which autonomous vehicles use \sysname's perception outputs to augment their own perception. In the second stage, autonomous vehicles will use \sysname's planned trajectories in the deployed area, and then revert to its onboard autonomous stack.

We have left to future work to consider partial deployment strategies, perform an economic analysis of these deployment strategies, explore how to form public-private partnership to install infrastructure \etc In this paper, we focus on the feasibility of \sysname: we design and implement perception and planning components that meet performance requirements for autonomous vehicles described above, namely, to be able to process LiDAR frames at full frame rate and within 100~ms.

%% % In a human-driven vehicle, the blue vehicle will move out of its lane because the driver cannot see the oncoming red vehicle. However, the moment the driver sees the oncoming vehicle, they will decide to overtake or not based on the two vehicles' relative speeds and distances \etc. Today's self-driving vehicles~\cite{avovertake}, although more conservative, react similarly to the overtake scenario. Like the human-driven case above, the self-driving vehicle will move out of its lane to see oncoming traffic. It will decide to overtake based on whether it can safely do so. Such maneuvers are not only unsafe but waste fuel and time.

% % Show how autonomous vehicles would do it
% % - show how it would work in our context
% % - this description should be in sufficient detail so that the components below become clear
% % On the other hand, in \sysname, sensors deployed on the road-side will have a real-time un-occluded map of the whole road with the three vehicles. So, the behavior decision  module that lies at the edge and processes this map will: a) instruct the blue vehicle to wait in its ego-lane if the red vehicle is approaching fast, or b) tell the oncoming red vehicle to slow down for the overtake maneuver to take place. This makes the maneuver more safe, reliable, and efficient. 
% % - end by discussing what happens in autonomous vehicles today for this scenario; discuss other approaches for this scenario (AVR) and say why NetDriving would be better
% %There are, of course, other ways to solve the overtaking problem \eg by sharing raw 3D sensor data in real-time between the two red vehicles like in AVR~\cite{AVR}. Even so, in such a scenario, \sysname is more efficient and reliable because it process the sensor data only once at the edge and its centralized control enables a more coordinated response from all the vehicles.

% % Components and where they reside
% \parab{Components of \sysname.}
% %\sysname has four main components: a) point-cloud stitching, b) object detection and tracking, c) path-planning and d) delivery of low-level control signals to the vehicle.
% To realize \sysname, we re-design the high-level architecture of autonomous by adding a network module and add sub-modules to the three existing modules (perception, control, and planning) as follows (\figref{fig:sys_overtaking} illustrates this). 

% \ramesh{May need a figure here as well, perhaps rolled into the previous figure?}
% \fawad{Can you check now please? I merged CarLA and our system architecture diagram together.}

% \ramesh{Please move all the text in section 3.1 and 3.2 into a separate file called design.tex. That file should come after the deployment scenarios.}

% \subsection{Deployment Scenarios}
% \label{sec:deployment}
% % Deployment scenarios
% We envision three deployment scenarios for \sysname as follows. For 
% each scenario, we also discuss reliability and benefit costs.
% % - Full

% \parab{Full deployment.}
% % Full deployment means all vehicles will use \sysname
% % Vehicles can afford to have fewer sensors and less compute
% % For instance, cruise control will be implemented at the edge
% In a full deployment, all roads will have infrastructure sensors and edge compute. As such, all self-driving vehicles will rely on them for perception and planning. Today, self-driving cars have a plethora of on-board sensors and powerful compute platforms. This increases the price of a self-driving car by an order of magnitude relative to a human-driven vehicle~\cite{qzvehiclecost,reutersvehiclecost}. By sharing infrastructural resources amongst vehicles, \sysname can significantly lower the cost of self-driving cars. Moreover, with ubiquitous infrastructural LiDARs generating a real-time view of the road, self-driving vehicles will not need pre-built 3D maps. Collecting and building these maps would otherwise cost a few thousand dollars per kilometer~\cite{3dmapcost}.

% \ramesh{What about map collection? Point out that we may not need this as well? Reference papers about its cost.}
% \fawad{Could not find a paper but found an article instead.}

% Moreover, \sysname's centralized approach promises more reliable autonomous driving. For instance, in a full deployment, applications like adaptive cruise control (ACC) will run at the edge. With better perception and coordinated control, ACC can plan more efficient, and safer trajectories for vehicles. Similarly, \sysname can also coordinate vehicles into platoons to for safer driving and increase road throughput by 2x~\cite{varaiyaplatoons}. A platoon is set of tightly coordinated vehicles that move together through traffic~\cite{varaiyaplatoons,platooning2011}. Platooning enables efficient driving because it reduces air resistance, and frequent stops. On the other hand, it also makes driving safer because all vehicles move at the same speed with fixed headway distances.

% \ramesh{Why ACC in particular? Also point to platooning? Add references to platooning?}
% \fawad{Addressed, would ACC and platooning be enough? Or should we add more applications}

% \parab{Augmentation.}
% In this deployment, self-driving vehicles will have their on-board sensors and compute but \sysname will augment them. Augmentation deployments can help in in high-risk and high-traffic regions like accident-prone areas, traffic intersections, and highways \etc. 

% % Improving reliability through better perception
% Occlusions and line-of-sight limits a self-driving vehicle's perception~\cite{AVR}. \sysname can extend a vehicle's vision beyond its sensor range. For instance, in \figref{fig:sys_overtaking}, \sysname can send 3D sensor data (raw point clouds, bounding boxes, or occupancy grids \etc) to the blue vehicle to enable it to see more. This way, the blue vehicle can not only avoid a unsafe maneuver and also save fuel. Similarly, in traffic intersections, \sysname can inform left-turning vehicles of oncoming traffic in the opposite lanes.
% % Improving reliability through edge compute
% Similarly, \sysname can provision edge compute to self-driving vehicles for heavy, relatively less latency-sensitive computations. This way, vehicles can use on-board compute for safety-critical and latency-sensitive tasks instead.

% When \sysname is augmented in high-risk areas, self-driving vehicles can afford to have fewer on-board sensors and less powerful compute. This reduces the per unit cost of self-driving vehicles.

% \ramesh{Also point out cost implications: may need fewer sensors on cars, if, for the difficult cases, infrastructure can augment perception and planning. Discuss where the augmentation will be deployed: high-traffic areas, intersections, places with accidents. Also, augmentation doesn't have to mean point cloud transmissions, can transmit other representations such as bounding boxes etc.}
% \fawad{Addressed.}

% \parab{Backwards compatible.}
% % Backwards compatible facilitates legacy vehicles
% Human-driven vehicles can also draw benefits from \sysname through vision extension, accident warnings or emergency controls. To extend vision, \sysname can share infrastructure 3D sensor data in the driver's blind spots with the vehicle. The vehicle can then display this on a heads-up display for better perception. This can help in lane changing, overtaking, and pulling out of parking spots \etc. For accident warning, since \sysname tracks every vehicle's motion, it can warn it of potential accidents. In vehicles with on-board diagnostics ports (OBD) and the CAN bus~\cite{savage}, \sysname can also use emergency controls. To do this, after market devices that plug into the OBD can act as a relay between the edge and the vehicle's CAN bus. To avoid accidents, \sysname can send control signals for emergency braking or steering maneuvers to the vehicle's OBD  port.

% edge-servers that vehicles connect to. Edge-servers use these paths for \textit{real-time path planning}.
% \ramesh{See my comment above about cloud.}
% \fawad{Addressed, said we can place it elsewhere as well.}

%%
% - (this will need to be tied into what we write in section 2, so feel free to update section 2 if necessary)
% - end with a brief description of how this is different from existing autonomous vehicles

% \parab{Benefits.}
% % Benefits
% % - discuss the cost and reliability benefits
% % - if we can reference articles that describe costs for car manufacturers, that would be great.
% \sysname has the potential of not only enhancing the reliability but also reducing reducing the overall cost of self-driving cars. Self-driving cars have a plethora of on-board sensors (multiple LiDARs, radars, accurate GPS/inertial units, cameras\etc) and powerful compute platforms. These pieces of equipment increase the overall price of a self-driving car by an order of magnitude as compared to a human-driven vehicle~\cite{qzvehiclecost,reutersvehiclecost}. \sysname shares infrastructural resources (sensors and compute platforms) amongst all vehicles on the road and has the ability to significantly lower the overall cost of a self-driving car. Moreover, \sysname's centralized promises more predictable and reliable autonomous driving as compared to every vehicle acting independently.

% \ramesh{Perhaps discuss benefits as part of deployment scenarios?}


==> refs.tex <==
\bibliography{references.bib}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> scratch.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\begin{tabular}{lccc}
Location Accuracy & Heading Error(Degree) & Speed Error(m/s)              & Speed Accuracy(\%)             \\
                  & 5.391914203           & 0.036 & 99.061 \\
                  & 11.37604246           & 0.046 & 98.588
\end{tabular}
\end{table}
